Competitive Policy Optimization

A core challenge in policy optimization in competitive Markov decision processes is the design of efficient optimization methods with desirable convergence and stability properties. To tackle this, we propose competitive policy optimization (CoPO), a novel policy gradient approach that exploits the game-theoretic nature of competitive games to derive policy updates. Motivated by the competitive gradient optimization method, we derive a bilinear approximation of the game objective. In contrast, off-the-shelf policy gradient methods utilize only linear approximations, and hence do not capture interactions among the players. We instantiate CoPO in two ways:(i) competitive policy gradient, and (ii) trust-region competitive policy optimization. We theoretically study these methods, and empirically investigate their behavior on a set of comprehensive, yet challenging, competitive games. We observe that they provide stable optimization, convergence to sophisticated strategies, and higher scores when played against baseline policy gradient methods.

==> extra/4.5-cpg_experiment.tex <==
In this section we present an empirical study of \cpg algorithm on seven games which are linear quadratic(LQ) game, bilinear game, linear bilinear game, rock paper scissors (RPS), matching pennies (MP), Markov soccer and the game of car racing. The set covers discrete as well as continuous state action games and is a mix of both single-shot stateless and finite horizon games. Players are simultaneously trained under self play using \cpg or \gda. For evaluation purposes, we compared convergence behavior of \cpg with \gda and finally for the game of Markov Soccer and car racing \cpg trained policies have competed face to face with that of \gda. The \gda agents are trained with stochastic gradient descent. The optimizer for \cpg
% is built upon \cgd optimizer, \cite{schfer2019implicit}.  
is built using Pytorch's autograd package for evaluating gradient and bilinear terms. The formulation allows the bilinear term to be efficiently computed using the hessian vector product trick instead of computing 2D matrices. More details are in the \appx \ref{appx: }. The code and experimental videos are publicly available\footnote{https://github.com/manish-pra/Competitive-Policy-Gradient}. The experiments present here are in a zero sum game formulation but the optimizer for general sum games is also available in the same GitHub repository. 

Empirically, we see that \cpg converges to a stable point whereas \gda based algorithms diverge in the bi-linear, MP, and RPS game. Unlike \gda, where each player foolishly maximizes his reward which often leads to diverging behavior, \cpg is able to learn an opponent aware strategy. For highly strategic games, where the policy of players are tightly coupled, \cpg was able to learn much better interactive strategy, e.g., in the game of  soccer \cpg players learn to defend, dodge and score goal as compared to its counter part \gda learns to lamely score a goal if he has the ball, otherwise give way to the other players. Also, in the game of racing between 2 cars, \cpg produces competing players who learn to block and fake each other. Overall, we observe \cpg considerably outperforms, in terms of convergence, learnt strategies, and gradient dynamics. \manish{Shall keep this para here or at the end of experimentes or conclusion? I want to write a brief para summarising all experiments, because going though experiment everytime is difficult}

%  Note that the bilinear approximation of the game objective requires gradient of policy sampled with previous actions, this is evaluated by adding logarithmic probability of selecting an action recursively for a monte carlo trajectory. Pytorch's autograd package is used for evaluating gradients. For efficient implementation hessian vector product trick is used instead of computing 2D Hessian matrix. 

\subsection{Simple games: Game with known Nash Equilibrium}
% This section presents an experimental study of \cpg with \gda on environments with known Nash equilibrium. 
\subsubsection{Linear Quadratic (LQ) Game} 
In a LQ game, state and action spaces are continuous, state is propagated using linear dynamics and the cost is quadratic.
% The complete description of the game and training is in \appx~\ref{appx: LQgame}. 
The zero sum LQ game is defined by: 
\begin{gather*} \label{eqn: lq_game}
    J(K^1,K^2) = \max_{K^1} \min_{K^2} \mathbb{E} \biggl[ \sum_{k=0}^{\infty} \gamma^k \bigl({s_k}^T Q s_k + {a^1_k}^T R_{11} a^1_k   + \ {a^2_k}^T R_{22} a^2_k \bigr) \biggr] \\
    \text{where:} \ s_{k+1} = As_k + B_{1}a^1_k + B_{2}a^2_k \numberthis \\
     \qquad \qquad \quad a^1_{k+1} = -K^1s_k, \ a^2_{k+1} = -K^2s_k
\end{gather*}
where, $s_k \in R^n$ is system state vector, $a^1 \in R^{d_1}$ and $a^2 \in R^{d_2}$ are control inputs by player 1 and 2 respectively. The matrix $A \in R^{n\times n}$, $B_1 \in R^{n \times d_1}$ and $ B_1 \in R^{n \times d_2}$ describe the system dynamics. Here, $K^1$ and $K^2$ denotes the controller policies.
% Apart from comparing performance on LQ game, we introduce bilinear terms in the cost function in order to tightly couple action (interaction) of two players.  \eq~\ref{eq : lq_game}, The resulting objective function of the player 1 (player 2) is to maximise (minimise) the infinite horizon rewards, takes the form,
% \begin{gather*} \label{eq: lq_bilinear }
%     J(K^1,K^2) = \max_{K^1} \min_{K^2} \mathbb{E} \biggl[ \sum_{k=0}^{\infty} {x_k}^T Q x_k + {u^1_k}^T R_{11} u^1_k   + \ {u^2_k}^T R_{22} u^2_k +  {u^1_k}^T R_{12} u^2_k + {u^2_k}^T R_{21} u^1_k \biggr] \numberthis
% \end{gather*}
We considered a simple game where, $A = 0.9,\ B_1 = 0.8,\ B_2 = 1.5,\ R_{11} = 1,\ R_{22} = 1$. These environment parameters are not known to the players. The policy of each player is linear in the state, and actions are sampled from a Gaussian distribution $a^1\sim\mathcal{N}(\mu^1,\sigma^1)$, $a^2\sim\mathcal{N}(\mu^2,\sigma^2)$, with initial values of $\mu^1_0 = 0.1$ and $\mu^2_0=-0.1$ and $\log(\sigma^1_0)=\log(\sigma^2_0)=0.1$.
% The game dynamics and rewards follows \eq~\ref{eqn: lq_game}. 
We collected a batch of 1000 trajectories, each 5 time steps long. Both \gda and \cpg converges to the optimal control policy $(K^{1*}, K^{2*} = -0.5735,-0.3059)$, which can be obtained using coupled riccatti equation ~\citep{zhang2019policyZerosum}. 
% Both \gda and \cpg converges to the optimal control policy. 
However, we observed that with the initially collected samples \gda estimated large gradients, along with high learning rate it resulted in large steps. The resulting policy then generated erratic trajectories in the next rollout, which caused instability and thus \gda did not converge (we denoted this runs with a $\oslash$ in \tab~\ref{tab: LQgameLR})
% However, we observed that with the initially collected samples \gda estimates large gradients, when parameters are updated with larger step size, it results in arbitrary trajectory collection in the next episode and this causes instability and blows up in the subsequent iteration (denoted as $\phi$ in the table below).
\cpg is robust towards this behavior and can potentially take even larger steps. 
The number of iterations it takes to converge for different learning rates is noted in Table~\ref{tab: LQgameLR}. \fig~\ref{fig: AdvLQgame} shows the advantage estimates $\sum_{\tau} f(\tau;\theta^1,\theta^2) \sum_{k=0}^{|\tau|-1}A(s_k,a_{k}^1,a_{k}^2;\theta^1,\theta^2)$ of \gda and \cpg for different learning rates. 
%  Players are competing with each other for maximising and minimising it and hence end up driving it to zero. 
 We can see that \cpg dynamics are not just faster at the same learning rate but more importantly, \cpg allows having larger learning rates.
 
 \begin{table}[ht]
\centering 
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
 learning rate & 0.1 & 0.05 & 0.01 & 0.05 & 0.001 & 0.0001\\
 \hline \hline
 \gda & $\oslash$ & $\oslash$ & 113 & 139 & 223 & 611\\
 \hline
 \cpg & 75 & 87 & 105 & 127 & 195 & 590\\
 \hline
\end{tabular}
\caption{Number of iterations to converge to optimal policies}
\label{tab: LQgameLR}
\end{table}


\begin{figure}[h]
	\centering
    \begin{subfigure}[t]{0.23\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/LQlr_1e2.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: LQlr_1e2}
    \end{subfigure}
~
    \begin{subfigure}[t]{0.23\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/LQlr_5e3.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: LQlr_5e3}
    \end{subfigure}
   ~
    \begin{subfigure}[t]{0.23\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/LQlr_1e3.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: LQlr_1e3}
    \end{subfigure}
~
  \begin{subfigure}[t]{0.23\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/LQlr_1e4.pdf}  
    \caption{}
    \label{Fig: LQlr_1e4}
  \end{subfigure}
%  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
%   \setlength{\abovecaptionskip}{-13pt}
%   \setlength{\belowcaptionskip}{-10pt}
  \caption{Advantage estimates of LQ game at different learning rates}
  \label{fig: AdvLQgame}
\end{figure}


% \begin{figure}[ht]
%   	\centering
%   	\includegraphics[width=0.7\linewidth]{images/lq_game.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{Advantage estimates for LQ game}
%     \label{fig: AdvLQgame}
% \end{figure}

%  although we observed that \gda is sensitive to learning rates due to instability caused by competitive nature of both the players. Hence, we could take much larger steps while training with \cpg.  

% \begin{figure}[ht]
% 	\centering
%     \begin{subfigure}[t]{0.48\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/sgd_ne.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     % \caption{}
%     \end{subfigure}
%     ~
%   \begin{subfigure}[t]{0.48\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/cpg_ne.pdf}  
%     % \caption{}
%   \end{subfigure}
% %  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
% %   \setlength{\abovecaptionskip}{-13pt}
% %   \setlength{\belowcaptionskip}{-10pt}
%   \caption{Shows performance of \gda and \cpg on the LQ game (a) \gda (b) \cpg}
%   \label{Fig: LQGame}
% \end{figure}

% \subsubsection{Linear Bilinear game}
% Next, we considered a cases in which cost is given by \eq \eqref{eq: bilinear }. Here, $K^{1},K^{2}$ are controller policies, modelled as Gaussian distribution. $K^{1*} = K^{2*} = 0$ is a stationary point for this game. Different horizon lengths were considered, if its is higher, then learning rate has to be low otherwise larger steps make system unstable. With increasing horizon, \gda diverges more readily and \cpg takes more time to converge to the origin. We never observed divergence of \cpg in our experiments for reasonable learning rate for the bilinear game. \fig~\ref{Fig: LinearBilinear}, shows plots for trajectories of both the players with horizon h=2,5 for both \gda and \cpg. We trained it for 20,000 iterations, parameters for \gda and \cpg were exactly same, although \cpg could have much high lr as compared to \gda. Also, it was observed that if critic loss increases, the controller policies moves away from the origin until critic loss is reduces again this is presumably due to exploring new states.  

% \begin{gather*} \label{eq: bilinear }
%     J(K^1,K^2) = \max_{K^1} \min_{K^2} \mathbb{E} \biggl[ \sum_{k=0}^{\infty} {u^1_k}^T R_{12} u^2_k + {u^2_k}^T R_{21} u^1_k \biggr] \numberthis
% \end{gather*}


% \begin{figure}[ht]
% 	\centering
%     \begin{subfigure}[t]{0.48\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/sgd_h2.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: sgd_h2}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[t]{0.48\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/cpg_h2.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: cpg_h2}
%     \end{subfigure}
    
%     \begin{subfigure}[t]{0.48\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/sgd_bilinear_lre_h5.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: sgd_bilinear_lre_h5}
%     \end{subfigure}
% ~
%   \begin{subfigure}[t]{0.48\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}  
%     \caption{}
%     \label{Fig: cpg_bilinear_lr2_h5_critic_lr2}
%   \end{subfigure}
% %  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
% %   \setlength{\abovecaptionskip}{-13pt}
% %   \setlength{\belowcaptionskip}{-10pt}
% \protect\caption{Represents policy trajectories for player 1 and player 2. \protect\mystar{green} is start point and \protect\mystar{red} is end point. (a) \gda, h = 2 (b) \cpg, h=2 (c) \gda, h=5 (d) \cpg, h=5 }
%   \label{Fig: LinearBilinear}
% \end{figure}
% We considered game for \eq \eqref{eq: lq_bilinear }, representing mixed bilinear and quadratic costs, the results were intermediate between the 2 cases presented above.

\subsubsection{Bilinear game}
\label{sec: CPGBilinear}
In a bilinear game both players play actions simultaneously and receive rewards based on product of their actions,
\begin{align}\label{eqn: BilinearRewardxy}
    r^1(a^1,a^2) = {a^1}^\top a^2 \;\;\;\;\;\;\;\;\; r^2(a^1,a^2) = -{a^1}^\top a^2
\end{align}
% see \eq~\ref{eqn: BilinearRewardxy} for the reward function, 
where $a^1\sim\mathcal{N}(\mu_1,\sigma_1)$ and $a^2\sim\mathcal{N}(\mu_2,\sigma_2)$ are actions of player 1 and player 2 respectively. For the first episode $\mu_i, \sigma_i, i\in\{1,2\}$ are randomly policy initializations. \cpg converges to a Nash equilibrium of the game but \gda diverges for all learning rates. \fig~\ref{Fig: BilinearGame} shows this behavior for a learning rate of 0.1.
% Extensive literature exists where bilinear dynamics are studied to propose tweaks and twists in gradient dynamics to make it converge to NE. 
% In our experiment setup, player's policy is modelled as a Gaussian distribution.  $\mu_i, \sigma_i, i\in\{1,2\}$ are random policy initialization. 
% \begin{align}\label{eqn: BilinearRewardxy}
%     r^1(a^1,a^2) = {a^1}^\top a^2 \;\;\;\;\;\;\;\;\; r^2(a^1,a^2) = -{a^1}^\top a^2
% \end{align}

\begin{figure}[h!]
	\centering
    \begin{subfigure}[t]{0.3\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/sgd_bilinear_mat.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: sgd_bilinear_mat}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.3\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/cpg_bilinear_mat.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: cpg_bilinear_mat}
    \end{subfigure}
\caption{Represents policy trajectories of player 1 vs player 2 in the bilinear matrix game.  (a) \gda (b) \cpg }
%\protect\mystar{green} is start point and \protect\mystar{red} is end point.
  \label{Fig: BilinearGame}
\end{figure}

% \subsection{Matrix games}
% Experiments were conducted on various matrix games, we present results for two famous examples: Matching pennies and Rock paper scissors where \gda is known to fail.

\subsubsection{Matching pennies}
\label{sec: CPGMP}
In the matching pennies game each player has two possible actions \{Head, Tail\}. Both the players secretly turn their coin to either head or tail. If pennies matches then player 1 wins and player 2 looses, and vice versa. The game matrix is given in Table~\ref{tab: matching_pennies}. 
\begin{table}[ht]
\centering 
\begin{tabular}{|c||c|c|}
\hline
 & H & T  \\
 \hline \hline
 H & 1,-1 & -1,1   \\
 \hline
 T & -1,1 & 1,-1   \\
\hline
\end{tabular}
\caption{Game matrix for matching pennies}
\label{tab: matching_pennies}
\end{table}
The policy of a player is modeled with $K$ classes categorical distribution, where $K=2$ is the dimension of the Matching pennies game. Players are randomly initialized and sample actions from softmax probability function. They receive rewards for their actions according to the game matrix. We collect a batch of 1000 trajectories, to estimate gradient and bilinear terms for every update iteration. \cpg converges to the unique Nash equilibrium of the game $\bigl(\frac{1}{2}, \frac{1}{2} \bigr)$, whereas \gda diverges for all learning rates. \fig~\ref{Fig: gda_matching_pennies} shows this behavior for learning rate of 0.1. 
\begin{figure}[ht]
\centering
    \begin{subfigure}[t]{0.3\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/gda_matching_pennies.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: sgd_matching_pennies}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.3\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/cpg_matching_pennies.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: cpg_matching_pennies}
    \end{subfigure}
\caption{Represents probability of selecting actions for player 1 in the matching pennies game. Player 2 is omitted, it has similar trajectory. (a) \gda (b) \cpg }
  \label{Fig: gda_matching_pennies}
\end{figure}

\subsubsection{Rock paper scissors}
\label{sec: CPGRPS}
Rock paper scissors game is played between two players, each player has three possible actions \{Rock, Paper, Scissors\}. Both players will simultaneously display one of three actions: a rock, paper, or scissors. A rock beats scissors, scissors beat paper by cutting it, and paper beats rock by covering it. This is captured in the game matrix given by~\ref{tab: rock_paper_scissors}. 

\begin{table}[ht]
\centering 
\begin{tabular}{|c||c|c|c|}
\hline
 & Rock & Paper & Scissors  \\
 \hline \hline
 Rock & 0,0 & -1,1 & 1,-1   \\
 \hline
 Paper & 1,-1 & 0,0 & -1,1   \\
 \hline
 Scissors & -1,1 & 1,-1 & 0,0   \\
\hline
\end{tabular}
\caption{Game matrix for rock paper scissors}
\label{tab: rock_paper_scissors}
\end{table}
Similar to the game of matching pennies, Player's policy is modeled with $K$ classes categorical distribution, where $K=3$ is the dimension of the RPS game. Players are randomly initialised and sample actions from softmax probability function over categorical distribution. They receive rewards for their actions according to the game matrix. We collect a batch of 1000 trajectories for every update iteration. \cpg converges to the only Nash equilibrium of the game, where probability of playing $(Rock, Paper, Scissors) = (\frac{1}{3},\frac{1}{3},\frac{1}{3})$, whereas \gda diverges for all learning rates. \fig~\ref{Fig: gda_rps} shows this behavior for learning rate = 0.1.
% After every update, players play with updated policies and the game continues until convergence to NE or divergence of the policies.
% \fig~\ref{Fig: gda_rps} shows that  and the \gda diverges. Note that a softmax layer is used due to which GDA rotations is restricted between 0-1. 

\begin{figure}[ht]
	\centering
	    \begin{subfigure}[t]{0.3\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/gda_rps.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: sgd_rps}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.3\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/cpg_rps.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: cpg_rps}
    \end{subfigure}
\caption{Represents probability of selecting actions from \{rock, paper, scissors\} of player 1 in the RPS game. (a) \gda (b) \cpg }
  \label{Fig: gda_rps}
\end{figure}
% \subsubsection{Rival actions}

\subsection{Markov Soccer Game}
\label{sec: CPGMarkovSoccer}
\begin{figure}[ht]
  	\centering
  	\includegraphics[width=0.4\linewidth]{images/Soccer.pdf}
    \caption{The Markov Soccer Game}
    \label{fig: soccer}
\end{figure}
The Markov soccer game is shown in \fig~\ref{fig: soccer}. It is a two-player game, where agents are supposed to pick up the ball and put in opponents' goal. The winner receives a +1 reward and -1 is awarded to the losing player. The game and training description is in \appx~\ref{appxsec: soccer}. For comparison between \cpg vs \gda, we played 10000 games between them, in which for 50\% of the games, \cpg was player A and for remaining \gda was player A. \cpg won more than 74\% games against \gda as shown in \fig~\ref{Fig: sgd_cpg_winning_plot}. \cpg was able to learn better tactics for seizing ball, dodging and defending its goal post. 
In order to capture this interaction between players, we recorded the number of times the ball is seized between the players before one player finally scores a goal. \fig~\ref{Fig: InteractionBilinear}[a,b,c], show interaction plots (description in the caption).
The interaction plots show that \cpg player learns smart interactive strategies of seizing ball from the opponent and scoring a goal, whereas \gda could hardly take the ball from \cpg (\fig~\ref{Fig: cpg_sgd_interaction_plot} x=4) when competed against each other. Also, only the \cpg vs \cpg game has 0 on the x axis which represents the case, where both players kept snatching the ball from each other and no one could score a goal within the episodic length. 

\begin{figure}[h]
	\centering
    \begin{subfigure}[t]{0.23\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/cpg_cpg_interaction_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: cpg_cpg_interaction_plot}
    \end{subfigure}
~
    \begin{subfigure}[t]{0.23\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/cpg_sgd_interaction_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: cpg_sgd_interaction_plot}
    \end{subfigure}
   ~
    \begin{subfigure}[t]{0.23\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/sgd_sgd_interaction_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: sgd_sgd_interaction_plot}
    \end{subfigure}
~
  \begin{subfigure}[t]{0.23\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/sgd_cpg_winning_plot.pdf}  
    \caption{}
    \label{Fig: sgd_cpg_winning_plot}
  \end{subfigure}
%  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
%   \setlength{\abovecaptionskip}{-13pt}
%   \setlength{\belowcaptionskip}{-10pt}
  \caption{a) \cpg vs \cpg, b) \cpg vs \gda, c) \gda vs \gda. a,b,c are interaction plots.  X-axis convention, 1: A scored goal, 2: B scores goal, 3: A scored goal after seizing ball from B. 4: B scores goal after seizing ball from A, 5: A scored goal by seizing ball from B which took the ball from A and so forth. 0: No one scores goal both kept on seizing from each other for 1000 steps.
%   Similarly, Ceil[x/2] denotes the number of times ball has been seized from each other before scored by player A (x=odd) or player B (x=even), where x is the x-axis index
  d) Shows probability of games won when \cpg competed against \gda}
  \label{Fig: InteractionBilinear}
\end{figure}

\subsection{Car Racing game}
\label{sec: CPG_ORCA}
Our final experimental setup is a racing game between two race cars, where the goal is to finish the race first. The test track which consists of 13 turns with different curvature can be seen in Figure \ref{Fig: orca}. The game involves both, learning a policy that can control a car at the limit of handling, as well as strategic interactions with the opposing car. The complete description of the game and training is in \appx~\ref{appx: ORCADescription}. Here we explain reward shaping to give intuition behind the competition involved. To formulate the racing game between two cars, we convert the objective of finishing the race first without an accident into a zero sum game. First to model our no accident constraints we use a freezing mechanism:
% (where one car is frozen and other is allowed to ear rewards): 
(i) If the car is leaving the track we freeze it until the episode ends, 
(ii) If the cars collide, the rear car is stopped for 1s. Note that this gives an advantage to the car ahead, but in car racing, the following car has to avoid collisions. 
(iii) The car which finishes first gets a +1 reward and the other car gets -1 reward. Furthermore, an episode ends if both cars are either frozen due to leaving the track or the first car finished the lap. 
(iv) Finally, to reward racing the players at every time step receive the following reward $r(s_k,a^1_{k+1},a^2_{k+1}) = \Delta \rho_{car_1} - \Delta \rho_{car_2}$, where $\Delta \rho = \rho_{k+1} - \rho_k$. $\rho$ is a progress of the car at $k^{th}$ time step in the track. This reward encourages the player to get as far ahead of the opponent player as possible. 

We trained the racing game with both \gda and \cpg, even though both players were able to learn to "drive" only \cpg was able to learn how to ``race". With \gda, only one player was able to learn, this either manifested in one player completely failing and the other finishing the race, or by an oscillation behavior where when one agent learns to go ahead, the other agent learns to stay at lower progress. Even if at some point one of the players learns to finish one lap, the player does not learn to interact with the other opponent. The players trained with \cpg on the other hand, both progress and learn to finish the lap and to interact with each other. See \fig~\ref{fig: ProgressOrcaCPG}, where the progress the two players at the end of an episode can be seen for \gda and \cpg, it is clearly visible that with \cpg both players get better over time, whereas in \gda the two player have an oscillation behavior, and at the end, only one of the two players finishes one lap. 

\begin{figure}[h!]
	\centering
    \begin{subfigure}[t]{0.32\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/orca_sgd.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: orca_sgd}
    \end{subfigure}
    ~
%     \begin{subfigure}[t]{0.32\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/orca_sgd_swing.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{fig: orca_trpo_gdap2}
%     \end{subfigure}
%     ~
    \begin{subfigure}[t]{0.32\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/orca_cpg_progress_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: orca_cpg_progress_plot}
    \end{subfigure}
  \caption{Progress of agents while training a) \gda b) \cpg both at  learning rate = 5e-5}
  \label{fig: ProgressOrcaCPG}
\end{figure}

To test the policies, we run 5000 episodes with the obtained policy. To evaluate the performance we run three types of races, \gda vs \gda, \cpg vs \cpg, \gda vs \cpg. For each episode, we counted the number of overtakes, the number of collisions with the track constraints, and recorded the lap time. For the \gda vs \cpg test we also counted the number of times which policy won, where we defined winning as finishing first. Since, \gda often collided with the track constraints, for the test, we replaced the freezing with a reset at the reference path routine. 

\begin{table}[ht]
\centering 
\begin{tabular}{|c||c|c|c|}
\hline
 & \cpg vs \cpg & \gda vs \gda \\
 \hline \hline
 Overtaking per lap & 3.35 & 0.68  \\
 \hline
 Track collision per lap & 0.59 & 1.12  \\
 \hline
 Laptime  & 10.89 & 13.32  \\
 \hline
\end{tabular}
\caption{Quantitative results for the racing game}
\label{tab: orca_same_players}
\end{table}

% \begin{table}[ht]
% \centering 
% \begin{tabular}{|c||c|c|c|}
% \hline
%  & \cpg vs \cpg & \gda vs \gda \\
%  \hline \hline
%  Overtaking per lap & 16772/3.35 & 3419/0.68  \\
%  \hline
%  Track collision per lap & 2941/0.59 & 5613/1.12  \\
%  \hline
%  Laptime  & 10.89 & 13.32  \\
%  \hline
% \end{tabular}
% \caption{Quantitative results for the racing game}
% \label{tab: orca_same_players}
% \end{table}

In Table \ref{tab: orca_same_players} we can clearly see that \cpg learned a policy that is both faster and more precise, as well as more interactive with about six times as many overtaking maneuvers. Thus, it is not surprising that in the 5000 race between \gda vs \cpg, \gda was only able to win 103 times. For these races, we also noted that the \gda player, go ``confused" by the interactive \cpg player which resulted in crashes of the \gda player, since the \gda player never experience such interactions in training. 

% Finally we want to study the type of strategies the \cpg players learned for overtaking and blocking. First, the player which is ahead clearly learned that he/she has strategic advantage, and on purpose braked to cause a freezing the following player. This strategy on the other hand resulted in adequate overtaking strategy which involved a significant safety distance.....

% The ORCA setup is developed at ETH Zurich for the purpose of developing high speed and real time path planning and control algorithms. The ORCA simulator uses dynamic bicycle model ($Cite car model$) and tire forces are modelled using Pacejka Magic formula 6.2 ($Cite mf$), further details are in appendix. The state $x \in R^n$ of race car is formulated in curvilinear coordinates, given by $ x = [\rho, d, \mu, V_x, V_y, \psi]^T$ where, $\rho$ is progress along a reference path, $d$ is deviation from a reference path, $\mu$ is heading deviation from a reference path, $V_x$ is longitudinal velocity in car frame, $V_y$ is lateral velocity in car frame and $\psi$ is yawrate of the car.

% The reference path can be any line in the track, for our experiments we took a laptime optimised trajectory. The control inputs are $[D, \delta]^T$, where $D \in [-0.2, 1]$ is throttle varying from full braking at -0.2 to full acceleration at 1 and $\delta \in [-0.35, 0.35]$ is steering angle from extreme left to extreme right. The dynamics are propagated using RK4 integrator. The track shown in \fig~\ref{Fig: orca}, tries to capture trajectory of varying bend radius, ranging from straights to $180^0$ turns in both left hand and right hand curvatures. 

\begin{figure}[ht]
  	\centering
  	\includegraphics[width=0.6\linewidth]{images/overtaking_manuever_northsouth.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption[Caption for LOF]
    {Overtaking maneuvers\footnotemark of \cpg agents in the Car Racing Game. The thick line shows trajectory when the loosing agent overtook.}
    \label{Fig: orca}
\end{figure}
\footnotetext{Video is available here}
% maneuvers\footnote{Video is available here}
% The ORCA setup is extended to the multi-car setup, for training under full observability we define state for car $i \in \{1,2\}$ as  $[state_{car_i}, state_{car_{i-}}]^T$, where $state_{car_i} = [\rho, d, \mu, V_x, V_y]^T$. Please note the $\psi$ dropped to reduce state size. The game starts with both the cars placed at start line which is $\rho = 0$ and randomly assigned $d \in \{0.1, -0.1\}$. The aim for each car is to beat the opponent by finishing as soon as possible and while avoiding collision and track boundaries. This task is formulated as zero sum game with reward shaping given below:
% \begin{itemize}
%     \item $r(s_k,a^1_{k+1},a^2_{k+1}) = \Delta \rho_{car_1} - \Delta \rho_{car_2}$, 
%     $\Delta \rho = \rho_{k+1} - \rho_k$
%     \item Track constraints are incorporated using a freezing mechanism, once a car hits the track boundary, its state is not propagated any more and hence $\Delta \rho_{car_i} = 0$ and based on performance of other car it receives a penalty. This reward structure indirectly penalises a car more if it hits in the beginning as compared to later.
%     \item Collisions constraints are similar to prey-predator game, the rear car is penalised for collision where as car in the front is awarded to promote blocking. Following freezing mechanism, here also we freeze the rear car but only for 0.1 seconds.
%     \item The car's state trajectory is collected by propagating until one of them reaches finish line or both cars reach freezing state.
% \end{itemize}

% This experiment was used to compared performance of \gda and \cpg. The naive \gda failed to converge where as \cpg was able to drive but had hard time learning more than 30\% of the track. We extended formulation of \gda and \cpg to adapt learning rate using RMS prop. Both are trained for 20000 episodes, for each episode we do a batch update. The batch is formed using 8 game trajectories, where the maximum trajectory length is restricted to 700 steps. Under give parameters, it takes 13 hours to train on a single core cpu and has been trained for 8 different random seeds. The algorithms are tuned for learning rates. We observed that a few times \gda faces oscillation while training i.e., when an player maximises his progress, the other player performance shrink to a low progress, hence the player learns to drive but given that the other player has low progress. Due to this once the learnt player is competed with strong opponent e.g., itself, then the both players tend to go out due to unforeseen state space during training. In case of \cpg, we observe that both player are trained together to maximise their progress. \cpg was able to learn the strategy of blocking and avoiding collisions. Further we competed \cpg with \gda with either of them as player 1 and player 2. The player with higher progress at the end of the game is declared as winner. We selected best trajectories according to maximum progress during training, and played 5000 games. During test, we reset player to center of the track upon collision with the track boundaries, for competitiveness between players. Table~\ref{tab: orca_same_players}, shows results for game between \cpg vs \cpg and \gda vs \gda. The trained players with \cpg tries to block and overtakes more often through out the track as compared to \gda where the player hardly overtakes apart from the start zone. \gda had hard time for both players to reach to the goal together, this is presumably due to unexplored state space. On competing with \cpg with \gda, \cpg wins almost all the matches due to better interactive strategies learnt by \cpg player. \manish{Make trajectory plot showing blocking and avoiding collision}  

% \begin{table}[ht]
% \centering 
% \begin{tabular}{|c||c|c|c|}
% \hline
%  & CPG vs CPG & GDA vs GDA \\
%  \hline \hline
%  Overtaking & 16772 & 3419  \\
%  \hline
%  Collosions & 2941 & 5613  \\
%  \hline
%  Laptime  & 10.89 & 13.32  \\
%  \hline
% \end{tabular}
% \caption{Comparative results for self-play on the ORCA setup}
% \label{tab: orca_same_players}
% \end{table}

% \begin{table}[ht]
% \centering 
% \begin{tabular}{|c||c|c|c|c|}
% \hline
%  & \multicolumn{2}{c|}{CPG vs GDA} &  \multicolumn{2}{c|}{GDA vs CPG} \\
%  \hline \hline
% %  \cline{2-5}
%  Wins & 4873 & 127 & 103 & 4897  \\
%  \hline
%  Overtaking  & 6324 & 3021 & 1927 & 5830  \\
%  \hline
%  Collosions & 2113 & 5114 & 5642 & 1943  \\
%  \hline 
% \end{tabular}
% \caption{Comparative results for \cpg vs \gda on the ORCA setup}
% \label{tab: orca_diff_players}
% \end{table}

% \manish{to do: Make histogram of number of overtakes/blocking for cpg vs cpg and gda vs gda, laptime for gda and cpg, Number of wins for cpg vs gda, number of collosions }
% Out of 5000, for 50\% games, \gda was player 1 for remaining 50\% \cpg was player 1. As shown in the histogram below, we observe that \cpg won 68\% games, among all the collisions and blocking in the games 84\% times victim was policy trained using \gda.       

==> extra/4.6-cpg_experiment.tex <==
\kamyar{Manish, at some point add a discussion on self play, and explain in symmetric game one can do deploy \cpo in self-play setting. Also run it on soccer game and study it in term of performance, and sensitivity. }




In this section, we empirically study the performance of \gda, and \cpg on six representative series of games, ranging from single-state repeated games to general sequential games, and categorical games with finite states/actions to infinite/continuous states/action: 1) linear-quadratic(LQ) game, 2) bilinear game, 3) matching pennies (MP), 4) rock paper scissors (RPS),  5) Markov soccer, and 6) car racing. These games are primitive enough that their study provides insightful conclusions, and at the same time challenging enough, to carry the core difficulties and interactions in competitive games. On a variety of experiment settings, we show that \cpg converges to stable points in the game, and learns opponent aware strategy, whereas \gda's greedy approach shows poor performance and even diverges when applied on the bi-linear, MP, and RPS games. 
%
In highly strategic games, where the policy of players are tightly coupled, we show that \cpg learns much better interactive strategy, e.g., in the soccer game, \cpg players learn to defend, dodge and score goal whereas each \gda player learns how to score when it is initialized with the ball, and give way to the other player otherwise. When a \cpg trained agent compete with \gda trained agent, we observe significant superior of \cpg agent. In the game of car racing, while \gda shows poor performance, \cpg produces competing players which learn to block and fake each other. Generally, we observe that \cpg considerably outperforms, in terms of convergence, learnt strategies, and gradient dynamics. 

% We observe that \cpg converges to a stable point whereas \gda based algorithms diverge in the bi-linear, MP, and RPS game. Unlike \gda, where each player foolishly maximizes his reward which often leads to diverging behavior, \cpg is able to learn an opponent aware strategy. 

We implement \gda, and \cpg on Pytorch platform~\citep{NEURIPS2019_9015}, and made the code and the videos publicly %\footnote{https://github.com/manish-pra/Competitive-Policy-Gradient}
. In our \gda/\cgd implementation, we deploy Pytorch's autograd package as well as Hessian vector product approach to efficiently compute the gradients and Hessian vector product to compute the bilinear terms in the optimzers.  Moreover, we use conjugate gradient trick to efficiently computed the inverses in \eq\ref{eqn: CGDSolution} which incurs a minimal computational overhead.(see \citep{CG_Jonathan1994} for more details) Moreover we compute inverse matrix vector product only for one player strategy let say $\Delta \theta^1$, and use optimal counter strategy for other player $\Delta \theta^2$ which can be computed without inverse matrix vector product. Also, the last optimal strategy can be used for warm start of conjugate gradient which ease in convergence. 
% \kamyar{Manish, can you elaborate here on the computation?} 
% In the following we split the study to two sections, \textbf{(I)} games that we have their closed form Nash equilibria (games 1,2,3,4), and \textbf{(I)} those that we do not (games 5,6).





% \subsubsection{Games with known Nash Equilibrium}
\paragraph{Games with known closed-form Nash equilibrium (games 1,2,3,4)}
Firstly, we considered a \textbf{zero sum LQ game} defined by \eq~\ref{eqn: lq_game} which is studied theoretically and have convergence guarantees ~\citep{zhang2019policyZerosum}. This makes LQ game an ideal platform to compare range of allowable step sizes and convergence rate of \cpg with \gda.
% In a LQ game, state and action spaces are continuous, state is propagated using linear dynamics and the cost is quadratic.
\begin{gather} \label{eqn: lq_game}
    J(K^1,K^2) = \max\nolimits_{K^1} \min\nolimits_{K^2} \mathbb{E}\big[  \sum\nolimits_{k=0}^{\infty} \gamma^k \bigl({s_k}^T Q s_k + {a^1_k}^T R_{11} a^1_k   + \ {a^2_k}^T R_{22} a^2_k \bigr)\big]  \\
    \text{where:} \ s_{k+1} = As_k + B_{1}a^1_k + B_{2}a^2_k,~\textit{and} \ \  a^1_{k+1} = -K^1s_k, \ a^2_{k+1} = -K^2s_k \nonumber
\end{gather}

In the LQ game (defined further in \appx~\ref{appxsec: LQgame}), we observed that with the initially collected samples \gda estimated large gradients, along with high learning rate it resulted in large steps. The resulting policy then generated erratic trajectories in the next rollout, which caused instability and thus \gda did not converge (we denoted this runs with a $\oslash$ in \appx \tab~\ref{tab: LQgameLR}). \cpg is robust towards this behavior and can potentially take even larger steps. \fig~\ref{fig: LQlr_1e2} shows the advantage estimates $\sum_{\tau} f(\tau;\theta^1,\theta^2) \sum_{k=0}^{|\tau|-1}A(s_k,a_{k}^1,a_{k}^2;\theta^1,\theta^2)$ of \gda and \cpg for different learning rates. We can see that \cpg dynamics are not just faster at the same learning rate but more importantly, \cpg allows having larger learning rates.
% as shown in \fig~\ref{fig: LQlr_1e2}.
Experiment details and results are documented in \appx~\ref{appxsec: LQgame}. 
\begin{figure}[h]
	\hspace{-3.00mm}
	\centering
    \begin{subfigure}[t]{0.27\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/LQlr_1e2.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: LQlr_1e2}
    \end{subfigure}
    \hspace{-6.00mm}
~
    \begin{subfigure}[t]{0.27\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/combined_bilinear_mat.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: combined_bilinear_mat}
    \end{subfigure}
    \hspace{-6.00mm}
   ~
    \begin{subfigure}[t]{0.27\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/combine_matching_pennies.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: combine_matching_pennies}
    \end{subfigure}
    \hspace{-6.00mm}
~
  \begin{subfigure}[t]{0.27\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/combined_rps.pdf}  
    \caption{}
    \label{fig: combined_rps}
  \end{subfigure}
  \hspace{-4.00mm}
%  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
%   \setlength{\abovecaptionskip}{-13pt}
%   \setlength{\belowcaptionskip}{-10pt}
  \caption{\cpg (C) vs \gda (G) behaviour on a) LQ game b) Bilinear Game c) Matching Pennies, Head(H) Tail(T) d) Rock(R) Paper(P) Scissors(S)}
  \hspace{-4.00mm}
\end{figure}
Next we considered a single shot \textbf{bilinear game}, where players exhibit a strong non cooperative behavior. \gda is known to diverge in the bilinear game and hence, it is widely studied to propose other gradient based optimizers ~\citep{BalduzziHamiltonian}.
In a bilinear game both players act simultaneously and receive a rewards based on product of their actions, $r(a^1,a^2) = {a^1}^\top a^2$ where $a^1\sim\mathcal{N}(\mu_1,\sigma_1)$ and $a^2\sim\mathcal{N}(\mu_2,\sigma_2)$.
% Players aim to learn optimal policies $(\mu_1,\mu_2)$.
In the bilinear game, \gda diverges for all learning rates, whereas \cpg converges to the Nash equilibrium of the game as shown in the \fig~\ref{fig: combined_bilinear_mat}.
% shows this behavior for a learning rate of 0.1.

Next we considered Matrix games, particularly \textbf{Matching pennies} and \textbf{Rock paper scissors}. The games are challenging and require an opponent aware optimization. The unique Nash equilibrium of these games is a mixed strategy. Traditionally, the games are approached with fictitious play, counterfactual regret methods ~\citep{CFR_RPS}.
% The game matrices are shown in the \tab~\ref{tab: rock_paper_scissors} , \ref{tab: matching_pennies}. 
\cpg converges to the unique Nash equilibrium of the MP \fig~\ref{fig: combine_matching_pennies} and RPS \fig~\ref{fig: combined_rps}, whereas \gda moves away from the Nash equilibrium for all learning rates. \gda actually approaches near deterministic strategies that are easily exploitable by other deterministic strategies leading to unstable learning. In contrast, \cpg agents learn to play the unique mixed Nash strategy, where players anticipate that exploiting a deviation from the Nash equilibrium increases their immediate return, but also renders them to be more exploitable by the opponent. More details and results are documented in \appx~\ref{appxsec: CPGMP} and \appx~\ref{appxsec: CPGRPS}.

% \begin{table}[ht]
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{|c||c|c|c|}
% \hline
%  & Rock & Paper & Scissors  \\
%  \hline \hline
%  Rock & 0,0 & -1,1 & 1,-1   \\
%  \hline
%  Paper & 1,-1 & 0,0 & -1,1   \\
%  \hline
%  Scissors & -1,1 & 1,-1 & 0,0   \\
% \hline
% \end{tabular}
% \caption{Game matrix for rock paper scissors}
% \label{tab: rock_paper_scissors}
% }
% \hfill
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{|c||c|c|}
% \hline
%  & Head & Tail  \\
%  \hline \hline
%  Head & 1,-1 & -1,1   \\
%  \hline
%  Tail & -1,1 & 1,-1   \\
% \hline
% \end{tabular}
% \caption{Game matrix for matching pennies}
% \label{tab: matching_pennies}
% }
% \end{table}


\subsubsection{Markov Soccer}
\label{sec: CPGMarkovSoccer}
The Markov soccer used here is similar to the one defined in ~\citet{littmansoccer} ~\citet{HeHeOppo}. Although both \gda and \cpg converge in this game, it is a strategic game where a smart agent learns sophisticated strategies of defending, dodging and scoring. The Markov soccer game is shown in \fig~\ref{fig: Soccer}. It is played between 2 players, where agents are supposed to pick up the ball and put in the opponents' goal. The winner receives a +1 reward and -1 is awarded to the losing player. The game and training is described in detail in \appx~\ref{appxsec: soccer}. 

For a comparison between \cpg and \gda, we played 10000 games between them, where in 50\% of the games, \cpg was player A and for the remaining \gda was player A. \cpg won more than 74\% of all games against \gda as shown in \fig~\ref{Fig: sgd_cpg_winning_plot}. 
In order to capture interaction between players, we recorded the number of times the ball is seized between the players before one player finally scores a goal. \fig~\ref{Fig: InteractionBilinear}[a,b,c], show interaction plots (description in the caption). In, \cpg vs \cpg game we see twice more probability of seizing ball as compared to \gda vs \gda (see x=3, x=4 in \fig~\ref{Fig: cpg_cpg_interaction_plot} vs \fig~\ref{Fig: sgd_sgd_interaction_plot}). Also in the match between \cpg vs \gda, \cpg agent could take balls 50\% of the time from \gda agent but \gda can hardly take ball back from \cpg. \cpg was able to learn better tactics for seizing and dodging the ball, as well as defending its goal post. 

\begin{figure}[h]
\hspace{-4.00mm}
	\centering
    \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/cpg_cpg_interaction_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: cpg_cpg_interaction_plot}
    \end{subfigure}
    \hspace{-5.00mm}
   ~
    \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/sgd_sgd_interaction_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: sgd_sgd_interaction_plot}
    \end{subfigure}
    \hspace{-5.00mm}
    ~
    \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/cpg_sgd_interaction_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: cpg_sgd_interaction_plot}
    \end{subfigure}
    \hspace{-5.00mm}
~
  \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/sgd_cpg_winning_plot.pdf}  
    \caption{}
    \label{Fig: sgd_cpg_winning_plot}
  \end{subfigure}
  \hspace{-4.00mm}
%  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
%   \setlength{\abovecaptionskip}{-13pt}
%   \setlength{\belowcaptionskip}{-10pt}
  \caption{a) \cpg vs \cpg, b) \gda vs \gda, c) \cpg vs \gda. a,b,c are interaction plots.  X-axis convention, 1: A scored goal, 2: B scores goal, 3: A scored goal after seizing ball from B. 4: B scores goal after seizing ball from A, 5: A scored goal by seizing ball from B which took the ball from A and so forth. 0: No one scores goal both kept on seizing from each other for 1000 steps.
%   Similarly, Ceil[x/2] denotes the number of times ball has been seized from each other before scored by player A (x=odd) or player B (x=even), where x is the x-axis index
  d) Shows probability of games won when \cpg competed against \gda}
  \label{Fig: InteractionBilinear}
\end{figure}

\begin{figure}[h]
{
    \begin{subfigure}[t]{0.40\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/Soccer.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
\vspace{-6.00mm}
    \caption{}
    \label{fig: Soccer}
    \end{subfigure}
    \hspace{-10.00mm}
    
\vspace{-45.00mm}
    
   	\hspace{-5.00mm}
    \begin{subfigure}[t]{0.25\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/orca_sgd.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: orca_sgd}
    \end{subfigure}
    \hspace{-6.00mm}
~
  \begin{subfigure}[t]{0.25\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/orca_cpg_progress_plot.pdf}  
    \caption{}
    \label{fig: orca_cpg_progress_plot}
  \end{subfigure}
  \hspace{-6.00mm}
}
    ~
    \begin{subfigure}[t]{0.65\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/overtaking_manuever_northsouth.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: overtaking_manuever_northsouth}
    \end{subfigure}
    \hspace{-12.00mm}
    
    \caption[Caption for LOF]
    {a) The Markov Soccer Game, b \& c) Normalised Progress of agents while training in the car racing game b) \gda c) \cpg ) corresponds to start line and 1 is Lap finish d) Overtaking maneuvers\footnotemark of \cpg agents in the Car Racing Game. The thick line shows trajectory when the trailing agent overtook.}
    \label{Fig: orca}
  \hspace{-4.00mm}
  \vspace{-5.00mm}
\end{figure}
\footnotetext{Video is available here}
% \vspace{-10.00mm}
\subsubsection{ORCA Racing}
\label{sec: CPG_ORCA}
Our final experimental setup is a racing game between two race cars, where the goal is to finish the race first. The game involves both, learning a policy that can control a car at the limit of handling, as well as strategic interactions with the opposing car. The test track which consists of 13 turns with different curvature can be seen in \fig~\ref{Fig: orca}. The game is formulated as a zero-sum, with reward $r(s_k,a^1_{k},a^2_{k}) = \Delta \rho_{car_1} - \Delta \rho_{car_2}$, where $\Delta \rho = \rho_{k+1} - \rho_k$ and $\rho_k$ is a progress of the car till $k^{th}$ time step in the track. If a car crosses track boundaries, then it is freezed i.e ($\Delta \rho = 0$), which results in its penalization using the above reward formulation corresponding to the $(\Delta \rho)$ of the other agent. Similarly during a collision, the rear car is freezed, which penalizes it and the car in the front receives positive rewards. This formulation promotes blocking by the car in front, overtaking by the car in the rear.  
% Here we explain reward shaping to give intuition behind the competition involved. To formulate the racing game between two cars, we convert the objective of finishing the race first without an accident into a zero sum game. First to model our no accident constraints we use a freezing mechanism:
% % (where one car is frozen and other is allowed to ear rewards): 
% (i) If the car is leaving the track we freeze it until the episode ends, 
% (ii) If the cars collide, the rear car is stopped for 1s. Note that this gives an advantage to the car ahead, but in car racing, the following car has to avoid collisions. 
% (iii) The car which finishes first gets a +1 reward and the other car gets -1 reward. Furthermore, an episode ends if both cars are either frozen due to leaving the track or the first car finished the lap. 
% (iv) Finally, to reward racing the players at every time step receive the following reward $r(s_k,a^1_{k+1},a^2_{k+1}) = \Delta \rho_{car_1} - \Delta \rho_{car_2}$, where $\Delta \rho = \rho_{k+1} - \rho_k$. $\rho$ is a progress of the car at $k^{th}$ time step in the track. This reward encourages the player to get as far ahead of the opponent player as possible. 

We trained the racing game with both \gda and \cpg, even though both players were able to learn to "drive" only \cpg was able to learn how to ``race". With \gda, only one player was able to learn, this either manifested in one player completely failing and the other finishing the race, or by an oscillation behavior where when one agent learns to go ahead, the other agent learns to stay at lower progress. Even if at some point one of the players learns to finish one lap, the player does not learn to interact with the other opponent. The players trained with \cpg on the other hand, both progress and learn to finish the lap and to interact with each other. See \fig~\ref{fig: orca_cpg_progress_plot} and \fig~\ref{fig: orca_sgd}, where the progress the two players during training can be seen for \gda and \cpg, it is clearly visible that with \cpg both players get better over time, whereas in \gda the two player have an oscillation behavior, and at the end, only one of the two players finishes the lap. 

% To test the policies, we run 5000 episodes with the obtained policy. To evaluate the performance we run three types of races, \gda vs \gda, \cpg vs \cpg, \gda vs \cpg. For each episode, we counted the number of overtakes, the number of collisions with the track constraints, and recorded the lap time. For the \gda vs \cpg test we also counted the number of times which policy won, where we defined winning as finishing first. Since, \gda often collided with the track constraints, for the test, we replaced the freezing with a reset at the reference path routine. 

To test the policies, we performed 10000 races between \cpg and \gda, with \cpg as player 1 in half of them. The \tab~\ref{tab: orca_diff_players} shows the normalised score. we can clearly see that \cpg learned a policy that is both faster and more precise. Although \gda was able to overtake, almost all of it's overtaking maneuvers leads to crash with the track boundaries. 

\begin{table}[ht]
\centering 
\begin{tabular}{|c||c|c|c|c|}
\hline
 & \multicolumn{2}{c|}{CPG vs GDA} &  \multicolumn{2}{c|}{GDA vs CPG} \\
 \hline \hline
%  \cline{2-5}
 Wins & 1 & 0 & 0 & 1  \\
 \hline
 Overtaking  & 1.68 & 1.01 & 1.04 & 1.65  \\
 \hline
 Collosions & 0.28 & 1.33 & 1.46 &  0.23  \\
 \hline 
\end{tabular}
\caption{Comparative results for \cpg vs \gda on the ORCA setup}
\label{tab: orca_diff_players}
\end{table}

% \begin{table}[ht]
% \centering 
% \begin{tabular}{|c||c|c|c|}
% \hline
%  & \cpg vs \cpg & \gda vs \gda \\
%  \hline \hline
%  Overtaking per lap & 3.35 & 0.68  \\
%  \hline
%  Track collision per lap & 0.59 & 1.12  \\
%  \hline
%  Laptime  & 10.89 & 13.32  \\
%  \hline
% \end{tabular}
% \caption{Quantitative results for the racing game}
% \label{tab: orca_same_players}
% \end{table}

% In Table \ref{tab: orca_same_players} we can clearly see that \cpg learned a policy that is both faster and more precise, as well as more interactive with about six times as many overtaking maneuvers. Thus, it is not surprising that in the 5000 race between \gda vs \cpg, \gda was only able to win 103 times. For the \gda vs \cpg races, we also noted that the \gda player got ``confused" by the interactive \cpg player which resulted in crashes of the \gda player, since the \gda player never experience such interactions in training. 

==> extra/5.7-trcpo_algorithm.tex <==
\begin{algorithm}[ht]
\label{alg: trcpo}
\SetAlgoLined
\textbf{Input:} Randomly initialise $\pi(\theta^1)$, $\pi(\theta^1)$ and $V_{\phi}(s)$. The environment and training parameters num\_episode (N), num\_batches (B), $D_{KL}^{max}$ $\delta$. \\ 
\For{$episode=1$ {\bfseries to} $N$}{
 \For{$batch=1$ {\bfseries to} $B$}{
  \For{$l=1$ {\bfseries to} $trajectory\,length$}{
  Sample actions $a^1 \sim \pi(a^1|s;\theta_1)$ and $a^2 \sim \pi(a^2|s;\theta_2)$, Execute actions $a = (a^1,a^2)$ at state $s$ in the environment. Record the tuple of state, action, reward and done
  }
  }
  \textbf{1)} Compute return y(\textit{s}) and advantage estimates $A(s,a^1,a^2;\theta^1,\theta^2)$ for each monte carlo trajectory ($\tau$).\\
  \textbf{2)} Update critic by minimising the loss  $\mathcal{L(\phi)} = \sum_{s}^{|\tau|}(V_{\phi}(s) - y(s))^2$\\ 
  \textbf{3)} Estimate gradient of the surrogate game objective wrt to each agent $i$, 
 \begin{align*}
    D_{\theta_{k+1}^1} G_{\theta_k^1,\theta_k^2}(\theta_{k+1}^1,\theta_{k+1}^2) = E_{\tau \sim (\pi(\theta_k^1),\pi(\theta_k^2))} \Bigl[ \frac{D_{\theta_{k+1}^1}\pi(a^1|s;\theta_{k+1}^1)\pi^2(a^2|s;\theta_{k+1}^2)}{\pi(a^1|s;\theta_k^1)\pi^2(a^2|s;\theta_k^2)}A(s,a^1,a^2;\theta_k^1,\theta_k^2) \Bigr] 
\end{align*}\\
  \textbf{4)} Estimate bilinear derivative of the game objective,
 \begin{align*}
    D^2_{\theta^1\theta^2} G^1_{\theta_k^1,\theta_k^2}(\theta_{k+1}^1,\theta_{k+1}^2) &= E_{\tau \sim (\pi(\theta_k^1),\pi(\theta_k^2))} \Bigl[ \frac{D_{\theta^1}\pi(a^1|s;\theta_{k+1}^1)D_{\theta^2}\pi^2(a^2|s;\theta_{k+1}^2)}{\pi(a^1|s;\theta^1)\pi^2(a^2|s;\theta^2)}A(s,a^1,a^2;\theta^1,\theta^2) \Bigr] 
\end{align*}\\
 \textbf{5)} Update policy parameters for each agent with $\theta = [\theta^{1^T}, \theta^{2^T}]^T$, and some parameter $\lambda$, \\
 \While{$\theta^TA\theta<\delta$}{
 $\lambda \xleftarrow{} 2 \lambda$
  \begin{gather*}
 \ A_{ij} = D^2_{\theta^i,\theta^j}\Bigl[D_{KL}( (\theta_k^1,\theta_k^2),(\theta_{k+1}^1,\theta_{k+1}^2))\Bigr], 
B = \begin{bmatrix}
0 & D^2_{\theta^1\theta^2}G^1\\
 D^2_{\theta^2 \theta^1}G^2 & 0\\
\end{bmatrix},
C =  \begin{bmatrix}
 D_{\theta^1}G^1\\
 D_{\theta^2}G^2
\end{bmatrix} \\
\theta = -(B + \lambda A)^{-1}C
 \end{gather*}
 }
 $\theta_{k+1} = \theta_{k} + \theta$
}
\caption{Trust Region Competitive Policy Optimisation}
\end{algorithm}

==> extra/6-trcpo_experiments.tex <==
In this section we describe an empirical study for \trcpo algorithm on the same platform as used in \sect~\ref{sec:cpg_experiments}. The TRCPO code link and experiment videos are available here.\footnote{https://github.com/manish-pra/trcpo} We compared \trcpo with \trpogda, where 2 agents trained with \TRPO in \gda fashion. Empirically, the contrast between \trcpo vs \trpogda similar to that of \cpg vs \gda. \trcpo converges to the unique Nash equilibrium where as \trpogda based algorithm diverges in the bi-linear, MP, and RPS game. Experiment details and results are in \appx~\ref{appx: TRCPOgameNash}. Also we compared \trcpo with \cpg, \trcpo converges significantly faster as compared with \cpg in all environment setup. 

Similar to \sect~\ref{fig: TRCPOMarkovScoccer}, \trcpo was competed with \trpogda in the game of soccer. \fig~\ref{fig: TRCPOMarkovScoccer} shows interaction plots.
It is clear that the \trcpo agent learned much better strategies of seizing ball from opponent and scoring goal, whereas \trpogda could hardly take the ball from \trcpo.
Also note that \trpogda renders unequal players, due to which player 1 gets ball quite often which corresponds to high bar corresponding to x = 3 in \fig~\ref{Fig: trpo_trpo_gmres_interaction_plot}.
Further we compared \gdapg, \cpg, \trpogda, and \trcpo in soccer game playing against each other.
\trcpo performs best,\cpg was runner up, then \trpogda, and lastly \gda, as shown in the \fig~\ref{fig: CompMarkovScoccer}.
Further details are in \appx~\ref{appxsec: TRCPOsoccer}

\begin{figure}[h!]
\hspace{-3.00mm}
	\centering
    \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/trcpo_trcpo_gmres_interaction_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: trcpo_trcpo_gmres_interaction_plot}
    \end{subfigure}
    \hspace{-4.00mm}
    ~
    \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/trpo_trcpo_gmres_interaction_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: trpo_trcpo_gmres_interaction_plot}
    \end{subfigure}
    \hspace{-4.00mm}
    ~
    \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/trpo_trpo_gmres_interaction_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: trpo_trpo_gmres_interaction_plot}
    \end{subfigure}
    \hspace{-4.00mm}
~
  \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/trpo_trcpo_winning_plot.pdf}  
    \caption{}
    \label{Fig: trpo_trcpo_winning_plot}
  \end{subfigure}
  \hspace{-4.00mm}
%  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
%   \setlength{\abovecaptionskip}{-13pt}
%   \setlength{\belowcaptionskip}{-10pt}
  \caption{a) \trcpo vs \trcpo, b) \trpogda vs \trcpo, c) \trpogda vs \trpogda. a,b,c are interaction plots.  X-axis convention, 1: A scored goal, 2: B scores goal, 3: A scored goal after seizing ball from B. 4: B scores goal after seizing ball from A, 5: A scored goal by seizing ball from B which took the ball from A and so forth. 0: No one scores goal both kept on seizing from each other for 1000 steps.}
  \label{fig: TRCPOMarkovScoccer}
\end{figure}


\begin{figure}[ht]
\hspace{-3.00mm}
	\centering
    \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/EX_sgd_trpo_winning_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: EX_sgd_trpo_winning_plot}
    \end{subfigure}
    \hspace{-4.00mm}
    ~
    \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/EX_trpo_cpg_winning_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: EX_trpo_cpg_winning_plot}
    \end{subfigure}
    \hspace{-4.00mm}
    ~
    \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/EX_cpg_trcpo_winning_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: EX_cpg_trcpo_winning_plot}
    \end{subfigure}
    \hspace{-4.00mm}
~
  \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/EX_sgd_trcpo_winning_plot.pdf}
    \caption{}
    \label{Fig: EX_sgd_trcpo_winning_plot}
  \end{subfigure}
  \hspace{-4.00mm}
%  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
%   \setlength{\abovecaptionskip}{-13pt}
%   \setlength{\belowcaptionskip}{-10pt}
  \caption{The games are player between a)\gda vs \trpogda b) \trpogda vs \cpg ,c) \cpg vs \trcpo and d) \gda vs \trcpo}
  \label{fig: CompMarkovScoccer}
\end{figure}


Next we compared \trcpo and \trpogda performance on the car racing game similar to ~\sect~\ref{sec: CPG_ORCA}. During training, we observed that \trpogda faces oscillation while training i.e. when an agent maximizes his progress, the other agent performance shrink to low progress due to zero-sum formulation. Also, a few times, one agent collapses near-zero progress, and the other agent learns to drive in this stationary environment as shown in the \fig~\ref{fig: ProgressOrca}. Due to this \trpogda trained agents had hard time to reach the goal together, presumably because of unexplored state space. Where as in the case of \trcpo, as shown in ~\fig ~\ref{fig: progress_plot_orca_trcpo} we observe that both agents are trained together to maximize their progress.  On competing with \trcpo with \trpogda, \trcpo wins almost all the matches due to better interactive strategies learned by \trcpo agent. Further comparisons and implementation details are in ~\sect~\ref{appxsec: TRCPOorca}. 

\begin{figure}[h!]
	\centering
    \begin{subfigure}[t]{0.31\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/trpo2gda_crash.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: trpo2gda_crash}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.31\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/trpo2gda_oscillations.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: trpo2gda_oscillations}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.31\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/progress_plot_orca_trcpo.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: progress_plot_orca_trcpo}
    \end{subfigure}
% ~
%   \begin{subfigure}[t]{0.48\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/EX_sgd_trcpo_winning_plot.pdf}
%     \caption{}
%     \label{Fig: bilinear}
%   \end{subfigure}
% %  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
% %   \setlength{\abovecaptionskip}{-13pt}
% %   \setlength{\belowcaptionskip}{-10pt}
  \caption{Progress of agents while training a) \trpogda $\delta=1e-5$ b) \trpogda $\delta=1e-4$ c) \trcpo $\delta=1e-4$}
  \label{fig: ProgressOrca}
\end{figure}

==> extra/Old2-preliminaries-withR.tex <==
A two player \CMDP is a tuple of $<\S,\A^1,\A^2,\R^1,\R^2,\T,\mathcal{P},\gamma>$, where $\S$ is the state space, $s \in \S$ is a state, for player $i\in\lbrace 1,2\rbrace$, $\A^i$ is the player $i$'s action spaces with $a^i\in\A^i$ that player's action. $\R^i$ is the reward kernels with mean reward function $r^i: \S\times \A^1 \times \A^2 \rightarrow \mathbb{R}$. For a probability measure $\mathcal{P}$ of initial state, $p$ denotes the probability distribution of initial state, and for the transition kernel $\T$, $T(s'|s,a^1,a^2)$ represents the distribution of successive state $s'$ after taking actions  $a^1,a^2$ simultaneously at state $s$, and finally $\gamma \in [0,1]$ is the discount factor. We consider episodic environments where there exists an absorbing state $\stermination$, such that with probability one (almost surely), the episode terminates at $\stermination$ in finite time. After termination of an episode, the environment resets to a new initial state drawn from $p$. At each time step $k\geq 0$ and state $s_k$, each player $i$ draws its action $a_{k}^i$ according to $\pi(a_{k}^i|s_k;\theta^i)$ distribution, where the policy  $\pi(\theta^i)$   is parameterized by $\theta^i\in \Theta^i$ and $\Theta^i\subset\mathbb{R}^{l}$ is a compact metric space. Each player $i$, receives its reward $r^i_{k}$, and the environment evolves to a new state $s_{k+1}$ at time step $k+1$. A realization of this stochastic process is a trajectory $\tau = \big( (s_j,a^1_{j},a^2_{j},r^1_{j},r^2_{j})_{j=0}^{|\tau|-1} ,s_{|\tau|}\big)$, an ordered sequence 
% $\tau = \lbrace s_0,a^1_{0},a^2_{0},r^1_{0},r^2_{1},s_1,a^1_{1},a^2_{1},r^1_{1},r^2_{1},\ldots, s_{|\tau|-1},a^1_{|\tau|-1},a^2_{|\tau|-1},r^1_{|\tau|-1},r^2_{|\tau|-1},s_{|\tau|}\rbrace$ 
with random length $|\tau|$, where $|\tau|$ is determined by episode termination time and state $s_{|\tau|}=\stermination$. Let $f(\tau;\theta^1,\theta^2)$ denote the probability distribution of trajectory $\tau$ following players policies $\pi(\cdot|\cdot\,;\theta^i)$, 
\begin{align*} \label{eq: trajectory_distribution}
f(\tau; \theta^1, \theta^2)= p(s_0) \prod_{k=0}^{|\tau|-1} \pi(a^1_{k}|s_k;\theta^1) \pi(a^2_{k}|s_k;\theta^2) T(s_{k+1}|s_k,a^1_{k},a^2_{k}). \numberthis
\end{align*}
% For each agent $i\in\lbrace 1,2\rbrace$, given the player's policy $\pi(\cdot|\cdot\,;\theta^i)$, the state-value (V) and state-action-value (Q) functions are as follows, $\forall s\in\S,a^i\in\A^i$,
For each agent $i\in\lbrace 1,2\rbrace$ with policy $\pi(\theta^i)$, $\forall s\in\S,a^i\in\A^i$ the the state-value (V) and state-action-value (Q) functions are as follows, 
\begin{align}\label{eqn: val_rew}
    V^i(s_k;\theta^1, \theta^2) &= \mathbb{E}_{\tau\sim f(\cdot; \theta^1, \theta^2)} \Big[ \sum\nolimits_{j=k}^{|\tau|-1} \gamma^{j-k} r^i(s_j,a^1_{j},a^2_{j})| s_k\, \Big],\nonumber \\
    Q^i(s_k,a^1_{k},a^2_{k};\theta^1, \theta^2) &= \mathbb{E}_{\tau\sim f(\cdot; \theta^1, \theta^2)} \Big[ \sum\nolimits_{j=k}^{|\tau|-1} \gamma^{j-k} r^i(s_j,a^1_{j},a^2_{j})| s_k, a^1_k, a^2_k \Big],
\end{align}
% where $V^i(s_k;\theta^1, \theta^2)$ denotes the expected return the $i$'th player receives starting from state $s_k$ at time step $k$, and players follow $\pi(\theta^1)$, $\pi(\theta^2)$ policies then on. Similarly, $Q^i(s_k,a^1_{k},a^2_{k};\theta^1, \theta^2)$ denote the analogous value when for the $k$'th time steps, players play actions $a^1_{k}$ and $a^2_{k}$.
and consequently, the $i$'th player's expected return $\eta^i (\theta^1,\theta^2) = \int_{s_{0}} p(s_{0})  V^i(s_0;\theta^1, \theta^2) ds_{0}$.
% \begin{align}\label{eq: eta_game}
% \eta^i (\theta^1,\theta^2) = \int_{s_{0}} p(s_{0})  V^i(s_0;\theta^1, \theta^2) ds_{0}.
% \end{align}
In zero-sum games, $r(s,a^1,a^2) := r^1(s,a^1,a^2) = -r^2(s,a^1,a^2)$, and $\eta$, the value/objective of the game, given the policies is  
$\eta (\theta^1,\theta^2):= \int_{\tau} f(\tau;\theta^1,\theta^2) R(\tau) d\tau$ with $R(\tau) = \sum_{k=0}^{|\tau|}\gamma^kr(s_k,a^1_k,a^2_k)$. We consider the case where $V$, $Q$, and $\eta$ are differentiable in $\Theta^1$ and $\Theta^2$, and therefore continuous. For any function $f$, defined on $\Theta^1$ and $\Theta^2$, for simplicity, we adopt $D_{\theta^i}f= \frac{\partial f({\theta'}^1,{\theta'}^2)}{\partial {\theta'}^i}\big|_{({\theta'}^1,{\theta'}^2)=({\theta}^1,{\theta}^2)}$ and $D_{\theta^i\theta^j} f = \frac{\partial}{\partial {\theta'}^i} \big( \frac{\partial f({\theta'}^1,{\theta'}^2)}{\partial {\theta'}^j} \big)\big|_{({\theta'}^1,{\theta'}^2)=({\theta}^1,{\theta}^2)}$ for $i,j\in\lbrace 1,2\rbrace$.

% $D_{\theta^2\theta^1} f = \frac{\partial}{\partial {\theta'}^2} \biggl( \frac{\partial f({\theta'}^1,{\theta'}^2)}{\partial {\theta'}^1} \biggr)\Big|_{({\theta'}^1,{\theta'}^2)=({\theta}^1,{\theta}^2)}$. 



% $D_{\theta^i}f({\theta}^1,{\theta}^2)= \frac{\partial f({\theta'}^1,{\theta'}^2)}{\partial {\theta'}^i}\Big|_{({\theta'}^1,{\theta'}^2)=({\theta}^1,{\theta}^2)}$ and $D_{\theta^2\theta^1} f({\theta}^1,{\theta}^2) = \frac{\partial}{\partial {\theta'}^2} \biggl( \frac{\partial f({\theta'}^1,{\theta'}^2)}{\partial {\theta'}^1} \biggr)\Big|_{({\theta'}^1,{\theta'}^2)=({\theta}^1,{\theta}^2)}$. 

==> extra/Old4.6-cpg_experiment.tex <==
\kamyar{Manish, at some point add a discussion on self play, and explain in symmetric game one can do deploy \cpo in self-play setting. Also run it on soccer game and study it in term of performance, and sensitivity. }

In this section we present an empirical study of \cpg algorithm on seven games which are linear quadratic(LQ) game, bilinear game, linear bilinear game, rock paper scissors (RPS), matching pennies (MP), Markov soccer and the game of car racing. The set covers discrete as well as continuous state action games and is a mix of both single-shot stateless and finite horizon games. Players are simultaneously trained under self play using \cpg or \gda. For evaluation purposes, we compared convergence behavior of \cpg with \gda and finally competed \cpg trained policies face to face with that of \gda in the game of Markov soccer and car racing. The \gda agents are trained with stochastic gradient descent. The optimizer for \cpg
% is built upon \cgd optimizer, \cite{schfer2019implicit}.  
is built using Pytorch's autograd package for evaluating gradient and bilinear terms. The \cpg formulation requires to evaluate bilinear term which can be efficiently computed with minimal overhead using hessian vector product trick $D_{\theta^i \theta^j} \eta \ v = \frac{\partial}{\theta^i} \big( (\frac{\partial}{\theta^j} \eta) v\big) $ instead of computing 2D matrices for the bilinear term. Moreover inorder to evaluate the inverse term in \eq~\ref{eqn: CGDSolution}, we utilised conjugate gradient to approximate inverse matrix vector product. (see \citet{schfer2019competitive} for more details). The link of the code and experiment videos is available in the footnote.\footnote{https://github.com/manish-pra/Competitive-Policy-Gradient}. Experiments presented here are in zero sum game formulation but the optimizer for general sum is also available in the same repository. Further we evaluated performance of \cpg with \maddpg which is documented in \appx~\ref{appx: maddpg_comp}.

Empirically, we see that \cpg converges to a stable point whereas \gda based algorithms diverge in the bi-linear, MP, and RPS game. Unlike \gda, where each player foolishly maximizes his reward which often leads to diverging behavior, \cpg is able to learn an opponent aware strategy. For highly strategic games, where the policy of players are tightly coupled, \cpg was able to learn much better interactive strategy, for eg, in the game of  soccer \cpg players learn to defend, dodge and score goal as compared to its counter part \gda learns to lamely score a goal if he has the ball, otherwise give way to the other player. Also, in the game of racing between 2 cars, \cpg produces competing players who learn to block and fake each other. Overall, We observe \cpg considerably outperforms, in terms of convergence, learnt strategies, and gradient dynamics. 
\manish{Shall keep this para here or at the end of experimentes or conclusion? I want to write a brief para summarising all experiments, because going though each experiment everytime is tedious for reader}

\subsubsection{Games with known Nash Equilibrium}
Here we consider the empirical study on the games with known Nash equilibrium, in order to study convergence behaviour. Firstly, we considered a \textbf{zero sum LQ game} defined by \eq~\ref{eqn: lq_game} which is studied theoretically and have convergence guarantees ~\citep{zhang2019policyZerosum}. This makes LQ game an ideal platform to compare range of allowable step sizes and convergence rate of \cpg with \gda.
% In a LQ game, state and action spaces are continuous, state is propagated using linear dynamics and the cost is quadratic.
\begin{gather} \label{eqn: lq_game}
    J(K^1,K^2) = \max\nolimits_{K^1} \min\nolimits_{K^2} \mathbb{E}\big[  \sum\nolimits_{k=0}^{\infty} \gamma^k \bigl({s_k}^T Q s_k + {a^1_k}^T R_{11} a^1_k   + \ {a^2_k}^T R_{22} a^2_k \bigr)\big]  \\
    \text{where:} \ s_{k+1} = As_k + B_{1}a^1_k + B_{2}a^2_k,~\textit{and} \ \  a^1_{k+1} = -K^1s_k, \ a^2_{k+1} = -K^2s_k \nonumber
\end{gather}

In the LQ game (defined further in \appx~\ref{appxsec: LQgame}), we observed that with the initially collected samples \gda estimated large gradients, along with high learning rate it resulted in large steps. The resulting policy then generated erratic trajectories in the next rollout, which caused instability and thus \gda did not converge (we denoted this runs with a $\oslash$ in \appx \tab~\ref{tab: LQgameLR}). \cpg is robust towards this behavior and can potentially take even larger steps. \fig~\ref{fig: LQlr_1e2} shows the advantage estimates $\sum_{\tau} f(\tau;\theta^1,\theta^2) \sum_{k=0}^{|\tau|-1}A(s_k,a_{k}^1,a_{k}^2;\theta^1,\theta^2)$ of \gda and \cpg for different learning rates. We can see that \cpg dynamics are not just faster at the same learning rate but more importantly, \cpg allows having larger learning rates.
% as shown in \fig~\ref{fig: LQlr_1e2}.
Experiment details and results are documented in \appx~\ref{appxsec: LQgame}. 
\begin{figure}[h]
	\hspace{-3.00mm}
	\centering
    \begin{subfigure}[t]{0.27\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/combine_matching_pennies.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: combine_matching_pennies}
    \end{subfigure}
    \hspace{-6.00mm}
~
    \begin{subfigure}[t]{0.27\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/combined_rps.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: combined_rps}
    \end{subfigure}
    \hspace{-6.00mm}
   ~
    \begin{subfigure}[t]{0.27\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/combined_bilinear_mat.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: combined_bilinear_mat}
    \end{subfigure}
    \hspace{-6.00mm}
~
  \begin{subfigure}[t]{0.27\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/LQlr_1e2.pdf}  
    \caption{}
    \label{fig: LQlr_1e2}
  \end{subfigure}
  \hspace{-4.00mm}
%  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
%   \setlength{\abovecaptionskip}{-13pt}
%   \setlength{\belowcaptionskip}{-10pt}
  \caption{\cpg (C) vs \gda (G) behaviour on a) Matching Pennies, Head(H) Tail(T)b) Rock(R) Paper(P) Scissors(S) c) Bilinear Game d) LQ game}
  \hspace{-4.00mm}
\end{figure}
Next we considered a single shot \textbf{bilinear game}, where players exhibit a strong non cooperative behavior. \gda is known to diverge in the bilinear game and hence, it is widely studied to propose other gradient based optimizers ~\citep{BalduzziHamiltonian}.
In a bilinear game both players act simultaneously and receive a rewards based on product of their actions, $r(a^1,a^2) = {a^1}^\top a^2$ where $a^1\sim\mathcal{N}(\mu_1,\sigma_1)$ and $a^2\sim\mathcal{N}(\mu_2,\sigma_2)$.
% Players aim to learn optimal policies $(\mu_1,\mu_2)$.
In the bilinear game, \gda diverges for all learning rates, whereas \cpg converges to the Nash equilibrium of the game as shown in the \fig~\ref{fig: combined_bilinear_mat}.
% shows this behavior for a learning rate of 0.1.

Next we considered Matrix games, particularly \textbf{Matching pennies} and \textbf{Rock paper scissors}. The games are challenging and require an opponent aware optimization. The unique Nash equilibrium of these games is a mixed strategy. Traditionally, the games are approached with fictitious play, counterfactual regret methods ~\citep{CFR_RPS}.
% The game matrices are shown in the \tab~\ref{tab: rock_paper_scissors} , \ref{tab: matching_pennies}. 
\cpg converges to the unique Nash equilibrium of the MP \fig~\ref{fig: combine_matching_pennies} and RPS \fig~\ref{fig: combined_rps}, whereas \gda moves away from the Nash equilibrium for all learning rates. \gda actually approaches near deterministic strategies that are easily exploitable by other deterministic strategies leading to unstable learning. In contrast, \cpg agents learn to play the unique mixed Nash strategy, where players anticipate that exploiting a deviation from the Nash equilibrium increases their immediate return, but also renders them to be more exploitable by the opponent. More details and results are documented in \appx~\ref{appxsec: CPGMP} and \appx~\ref{appxsec: CPGRPS}.

% \begin{table}[ht]
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{|c||c|c|c|}
% \hline
%  & Rock & Paper & Scissors  \\
%  \hline \hline
%  Rock & 0,0 & -1,1 & 1,-1   \\
%  \hline
%  Paper & 1,-1 & 0,0 & -1,1   \\
%  \hline
%  Scissors & -1,1 & 1,-1 & 0,0   \\
% \hline
% \end{tabular}
% \caption{Game matrix for rock paper scissors}
% \label{tab: rock_paper_scissors}
% }
% \hfill
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{|c||c|c|}
% \hline
%  & Head & Tail  \\
%  \hline \hline
%  Head & 1,-1 & -1,1   \\
%  \hline
%  Tail & -1,1 & 1,-1   \\
% \hline
% \end{tabular}
% \caption{Game matrix for matching pennies}
% \label{tab: matching_pennies}
% }
% \end{table}


\subsubsection{Markov Soccer}
\label{sec: CPGMarkovSoccer}
The Markov soccer used here is similar to the one defined in ~\citet{littmansoccer} ~\citet{HeHeOppo}. Although both \gda and \cpg converge in this game, it is a strategic game where a smart agent learns sophisticated strategies of defending, dodging and scoring. The Markov soccer game is shown in \fig~\ref{fig: Soccer}. It is played between 2 players, where agents are supposed to pick up the ball and put in the opponents' goal. The winner receives a +1 reward and -1 is awarded to the losing player. The game and training is described in detail in \appx~\ref{appxsec: soccer}. For a comparison between \cpg and \gda, we played 10000 games between them, where in 50\% of the games, \cpg was player A and for the remaining \gda was player A. \cpg won more than 74\% of all games against \gda as shown in \fig~\ref{Fig: sgd_cpg_winning_plot}. 
In order to capture interaction between players, we recorded the number of times the ball is seized between the players before one player finally scores a goal. \fig~\ref{Fig: InteractionBilinear}[a,b,c], show interaction plots (description in the caption). In, \cpg vs \cpg game we see twice more probability of seizing ball as compared to \gda vs \gda (see x=3, x=4 in \fig~\ref{Fig: cpg_cpg_interaction_plot} vs \fig~\ref{Fig: sgd_sgd_interaction_plot}). Also in the match between \cpg vs \gda, \cpg agent could take balls 50\% of the time from \gda agent but \gda can hardly take ball back from \cpg. \cpg was able to learn better tactics for seizing and dodging the ball, as well as defending its goal post. 

\begin{figure}[h]
\hspace{-4.00mm}
	\centering
    \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/cpg_cpg_interaction_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: cpg_cpg_interaction_plot}
    \end{subfigure}
    \hspace{-5.00mm}
   ~
    \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/sgd_sgd_interaction_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: sgd_sgd_interaction_plot}
    \end{subfigure}
    \hspace{-5.00mm}
    ~
    \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/cpg_sgd_interaction_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: cpg_sgd_interaction_plot}
    \end{subfigure}
    \hspace{-5.00mm}
~
  \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/sgd_cpg_winning_plot.pdf}  
    \caption{}
    \label{Fig: sgd_cpg_winning_plot}
  \end{subfigure}
  \hspace{-4.00mm}
%  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
%   \setlength{\abovecaptionskip}{-13pt}
%   \setlength{\belowcaptionskip}{-10pt}
  \caption{a) \cpg vs \cpg, b) \gda vs \gda, c) \cpg vs \gda. a,b,c are interaction plots.  X-axis convention, 1: A scored goal, 2: B scores goal, 3: A scored goal after seizing ball from B. 4: B scores goal after seizing ball from A, 5: A scored goal by seizing ball from B which took the ball from A and so forth. 0: No one scores goal both kept on seizing from each other for 1000 steps.
%   Similarly, Ceil[x/2] denotes the number of times ball has been seized from each other before scored by player A (x=odd) or player B (x=even), where x is the x-axis index
  d) Shows probability of games won when \cpg competed against \gda}
  \label{Fig: InteractionBilinear}
\end{figure}

\begin{figure}[h]
{
    \begin{subfigure}[t]{0.40\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/Soccer.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
\vspace{-6.00mm}
    \caption{}
    \label{fig: Soccer}
    \end{subfigure}
    \hspace{-10.00mm}
    
\vspace{-45.00mm}
    
   	\hspace{-5.00mm}
    \begin{subfigure}[t]{0.25\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/orca_sgd.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: orca_sgd}
    \end{subfigure}
    \hspace{-6.00mm}
~
  \begin{subfigure}[t]{0.25\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/orca_cpg_progress_plot.pdf}  
    \caption{}
    \label{fig: orca_cpg_progress_plot}
  \end{subfigure}
  \hspace{-6.00mm}
}
    ~
    \begin{subfigure}[t]{0.65\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/overtaking_manuever_northsouth.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: overtaking_manuever_northsouth}
    \end{subfigure}
    \hspace{-12.00mm}
    
    \caption[Caption for LOF]
    {a) The Markov Soccer Game, b \& c) Progress of agents while training b) \gda c) \cpg progress = 1 is end of the track d) Overtaking maneuvers\footnotemark of \cpg agents in the Car Racing Game. The thick line shows trajectory when the loosing agent overtook.}
    \label{Fig: orca}
  \hspace{-4.00mm}
  \vspace{-5.00mm}
\end{figure}
\footnotetext{Video is available here}
% \vspace{-10.00mm}
\subsubsection{ORCA Racing}
\label{sec: CPG_ORCA}
Our final experimental setup is a racing game between two race cars, where the goal is to finish the race first. The game involves both, learning a policy that can control a car at the limit of handling, as well as strategic interactions with the opposing car. The test track which consists of 13 turns with different curvature can be seen in \fig~\ref{Fig: orca}. The game is formulated as a zero-sum, with reward $r(s_k,a^1_{k},a^2_{k}) = \Delta \rho_{car_1} - \Delta \rho_{car_2}$, where $\Delta \rho = \rho_{k+1} - \rho_k$ and $\rho_k$ is a progress of the car till $k^{th}$ time step in the track. If a car crosses track boundaries, then it is freezed i.e ($\Delta \rho = 0$), which results in its penalization using the above reward formulation corresponding to the $(\Delta \rho)$ of the other agent. Similarly during a collision, the rear car is freezed, which penalizes it and the car in the front receives positive rewards. This formulation promotes blocking by the car in front, overtaking by the car in the rear.  
% Here we explain reward shaping to give intuition behind the competition involved. To formulate the racing game between two cars, we convert the objective of finishing the race first without an accident into a zero sum game. First to model our no accident constraints we use a freezing mechanism:
% % (where one car is frozen and other is allowed to ear rewards): 
% (i) If the car is leaving the track we freeze it until the episode ends, 
% (ii) If the cars collide, the rear car is stopped for 1s. Note that this gives an advantage to the car ahead, but in car racing, the following car has to avoid collisions. 
% (iii) The car which finishes first gets a +1 reward and the other car gets -1 reward. Furthermore, an episode ends if both cars are either frozen due to leaving the track or the first car finished the lap. 
% (iv) Finally, to reward racing the players at every time step receive the following reward $r(s_k,a^1_{k+1},a^2_{k+1}) = \Delta \rho_{car_1} - \Delta \rho_{car_2}$, where $\Delta \rho = \rho_{k+1} - \rho_k$. $\rho$ is a progress of the car at $k^{th}$ time step in the track. This reward encourages the player to get as far ahead of the opponent player as possible. 

We trained the racing game with both \gda and \cpg, even though both players were able to learn to "drive" only \cpg was able to learn how to ``race". With \gda, only one player was able to learn, this either manifested in one player completely failing and the other finishing the race, or by an oscillation behavior where when one agent learns to go ahead, the other agent learns to stay at lower progress. Even if at some point one of the players learns to finish one lap, the player does not learn to interact with the other opponent. The players trained with \cpg on the other hand, both progress and learn to finish the lap and to interact with each other. See \fig~\ref{fig: orca_cpg_progress_plot} and \fig~\ref{fig: orca_sgd}, where the progress the two players during training can be seen for \gda and \cpg, it is clearly visible that with \cpg both players get better over time, whereas in \gda the two player have an oscillation behavior, and at the end, only one of the two players finishes the lap. 

% To test the policies, we run 5000 episodes with the obtained policy. To evaluate the performance we run three types of races, \gda vs \gda, \cpg vs \cpg, \gda vs \cpg. For each episode, we counted the number of overtakes, the number of collisions with the track constraints, and recorded the lap time. For the \gda vs \cpg test we also counted the number of times which policy won, where we defined winning as finishing first. Since, \gda often collided with the track constraints, for the test, we replaced the freezing with a reset at the reference path routine. 

To test the policies, we performed 10000 races between \cpg and \gda, with \cpg as player 1 in half of them. The \tab~\ref{tab: orca_diff_players} shows the normalised score. we can clearly see that \cpg learned a policy that is both faster and more precise. Although \gda was able to overtake, almost all of it's overtaking maneuvers leads to crash with the track boundaries. 

\begin{table}[ht]
\centering 
\begin{tabular}{|c||c|c|c|c|}
\hline
 & \multicolumn{2}{c|}{CPG vs GDA} &  \multicolumn{2}{c|}{GDA vs CPG} \\
 \hline \hline
%  \cline{2-5}
 Wins & 1 & 0 & 0 & 1  \\
 \hline
 Overtaking  & 1.68 & 1.01 & 1.04 & 1.65  \\
 \hline
 Collosions & 0.28 & 1.33 & 1.46 &  0.23  \\
 \hline 
\end{tabular}
\caption{Comparative results for \cpg vs \gda on the ORCA setup}
\label{tab: orca_diff_players}
\end{table}

% \begin{table}[ht]
% \centering 
% \begin{tabular}{|c||c|c|c|}
% \hline
%  & \cpg vs \cpg & \gda vs \gda \\
%  \hline \hline
%  Overtaking per lap & 3.35 & 0.68  \\
%  \hline
%  Track collision per lap & 0.59 & 1.12  \\
%  \hline
%  Laptime  & 10.89 & 13.32  \\
%  \hline
% \end{tabular}
% \caption{Quantitative results for the racing game}
% \label{tab: orca_same_players}
% \end{table}

% In Table \ref{tab: orca_same_players} we can clearly see that \cpg learned a policy that is both faster and more precise, as well as more interactive with about six times as many overtaking maneuvers. Thus, it is not surprising that in the 5000 race between \gda vs \cpg, \gda was only able to win 103 times. For the \gda vs \cpg races, we also noted that the \gda player got ``confused" by the interactive \cpg player which resulted in crashes of the \gda player, since the \gda player never experience such interactions in training. 

==> extra/appx2.5-cpg_experiments.tex <==
\section{Experiment details}
% \kamyar{Manish, at some point add a discussion on self play, and explain in symmetric game one can do deploy \cpo in self-play setting. Also run it on soccer game and study it in term of performance, and sensitivity.}


We implemented all algorithms on Pytorch platform~\citep{NEURIPS2019_9015}, and made the code and the videos public %\footnote{https://github.com/manish-pra/Competitive-Policy-Gradient}
% \footnote{https://github.com/manish-pra/trcpo}
. In our \gda/\cgd implementation, we deploy Pytorch's autograd package as well as Hessian vector product approach to efficiently compute the gradients and Hessian vector product to compute the bilinear terms in the optimizer.  Moreover, we use conjugate gradient trick to efficiently computed the inverses in \eq\ref{eqn: CGDSolution} which incurs a minimal computational overhead (see \citep{CG_Jonathan1994} for more details). Also we computed inverse matrix vector product only for one player strategy let say $\Delta \theta^1$, and use optimal counter strategy for other player $\Delta \theta^2$ which can be computed without inverse matrix vector product. Also, the last optimal strategy can be used for warm start of conjugate gradient which ease in convergence. 

\subsection{Games with known closed-form Nash Equilibrium}
\label{appxsec: NashGame}
\subsubsection{Linear Quadratic (LQ) Game} 
\label{appxsec: LQgame}
The zero sum LQ game is defined by: 
\begin{gather} \label{appxeqn: lq_game}
    J(K^1,K^2) = \max_{K^1} \min_{K^2} \mathbb{E} \biggl[ \sum_{k=0}^{|\tau|} \gamma^k \bigl({s_k}^T Q s_k + {a^1_k}^T R_{11} a^1_k   + \ {a^2_k}^T R_{22} a^2_k \bigr) \biggr] \\
    \text{where:} \ s_{k+1} = As_k + B_{1}a^1_k + B_{2}a^2_k 
     \qquad \qquad a^1_{k+1} = -K^1s_k, \ a^2_{k+1} = -K^2s_k \nonumber
\end{gather}
where, $s_k \in R^n$ is system state vector, $a^1 \in R^{d_1}$ and $a^2 \in R^{d_2}$ are control inputs by player 1 and 2 respectively. The matrix $A \in R^{n\times n}$, $B_1 \in R^{n \times d_1}$ and $ B_1 \in R^{n \times d_2}$ describe the system dynamics. Here, $K^1$ and $K^2$ denotes the controller policies. We considered a simple game where, $A = 0.9,\ B_1 = 0.8,\ B_2 = 1.5,\ R_{11} = 1,\ R_{22} = 1$. These environment parameters are not known to the players. Policy of each player is linear in state and actions are sampled from Gaussian distribution $a^1\sim\mathcal{N}(\mu^1,\sigma^1)$, $a^2\sim\mathcal{N}(\mu^2,\sigma^2)$, where initial value $\mu^1_0 = 0.1$ and $\mu^2_0=-0.1$ and $\log(\sigma^1_0)=\log(\sigma^2_0)=0.1$. The game dynamics and rewards follows \eq~\ref{appxeqn: lq_game}. We collected a batch of 1000 trajectories, each 5 time steps long. The optimal control policy $(K^{1*}, K^{2*} = -0.5735,-0.3059)$, obtained using coupled riccatti equation ~\citep{zhang2019policyZerosum}. The experiment is performed for 5 different random seeds. As per discussion in \appx~\ref{appx: advantagebilinear}, we used \GAE~for advantage estimation with $\lambda=0.95$ and $\gamma=0.99$. The number of iterations it takes to converge for different learning rates is noted in Table~\ref{tab: LQgameLR}.
 \fig~\ref{fig: AdvLQgame} shows the advantage estimates $\sum_{\tau} f(\tau;\theta^1,\theta^2) \sum_{k=0}^{|\tau|-1}A(s_k,a_{k}^1,a_{k}^2;\theta^1,\theta^2)$ of \gda and \cpg for different learning rates. 
 
  \begin{table}[ht]
\centering 
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
 learning rate & 0.1 & 0.05 & 0.01 & 0.05 & 0.001 & 0.0001\\
 \hline \hline
 \gda & $\oslash$ & $\oslash$ & 113 & 139 & 223 & 611\\
 \hline
 \cpg & 75 & 87 & 105 & 127 & 195 & 590\\
 \hline
\end{tabular}
\caption{Number of iterations to converge to optimal policies}
\label{tab: LQgameLR}
\end{table}

\begin{figure}[h]
\hspace{-4.00mm}
	\centering
    \begin{subfigure}[t]{0.25\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/LQlr_1e2.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: LQlr_1e2}
    \end{subfigure}
    \hspace{-4.00mm}
~
    \begin{subfigure}[t]{0.25\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/LQlr_5e3.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: LQlr_5e3}
    \end{subfigure}
    \hspace{-4.00mm}
   ~
    \begin{subfigure}[t]{0.25\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/LQlr_1e3.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: LQlr_1e3}
    \end{subfigure}
    \hspace{-4.00mm}
~
  \begin{subfigure}[t]{0.25\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/LQlr_1e4.pdf}  
    \caption{}
    \label{Fig: LQlr_1e4}
  \end{subfigure}
%  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
%   \setlength{\abovecaptionskip}{-13pt}
%   \setlength{\belowcaptionskip}{-10pt}
  \caption{Advantage estimates of LQ game at different learning rates}
  \label{fig: AdvLQgame}
\end{figure}

\subsubsection{Bilinear game}
\label{appxsec: CPGBilinear}
In bilinear game both players play actions simultaneously and receive rewards based on product of their actions given by \eq~\ref{eqn: BilinearReward}, where $a^1\sim\mathcal{N}(\mu_1,\sigma_1)$ and $a^2\sim\mathcal{N}(\mu_2,\sigma_2)$ are actions of player 1 and player 2 respectively. In our experiment setup, player's policy is modelled as a Gaussian distribution with  $\mu_i, \sigma_i, i\in\{1,2\}$ as mean and variance respectively. The policy is randomly initialised. We collected batch of 1000 trajectories. We performed this experiment for learning rate between 0.1 and 0.001 for 8 random seeds.  In this single shot game, we used Monte Carlo approach to get returns.
\begin{align}\label{eqn: BilinearReward}
    r^1(a^1,a^2) = a^1a^2 \;\;\;\;\;\;\;\;\; r^2(a^1,a^2) = -a^1a^2
\end{align}

\subsubsection{Matching pennies}
\label{appxsec: CPGMP}
Matching pennies game is played between two players, each player has two possible actions \{Head, Tail\}. Both the players secretly turn their coin to either head or tail. If pennies of both the players matches then player 1 wins and player 2 looses. Otherwise, if pennies do not match then player 2 wins and player 1 loses. The game matrix is given in \tab~\ref{appxtab: matching_pennies} captures win and lose of players for every possible action pair. 
\begin{table}[ht]
\centering 
\begin{tabular}{|c||c|c|}
\hline
 & H & T  \\
 \hline \hline
 H & 1,-1 & -1,1   \\
 \hline
 T & -1,1 & 1,-1   \\
\hline
\end{tabular}
\caption{Game matrix for matching pennies}
\label{appxtab: matching_pennies}
\end{table}
Player's policy is modelled with a two classes categorical distribution. Players are randomly initialised and sample actions from softmax probability function over categorical distribution. They receive rewards for their actions according to the game matrix. We collect a batch of 1000 trajectories, to estimate gradient and bilinear terms in every epoch. \cpg converges to Nash equilibrium of the game $\bigl(\frac{1}{2}, \frac{1}{2} \bigr)$.  We performed this experiment for learning rate between 0.1 and 0.001 for 8 random seeds.

\subsubsection{Rock paper scissors}
\label{appxsec: CPGRPS}
Rock paper scissors game is played between two players, each player has three possible actions \{Rock, Paper, Scissors\}. Both players will simultaneously display one of three actions: a rock, paper, or scissors. A rock beats scissors, scissors beat paper by cutting it, and paper beats rock by covering it. This is captured in the game matrix given by \tab~\ref{appxtab: rock_paper_scissors}. 

\begin{table}[ht]
\centering 
\begin{tabular}{|c||c|c|c|}
\hline
 & Rock & Paper & Scissors  \\
 \hline \hline
 Rock & 0,0 & -1,1 & 1,-1   \\
 \hline
 Paper & 1,-1 & 0,0 & -1,1   \\
 \hline
 Scissors & -1,1 & 1,-1 & 0,0   \\
\hline
\end{tabular}
\caption{Game matrix for rock paper scissors}
\label{appxtab: rock_paper_scissors}
\end{table}
Player's policy is modelled with 3 classes categorical distribution, Players are randomly initialised and sample actions from softmax probability function over categorical distribution. They receive reward for their actions according to the game matrix. We collect a batch of 1000 trajectories. \cpg converges to the unique Nash equilibrium of the game, where probability of playing $(Rock, Paper, Scissors) = (\frac{1}{3},\frac{1}{3},\frac{1}{3})$. We performed this experiment for learning rate between 0.1 and 0.001 for 8 random seeds.

\subsection{Markov Soccer Game}
\label{appxsec: soccer}
The soccer game setup \fig~\ref{fig: Soccer}, used here is similar to the one defined in ~\citet{littmansoccer} ~\citet{HeHeOppo}. The game is played between two players A and B, both are randomly initialized in one of the 4x5 grid cells. The ball is also randomly initialised in one of the 4x5 grid cells, this contrast to the previous studies, where one of the players was randomly initialised with the ball. Players are supposed to pick up the ball and place it in the opponent's goal. The players are allowed to move \textit{up, down, left, right} or stand still. The player with no ball seizes the ball, if both players move simultaneously in the same grid cell. The game ends if any player scores a goal or none of them scores within 1000 steps. The winner receives a +1 reward and -1 is awarded to the losing player, hence formulated as a zero sum game. This game does not have an optimal deterministic policy. This game depicts heavy interactions, where strategy depends on what the other player plays. Potentially, a good player can learn defending, dodging and scoring. 

The state vector of player P with respect to opponent O is $s^P = [x_{G_O},y_{G_O},x_{ball},y_{ball},x_{O},y_{O}]$, where $P, O \in \{A,B\}$. $G_O$ is goal of the opponent, $x,y$ is relative position from player. The state vector of the game used during training is $s = [s^A,s^B]$, $s \in \mathcal{R}^{12}$, it captures position of each player relative to the goal, the ball and relative to the opponent. The players' policy maps state vector of the game to a categorical distribution with 5 categories using a network with two hidden layers one with 64 and other with 32 neurons. Players sample actions from softmax probability function over the categorical distribution. The players were trained in a self play setting, where \gda and \cpg were trained against identical players. Both the players were trained for roughly 30,000 episodes until the number of wins against any good player saturates. In each epoch we collected a batch consists of 10 trajectories. A trajectory is terminated with anyone of the agent scores goal or none of them scores in 1000 steps. All the parameters were same throughout the training for \cpg and \gda. The experiment was tested with 6 different random seeds. We used \GAE~for advantage estimation with $\lambda=0.95$ and $\gamma=0.99$.  
% The final match was played between \cpg and \gdapg for 10000 games, in which for 50\% of the games \cpg was player A and for remaining \gdapg was player A. \cpg won more than 74\% games against \gdapg as shown in \fig~\ref{Fig: InteractionBilinear}. \cpg was able to learn better tactics for seizing of ball and dodging and defending it's goal post. 
% In order to capture interaction between players, we recorded number of times the ball is seized before one of the player scores. \fig~\ref{Fig: InteractionBilinear} a,b,c, show interaction plots.  The interaction plots show that \cpg player learns smart interactive strategies of seizing ball from another player and scoring goal. Also, CPG has 0 on the x axis which represents the case, where both player keep of snatching ball from each other and no one could score goal with in 1000 steps. 

% \begin{figure}[h]
% 	\centering
%     \begin{subfigure}[t]{0.23\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/cpg_cpg_interaction_plot.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: cpg_cpg_interaction_plot}
%     \end{subfigure}
% ~
%     \begin{subfigure}[t]{0.23\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/cpg_sgd_interaction_plot.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: cpg_sgd_interaction_plot}
%     \end{subfigure}
%   ~
%     \begin{subfigure}[t]{0.23\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/sgd_sgd_interaction_plot.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: sgd_sgd_interaction_plot}
%     \end{subfigure}
% ~
%   \begin{subfigure}[t]{0.23\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/sgd_cpg_winning_plot.pdf}  
%     \caption{}
%     \label{Fig: sgd_cpg_winning_plot}
%   \end{subfigure}
% %  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
% %   \setlength{\abovecaptionskip}{-13pt}
% %   \setlength{\belowcaptionskip}{-10pt}
%   \caption{a),b),c) are interaction plots. The x axis follows following convention, 1(odd): A scores goal, 2(even): B scores goal, 3: A scores goal after seizing ball from B. 4: B scores goal after seizing ball from A, 5: A scores goal by seizing ball from B which took ball from A. Similarly, Ceil[x/2] denotes number of times ball has been seized from each other before scored by player A (x=odd) or player B (x=even), where x is the x-axis index d) Represents probability of games won when \cpg competed against \gdapg played being both player A and B \manish{Change 4th plot size}}
%   \label{Fig: InteractionBilinear}
% \end{figure}

\subsection{Car Racing game (ORCA)}
\label{appx: ORCADescription}
Our final experimental setup is a racing game between two miniature race cars, where the goal is to finish the one lap race first. This involves both, learning a policy that can control a car at the limit of handling, as well as strategic interactions with the opposing car. Only if one is relative position to the opponent is correct, one is able to overtake or to block an overtaking. Our simulation study mimics the experimental platform located at ETH Zurich, which use miniature autonomous race cars\footnote{see \url{www.youtu.be/asdf} for an example of two cars racing on the experimental setup}.

Following ~\citet{Liniger2017OptimizationBasedAR} the dynamics of one car is modeled as a dynamic bicycle model with Pacejka tire models ~\citep{mf}. However, compared to ~\citet{Liniger2017OptimizationBasedAR} we formulate the dynamics in curvilinear coordinates cite[] where the position and orientation are represented relative to a reference path. This change in coordinates significantly simplifies the definition of our reward, and is simplified the policy learning. The resulting state of a single car is given as $z =  [\rho, d, \mu, V_x, V_y, \psi]^T$, where $\rho$ is the progress along a reference path, $d$ is the deviation from a reference path, $\mu$ is the heading local heading with respect to the reference path, $V_x$ and $V_y$ are the longitudinal and the lateral velocity respectively in car frame and $\psi$ is the yawrate of the car. The inputs to the car is $[D, \delta]^T$, where $D \in [-1, 1]$ is duty cycle input to the electric motor varying from full braking at $-1$ to full acceleration at $1$ and $\delta \in [-1, 1]$ is the steering angle. The test track which consists of 13 turns with different curvature can be seen in Figure \ref{Fig: orca}. For the reference path we used the X-Y path obtained by a laptime optimization tool cite[], note that it is not necessary to use a pre-optimize reference path, but we saw that it helped the convergence of the algorithm. Finally, to get a discrete time MDP we discretize the continuous time dynamics using an RK4 integrator and a sampling time of 0.03s. 

To formulate the racing game between to cars, we first define the state of the game as the concatenated state of the two players, $s = [z^1,z^2]$. Second we convert the objective of finishing the race first without an accident into a zero sum game. Therefore, we define the following reward function using reward shaping. First to model our no accident constraints we use a freezing mechanism: (i) If the car is leaving the track we freeze it until the episode ends, (ii) if the cars collide, the rear car (car with the lower progress $\rho$) is stopped for 0.1s, which corresponds to a penalty of about two car lengths. Note that this gives an advantage to the car ahead, but in car racing the following car has to avoid collisions. Furthermore, an episode ends if both cars are either frozen due to leaving the track or the first car finished the lap. Finally, to reward racing the players at every time step receive the following reward $r(s_k,a^1_{k+1},a^2_{k+1}) = \Delta \rho_{car_1} - \Delta \rho_{car_2}$, where $\Delta \rho = \rho_{k+1} - \rho_k$. This reward encourages the player to get as far ahead of the of the opponent player as possible. 

For the training we started the players on the start finish line ($\rho = 0$) and randomly  assigned $d \in \{0.1, -0.1\}$. We also limited one episode to 700 time steps, which is about twice as long as it takes and expert player to finish a lap. For each policy gradient step we generated a batch of 8 game trajectories, and we run the training for roughly 20000 epochs until the player consistently finish the lap. To increase the performance and robustness of learning we adapted the learning rate with RMSprop for both \gda and \cpg and used a slow learning rate of $5.10^{-5}$ for both players. For our experiments we run 8 different random seeds and report the numbers of the best seed. As a policy we use a mulit-layer perceptron with tow hidden layer, each with 128 neurons, we used ReLU activation functions and a Tanh output layer to enforce the input constraints. 

\subsection{Comparison with MADDPG}
\label{appx: maddpg_comp}
We compared performance of \cpg with multi agent deep deterministic policy gradient (\maddpg)~\citep{lowe2017multi} on the game of soccer and the car racing game.
% \maddpg is \gda based algorithm and hence diverges in non transitive game such as RPS, MP and bilinear game. 
To compare performance of \maddpg on discrete action space, we used policies that can produce differentiable samples through a Gumbel-Softmax distribution, similar to ~\citep{iqbal19a}. Both the experiments are conducted for 8 random seeds. \fig~\ref{fig: EX_sgd_maddpg_winning_plot}  show that policy learnt by \maddpg agent is similar to that of \gda. But when competed against \cpg, \fig~\ref{fig: EX_sgd_maddpg_winning_plot} shows that \cpg agent wins 80\% of the games. Next we evaluated \maddpg policy in the game of car racing. \fig~\ref{fig: progress_plot_orca_maddpg} show that training behaviour is similar to \gda. The car learns to drive upto 30\% of the track, but after that agent show oscillatory behaviour in training as shown in \fig~\ref{fig: progress_plot_orca_maddpg}.  
% \begin{figure}[h]
% % \hspace{-4.00mm}
% 	\centering
%     \begin{subfigure}[t]{0.25\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/EX_sgd_maddpg_winning_plot.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{fig: EX_sgd_maddpg_winning_plot}
%     \end{subfigure}
%     % \hspace{-4.00mm}
% ~
%     \begin{subfigure}[t]{0.25\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/EX_cpg_maddpg_winning_plot.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: EX_cpg_maddpg_winning_plot}
%     \end{subfigure}
%     % \hspace{-4.00mm}
%  ~
%   \begin{subfigure}[t]{0.25\columnwidth}
%   \centering
%   \includegraphics[width=\linewidth]{images/progress_plot_orca_maddpg.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{fig: progress_plot_orca_maddpg}
%     \end{subfigure}
%     % \hspace{-4.00mm}
%   \caption{Policy evaluation on the game of soccer a) \gda vs \maddpg b) \cpg vs \maddpg c) Progress plot of \maddpg during training in the car racing game}
%   \label{fig: MADDPG_plots}
% \end{figure}


% We trained the racing game with both \gda and \cpg, even thought both players were able to learn to "drive" only \cpg was able to learn how to "race". With \gda, only one player was able to learn, this either manifested in one player completely failing and the other finishing the race, or by a oscillation behavior or by an oscillation behavior where when one agent learns to go ahead, the other agent learns to stay at lower progress. Even if at some point one of the players learns to finish one lap, the player does not learn to interact with the other opponent. The players trained with \cpg on the other hand, both progress and learn both to finish the lap and to interact with each other. 

% See \fig~\ref{fig: ProgressOrcaCPG}, where the progress the two players at the end of an episode can be seed for \gda and \cpg, it is clearly visible that with \cpg both players get better over time, whereas in \gda the two player have an oscillation behavior, and at the end only one of the two players finishes one lap. 


% \begin{figure}[h!]
% 	\centering
%     \begin{subfigure}[t]{0.32\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/orca_sgd.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{fig: orca_sgd}
%     \end{subfigure}
%     ~
% %     \begin{subfigure}[t]{0.32\columnwidth}
% %   	\centering
% %   	\includegraphics[width=\linewidth]{images/orca_sgd_swing.pdf}
% % %   	\setlength{\abovecaptionskip}{0pt}
% % %   	\setlength{\belowcaptionskip}{0pt}
% %     \caption{}
% %     \label{fig: orca_trpo_gdap2}
% %     \end{subfigure}
% %     ~
%     \begin{subfigure}[t]{0.32\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/orca_cpg_progress_plot.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{fig: orca_cpg_progress_plot}
%     \end{subfigure}
%   \caption{Progress of agents while training a) \gda b) \cpg both at  learning rate = 5e-5}
%   \label{fig: ProgressOrcaCPG}
% \end{figure}

% To test the policies, we run 5000 episodes with the obtained policy. To evaluate the performance we run three types of races, \gda vs \gda, \cpg vs \cpg, \gda vs \cpg. For each episode, we counted the number of overtakes, the number of collisions with the track constraints and recorded the lap time. For the \gda vs \cpg test we also counted the number of times which policy won, where we defined winning as finishing first. Since, \gda often collided with the track constraints, for the test we replaced the freezing with a reset at the reference path routine. 

% \begin{table}[ht]
% \centering 
% \begin{tabular}{|c||c|c|c|}
% \hline
%  & \cpg vs \cpg & \gda vs \gda \\
%  \hline \hline
%  Overtaking per lap & 16772/3.35 & 3419/0.68  \\
%  \hline
%  Track collision per lap & 2941/0.59 & 5613/1.12  \\
%  \hline
%  Laptime  & 10.89 & 13.32  \\
%  \hline
% \end{tabular}
% \caption{Quantitative results for the racing game}
% \label{tab: orca_same_players}
% \end{table}

% In Table \ref{tab: orca_same_players} we can clearly see that \cpg learned a policy that is both faster and more precise, as well as more interactive with about six times as many overtaking maneuvers. Thus, it is not surprising that in the 5000 race between \gda vs \cpg, \gda was only able to win 103 times. For these races we also noted that the \gda player, go ``confused" by the interactive \cpg player which resulted in crashes of the \gda player, since the \gda player never experience such interactions in training. 

% Finally we want to study the type of strategies the \cpg players learned for overtaking and blocking. First, the player which is ahead clearly learned that he/she has strategic advantage, and on purpose braked to cause a freezing the following player. This strategy on the other hand resulted in adequate overtaking strategy which involved a significant safety distance.....



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The ORCA setup is developed at ETH Zurich for the purpose of developing high speed and real time path planning and control algorithms. The ORCA simulator uses dynamic bicycle model ($Cite car model$) and tire forces are modelled using Pacejka Magic formula 6.2 ($Cite mf$), further details are in appendix. The state $x \in R^n$ of race car is formulated in curvilinear coordinates, given by $ x = [\rho, d, \mu, V_x, V_y, \psi]^T$ where, $\rho$ is progress along a reference path, $d$ is deviation from a reference path, $\mu$ is heading deviation from a reference path, $V_x$ is longitudinal velocity in car frame, $V_y$ is lateral velocity in car frame and $\psi$ is yawrate of the car.

% The reference path can be any line in the track, for our experiments we took a laptime optimised trajectory. The control inputs are $[D, \delta]^T$, where $D \in [-0.2, 1]$ is throttle varying from full braking at -0.2 to full acceleration at 1 and $\delta \in [-0.35, 0.35]$ is steering angle from extreme left to extreme right. The dynamics are propagated using RK4 integrator. The track shown in \fig~\ref{Fig: orca}, tries to capture trajectory of varying bend radius, ranging from straights to $180^0$ turns in both left hand and right hand curvatures. 

% \begin{figure}[ht]
%   	\centering
%   	\includegraphics[width=0.48\linewidth]{images/orca.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{The ORCA setup}
%     \label{Fig: orca}
% \end{figure}

% The ORCA setup is extended to the multi-car setup, for training under full observability we define state for car $i \in \{1,2\}$ as  $[state_{car_i}, state_{car_{i-}}]^T$, where $state_{car_i} = [\rho, d, \mu, V_x, V_y]^T$. Please note the $\psi$ dropped to reduce state size. The game starts with both the cars placed at start line which is $\rho = 0$ and randomly assigned $d \in \{0.1, -0.1\}$. The aim for each car is to beat the opponent by finishing as soon as possible and while avoiding collision and track boundaries. This task is formulated as zero sum game with reward shaping given below:
% \begin{itemize}
%     \item $r(s_k,a^1_{k+1},a^2_{k+1}) = \Delta \rho_{car_1} - \Delta \rho_{car_2}$, 
%     $\Delta \rho = \rho_{k+1} - \rho_k$
%     \item Track constraints are incorporated using a freezing mechanism, once a car hits the track boundary, it's state is not propagated any more and hence $\Delta \rho_{car_i} = 0$ and based on performance of other car it receives a penalty. This reward structure indirectly penalises a car more if it hits in the beginning as compared to later.
%     \item Collisions constraints are similar to prey-predator game, the rear car is penalised for collision where as car in the front is awarded to promote blocking. Following freezing mechanism, here also we freeze the rear car but only for 0.1 seconds.
%     \item The car's state trajectory is collected by propagating until one of them reaches finish line or both cars reach freezing state.
% \end{itemize}

% This experiment was used to compared performance of \gda and \cpg. The naive \gda failed to converge where as \cpg was able to drive but had hard time learning more than 30\% of the track. We extended formulation of \gda and \cpg to adapt learning rate using RMS prop. Both are trained for 20000 episodes, for each episode we do a batch update. The batch is formed using 8 game trajectories, where the maximum trajectory length is restricted to 700 steps. Under give parameters, it takes 13 hours to train on a single core cpu and has been trained for 8 different random seeds. The algorithms are tuned for learning rates. We observed that a few times \gda faces oscillation while training i.e., when an player maximises his progress, the other player performance shrink to a low progress, hence the player learns to drive but given that the other player has low progress. Due to this once the learnt player is competed with strong opponent e.g., itself, then the both players tend to go out due to unforeseen state space during training. In case of \cpg, we observe that both player are trained together to maximise their progress. \cpg was able to learn the strategy of blocking and avoiding collisions. Further we competed \cpg with \gda with either of them as player 1 and player 2. The player with higher progress at the end of the game is declared as winner. We selected best trajectories according to maximum progress during training, and played 5000 games. During test, we reset player to center of the track upon collision with the track boundaries, for competitiveness between players. Table~\ref{tab: orca_same_players}, shows results for game between \cpg vs \cpg and \gda vs \gda. The trained players with \cpg tries to block and overtakes more often through out the track as compared to \gda where the player hardly overtakes apart from the start zone. \gda had hard time for both players to reach to the goal together, this is presumably due to unexplored state space. On competing with \cpg with \gda, \cpg wins almost all the matches due to better interactive strategies learnt by \cpg player. \manish{Make trajectory plot showing blocking and avoiding collision}  

% \begin{table}[ht]
% \centering 
% \begin{tabular}{|c||c|c|c|}
% \hline
%  & CPG vs CPG & GDA vs GDA \\
%  \hline \hline
%  Overtaking & 16772 & 3419  \\
%  \hline
%  Collosions & 2941 & 5613  \\
%  \hline
%  Laptime  & 10.89 & 13.32  \\
%  \hline
% \end{tabular}
% \caption{Comparative results for self-play on the ORCA setup}
% \label{tab: orca_same_players}
% \end{table}

% \begin{table}[ht]
% \centering 
% \begin{tabular}{|c||c|c|c|c|}
% \hline
%  & \multicolumn{2}{c|}{CPG vs GDA} &  \multicolumn{2}{c|}{GDA vs CPG} \\
%  \hline \hline
% %  \cline{2-5}
%  Wins & 4873 & 127 & 103 & 4897  \\
%  \hline
%  Overtaking  & 6324 & 3021 & 1927 & 5830  \\
%  \hline
%  Collosions & 2113 & 5114 & 5642 & 1943  \\
%  \hline 
% \end{tabular}
% \caption{Comparative results for \cpg vs \gda on the ORCA setup}
% \label{tab: orca_diff_players}
% \end{table}

% \manish{to do: Make histogram of number of overtakes/blocking for cpg vs cpg and gda vs gda, laptime for gda and cpg, Number of wins for cpg vs gda, number of collosions }
% Out of 5000, for 50\% games, \gda was player 1 for remaining 50\% \cpg was player 1. As shown in the histogram below, we observe that \cpg won 68\% games, among all the collisions and blocking in the games 84\% times victim was policy trained using \gda.       


% Apart from comparing performance on LQ game, we introduce bilinear terms in the cost function in order to tightly couple action (interaction) of two players.  \eq~\ref{eq : lq_game}, The resulting objective function of the player 1 (player 2) is to maximise (minimise) the infinite horizon rewards, takes the form,
% \begin{gather*} \label{eq: lq_bilinear }
%     J(K^1,K^2) = \max_{K^1} \min_{K^2} \mathbb{E} \biggl[ \sum_{k=0}^{\infty} {x_k}^T Q x_k + {u^1_k}^T R_{11} u^1_k   + \ {u^2_k}^T R_{22} u^2_k +  {u^1_k}^T R_{12} u^2_k + {u^2_k}^T R_{21} u^1_k \biggr] \numberthis
% \end{gather*}


% \subsubsection{Linear Bilinear game}
% Next, we considered a cases in which cost is given by \eq \eqref{eq: bilinear }. Here, $K^{1},K^{2}$ are controller policies, modelled as Gaussian distribution. $K^{1*} = K^{2*} = 0$ is a stationary point for this game. Different horizon lengths were considered, if it's is higher, then learning rate has to be low otherwise larger steps make system unstable. With increasing horizon, \gdapg diverges more readily and \cpg takes more time to converge to the origin. We never observed divergence of \cpg in our experiments for reasonable learning rate for the bilinear game. \fig~\ref{Fig: LinearBilinear}, shows plots for trajectories of both the players with horizon h=2,5 for both \gdapg and \cpg. We trained it for 20,000 iterations, parameters for \gdapg and \cpg were exactly same, although \cpg could have much high lr as compared to \gdapg. Also, it was observed that if critic loss increases, the controller policies moves away from the origin until critic loss is reduces again this is presumably due to exploring new states.  

% \begin{gather*} \label{eq: bilinear }
%     J(K^1,K^2) = \max_{K^1} \min_{K^2} \mathbb{E} \biggl[ \sum_{k=0}^{\infty} {u^1_k}^T R_{12} u^2_k + {u^2_k}^T R_{21} u^1_k \biggr] \numberthis
% \end{gather*}


% \begin{figure}[ht]
% 	\centering
%     \begin{subfigure}[t]{0.48\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/sgd_h2.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: sgd_h2}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[t]{0.48\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/cpg_h2.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: cpg_h2}
%     \end{subfigure}
    
%     \begin{subfigure}[t]{0.48\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/sgd_bilinear_lre_h5.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: sgd_bilinear_lre_h5}
%     \end{subfigure}
% ~
%   \begin{subfigure}[t]{0.48\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}  
%     \caption{}
%     \label{Fig: cpg_bilinear_lr2_h5_critic_lr2}
%   \end{subfigure}
% %  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
% %   \setlength{\abovecaptionskip}{-13pt}
% %   \setlength{\belowcaptionskip}{-10pt}
% \protect\caption{Represents policy trajectories for player 1 and player 2. \protect\mystar{green} is start point and \protect\mystar{red} is end point. (a) \gdapg, h = 2 (b) \cpg, h=2 (c) \gdapg, h=5 (d) \cpg, h=5 }
%   \label{Fig: LinearBilinear}
% \end{figure}
% We considered game for \eq \eqref{eq: lq_bilinear }, representing mixed bilinear and quadratic costs, the results were intermediate between the 2 cases presented above.




\begin{figure}[!h]
\hspace{-3.00mm}
	\centering
    \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/EX_sgd_trpo_winning_plot.pdf}
    \caption{\gda vs \trpogda}
    \label{Fig: EX_sgd_trpo_winning_plot}
    \end{subfigure}
    \hspace{-4.00mm}
    ~
    \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/EX_trpo_cpg_winning_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{\trpogda vs \cpg }
    \label{Fig: EX_trpo_cpg_winning_plot}
    \end{subfigure}
    \hspace{-4.00mm}
    ~
    \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/EX_cpg_trcpo_winning_plot.pdf}
    \caption{\cpg vs \trcpo}
    \label{Fig: EX_cpg_trcpo_winning_plot}
    \end{subfigure}
    \hspace{-4.00mm}
~
  \begin{subfigure}[t]{0.26\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/EX_sgd_trcpo_winning_plot.pdf}
    \caption{\gda vs \trcpo}
    \label{Fig: EX_sgd_trcpo_winning_plot}
  \end{subfigure}
  \hspace{-4.00mm}
  \caption{ Win probability in soccer game played between \gda, \cpg, \trpogda and \trcpo }
  \label{fig: CompMarkovScoccer}
\end{figure}
\begin{figure}[h]
{
    \begin{subfigure}[t]{0.30\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/Soccer.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
% \vspace{-6.00mm}
    \caption{}
    \label{fig: Soccer}
    \end{subfigure}
    % \hspace{-10.00mm}
    
\vspace{-35.00mm}
    
   	% \hspace{-5.00mm}
    \begin{subfigure}[t]{0.18\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/EX_sgd_maddpg_winning_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: EX_sgd_maddpg_winning_plot}
    \end{subfigure}
    % \hspace{-6.00mm}
~
  \begin{subfigure}[t]{0.18\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/EX_cpg_maddpg_winning_plot.pdf}
    \caption{}
    \label{fig: EX_cpg_maddpg_winning_plot}
  \end{subfigure}
%   \hspace{-6.00mm}
}
    ~
    \begin{subfigure}[t]{0.5\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/overtaking_manuever_northsouth.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: overtaking_manuever_northsouth}
    \end{subfigure}
    % \hspace{-12.00mm}
    
    \caption[Caption for LOF]
    {a) The Markov Soccer Game, b \& c) Win probability in the soccer game played between  b) \gda vs \maddpg c) \maddpg d) Overtaking maneuvers\footnotemark of \cpg agents in the Car Racing Game. The thick line shows trajectory when the trailing agent overtook.}
    \label{Fig: orca}
  \hspace{-4.00mm}
  \vspace{-5.00mm}
\end{figure}
\footnotetext{Video is available here}

==> extra/appx4-trcpo_experiment.tex <==
\subsection{TRCPO on the games of known Nash Equilibrium}
\label{appx: TRCPOgameNash}
\subsubsection{Bilinear game}
The setup is explained in \sect~\ref{appxsec: CPGBilinear}. The agent’s policy is modelled as a Gaussian distribution. Both agents play actions simultaneously and receive rewards based on product of their actions. Starting from some random policy initialization \trcpo converges to the unique Nash equilibrium of the game whereas \trpogda diverges for all $\delta$. \fig~\ref{fig: TRCPOBilinear} shows such behavior for $\delta$ of 0.001. Experiment was performed for 8 different random seeds.
% \fig~\ref{fig: TRCPOBilinear_policyvsstep} shows agents' policies with iteration, there is a phase shift, which marks agents that an agent turn to slow down given other agent cross the origin mark. But here \trpogda is not aware of ther other agent and just maximise his reward, which lead to larger negative reward in next iterations.
\begin{figure}[ht]
	\centering
%     \begin{subfigure}[t]{0.32\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/trcpo_bilinear.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: trcpo_bilinear}
%     \end{subfigure}
%     ~
    \begin{subfigure}[t]{0.32\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/trpo2gda_bilinear_steps.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: TRCPOBilinear_policyvsstep}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.32\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/trcpo_bilinear_steps.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: trcp2gda_bilinear_steps}
    \end{subfigure}
\caption{Policy trajectories of player 1 in a bilinear game. (a) \trpogda (b) \trcpo}
%\protect\mystar{green} is start point and \protect\mystar{red} is end point. 
  \label{fig: TRCPOBilinear}
\end{figure}
% \subsection{LQ game}

\subsubsection{Matching pennies}
The game is explained in \appx~\ref{appxsec: CPGMP} 
% Similar to \cpg~\ref{sec: CPGMP}, Each agent's policy is modelled as categorical distribution with 2 classes. Agents sample actions from softmax probability function over categorical distribution. They receive reward for their actions according to their game matrix~\ref{tab: matching_pennies}.
In the Matching pennies game we observe that \trcpo converges to unique Nash equilibrium of the game $(H,T)$ = $\bigl(\frac{1}{2}, \frac{1}{2} \bigr)$, whereas \trpogda diverges for all $\delta$. \fig~\ref{fig: TRCPOMatchingPennies} shows this behaviour for $\delta$ of 0.01. Experiment was performed for 8 different random seeds.

\begin{figure}[ht]
	\centering
    \begin{subfigure}[t]{0.32\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/trpo2gda_matching_pennies.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: trpo2gda_matching_pennies}
    \end{subfigure}
    ~
        \begin{subfigure}[t]{0.32\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/ctrpo_matching_pennies.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: trcpo_matching_pennies}
    \end{subfigure}
\caption{Policy trajectories of player 1 and player 2 for the game of matching pennies (a) \trpogda (b) \trcpo }
  \label{fig: TRCPOMatchingPennies}
\end{figure}

\subsubsection{Rock Paper Scissors game}
The game is explained in \appx~\ref{appxsec: CPGRPS}.
% Similar to \cpg~\ref{sec: CPGRPS}, Each agent's policy is modelled as categorical distribution with 3 classes. Agents sample actions from softmax probability function over categorical distribution. They receive reward for their actions according to their game matrix~\ref{tab: rock_paper_scissors}. 
In the game of RPS, \trcpo agent converges to unique Nash equilibrium of the game $(R,P,S)$= $\bigl(\frac{1}{3}, \frac{1}{3}, \frac{1}{3} \bigr)$, where as \trpogda diverges. \fig~\ref{fig: TRCPORPS} shows this behavior for $\delta$ of 0.001.  Experiment was performed for 8 different random seeds.

\begin{figure}[h!]
    \centering
    \begin{subfigure}[t]{0.23\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/trpo2gda_rps_p1.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: trpo2gda_rps_p1}
    \end{subfigure}
    ~
    \centering
    \begin{subfigure}[t]{0.23\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/trpo2gda_rps_p2.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: trpo2gda_rps_p2}
    \end{subfigure}
    ~
	\centering
    \begin{subfigure}[t]{0.23\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/trcpo_rps2_p1.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: trcpo_rps2_p1}
    \end{subfigure}
    ~
    \centering
    \begin{subfigure}[t]{0.23\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/trcpo_rps2_p2.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{Fig: trcpo_rps2_p2}
    \end{subfigure}

\caption{Policy trajectories in a rock paper scissors game. (a) Player 1 \trpogda (b) Player 2 \trpogda (c) Player 1 \trcpo (d) Player 2 \trcpo}
  \label{fig: TRCPORPS}
\end{figure}

\subsubsection{Markov Soccer}
\label{appxsec: TRCPOsoccer}
% \begin{figure}[h!]
% 	\centering
%     \begin{subfigure}[t]{0.23\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/trcpo_trcpo_gmres_interaction_plot.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: trcpo_trcpo_gmres_interaction_plot}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[t]{0.23\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/trpo_trcpo_gmres_interaction_plot.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: trpo_trcpo_gmres_interaction_plot}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[t]{0.23\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/trpo_trpo_gmres_interaction_plot.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: trpo_trpo_gmres_interaction_plot}
%     \end{subfigure}
% ~
%   \begin{subfigure}[t]{0.23\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/trpo_trcpo_winning_plot.pdf}  
%     \caption{}
%     \label{Fig: trpo_trcpo_winning_plot}
%   \end{subfigure}
% %  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
% %   \setlength{\abovecaptionskip}{-13pt}
% %   \setlength{\belowcaptionskip}{-10pt}
%   \caption{a) \trcpo vs \trcpo, b) \trpogda vs \trcpo, c) \trpogda vs \trpogda. a,b,c are interaction plots.  X-axis convention, 1: A scored goal, 2: B scores goal, 3: A scored goal after seizing ball from B. 4: B scores goal after seizing ball from A, 5: A scored goal by seizing ball from B which took the ball from A and so forth. 0: No one scores goal both kept on seizing from each other for 1000 steps.}
%   \label{fig: TRCPOMarkovScoccer}
% \end{figure}
The game setting is similar to explained in \ref{appxsec: soccer}.
The players were trained in a self play setting, with \trcpo or \trpogda. Both the agents were trained for 5,000 episodes, each episode denotes a batch update where each batch consists of 10 trajectories.  The game ends if any player scores a goal or none of them scores within 1000 steps. The experiment was run with 6 different random seeds. We used \GAE~ for advantage estimation with $\lambda = 0.95$ and $\gamma =0.99$. The players were trained in a self-play manner, with \trcpo or \trpogda. For comparison, we played 10000 games between agents trained using \trcpo and with that using \trpogda, in which for 50\% of the games \trcpo was player A and for remaining \trpogda was player A. \trpogda renders unequal players, on competing with stronger \trpogda agent, still \trcpo agent, won more than 75\% games against \trpogda as shown in \fig~\ref{Fig: trpo_trcpo_winning_plot}. \trcpo was able to learn better tactics for snatching the ball and dodging and defending its goal post.
% Similar to~\ref{sec: CPGMarkovSoccer}, we plotted interaction plots \fig~\ref{fig: TRCPOMarkovScoccer}[a,b,c] for \trcpo vs \trcpo, \trpogda vs \trpogda and \trpogda vs \trcpo respectively. The interaction plots show that the \trcpo agent learned much better strategies of seizing ball from opponent and scoring goal, whereas \trpogda could hardly take the ball from \trcpo \fig~\ref{Fig: trpo_trcpo_gmres_interaction_plot}. Also, \trcpo has 0 on the x-axis. Also note that \trpogda renders unequal players, due to which one player 1 gets ball quite often which corresponds to high bar corresponding to x = 3 in \fig~\ref{Fig: trpo_trpo_gmres_interaction_plot}.

% We further compared \gdapg, \cpg, \trpogda, and \trcpo on 10000 games played against each other. We observed that \trcpo performs best,\cpg was runner up, then \trpogda, and lastly \gda, as shown in the figure below.

% \begin{figure}[ht]
% 	\centering
%     \begin{subfigure}[t]{0.23\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/EX_sgd_trpo_winning_plot.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: EX_sgd_trpo_winning_plot}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[t]{0.23\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/EX_trpo_cpg_winning_plot.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: EX_trpo_cpg_winning_plot}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[t]{0.23\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/EX_cpg_trcpo_winning_plot.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: EX_cpg_trcpo_winning_plot}
%     \end{subfigure}
% ~
%   \begin{subfigure}[t]{0.23\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/EX_sgd_trcpo_winning_plot.pdf}
%     \caption{}
%     \label{Fig: EX_sgd_trcpo_winning_plot}
%   \end{subfigure}
% %  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
% %   \setlength{\abovecaptionskip}{-13pt}
% %   \setlength{\belowcaptionskip}{-10pt}
%   \caption{The games are player between a)\gda vs \trpogda b) \trpogda vs \cpg ,c) \cpg vs \trcpo and d) \gda vs \trcpo}
%   \label{fig: CompMarkovScoccer}
% \end{figure}


\subsubsection{Car Racing game}
\label{appxsec: TRCPOorca}
% The game is explained in Section~\ref{sec: CPG_ORCA}. 
% \begin{figure}[h!]
% 	\centering
%     \begin{subfigure}[t]{0.31\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/trpo2gda_player1.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{fig: orca_trpo_gdap1}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[t]{0.31\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/trpo2gda_player2.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{fig: orca_trpo_gdap2}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[t]{0.31\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/progress_plot_orca_trcpo.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{fig: orca_trcpo}
%     \end{subfigure}
% ~
%   \begin{subfigure}[t]{0.48\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/EX_sgd_trcpo_winning_plot.pdf}
%     \caption{}
%     \label{Fig: bilinear}
%   \end{subfigure}
% %  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
% %   \setlength{\abovecaptionskip}{-13pt}
% %   \setlength{\belowcaptionskip}{-10pt}
%   \caption{Progress of agents while training a) Player1 \trpogda b) Player2 \trpogda c) \trcpo both players $\delta$=5e-4}
%   \label{fig: ProgressOrca}
% \end{figure}

The game setting is similar to explained in \sect~\ref{appx: ORCADescription}. Here, this experiment is used to compare performance of \trcpo and \trpogda. Both are trained for 20000 episodes, for each episode we do a batch update. The batch is formed using 8 game trajectories, where the maximum trajectory length is restricted to 700 steps. We used $\delta$ between 1e-4 to 1e-5 and ran algorithm for 8 different random seeds. \GAE~ is used for advantage estimation with $\lambda = 0.95$ and $\gamma =0.99$. During training, it is observed that \gda faces oscillation while training i.e. when an agent maximizes his progress, the other agent performance shrink to low progress due to zero-sum formulation. Also, a few times, one agent collapses near-zero progress, and the other agent learns to drive in this stationary environment as shown in the \fig~\ref{fig: ProgressOrca}. Due to this when the learned agent is competed against a strong opponent e.g., itself, then both agents tend to go out due to unforeseen state space during training.
In the case of \trcpo, we observe that both agents are trained together to maximize their progress. \trcpo was able to learn the strategy of blocking and avoiding collisions.
Further, we competed \trcpo with \trpogda with either of them as player 1 and player 2. Similar to~\ref{sec: CPG_ORCA}, The player with higher progress at the end of the game is declared as the winner.We selected policies according to maximum progress during training and played 5000 games.
% During test, we reset agent to center of the track upon collision with the track boundaries, for competitiveness between agents. 

\begin{table}[ht]
\centering 
\begin{tabular}{|c||c|c|c|}
\hline
 & \trcpo vs \trcpo & \trpogda vs \trpogda \\
 \hline \hline
 Overtaking per lap & 3.35 & 0.68  \\
 \hline
 Track collision per lap & 0.59 & 1.12  \\
 \hline
 Laptime  & 10.89 & 13.32  \\
 \hline
\end{tabular}
\caption{Quantitative results for the racing game}
\label{tab: orca_trcpo}
\end{table}

Table~\ref{tab: orca_trcpo},shows normalised results for game between \trcpo vs \trcpo and \trpogda vs \trpogda. The trained agents with \trcpo try to block and overtake more often throughout the track as compared to \trpogda where the agent hardly overtakes apart from the start zone. \trpogda had a hard time for both agents to reach the goal together, this is presumably due to unexplored state space. On competing with \trcpo with \trpogda, \trcpo wins almost all the matches due to better interactive strategies learned by \trcpo agent.


==> extra/cpg_proof_complete.tex <==
\newpage
\section{Competitive policy gradient}
\subsection{Proof for \prop~\ref{prop: CPOGradHessianTrajDist}:}
\label{appx: CPOGradHessianTrajDist}

% \begin{proposition}\label{appxprop: CPOGradHessianTrajDist}
% Given a \CMDP, for each player $i\in\!\lbrace 1,2\rbrace$ and its policy parameterized with $\theta^i$,
% \begin{align*}%\label{eqn: Hessiantrajectorydistribution}
% \!D_{\theta^i}\eta(\theta^1,\theta^2) \!=\!\! \int_{\tau}\! f(\tau;\theta^1,\theta^2) g(\tau, \theta^i) R(\tau) d\tau,\textit{and}~D_{\theta^2\theta^1} \eta(\theta^1,\theta^2)\! =\!\! \int_{\tau}\! f(\tau;\theta^1,\theta^2)  g(\tau, \theta^2) g(\tau, \theta^1)^\top R(\tau) d\tau.
% \end{align*}
% with $g(\tau, \theta^i):= D_{\theta^i}(\log(\prod_{k=0}^{|\tau|-1} \pi(a_{k}|s_k;\theta^i)))$ denote the score function.
% \end{proposition}
\begin{proof}
we know that the game objective is,
\begin{align}
\eta(\theta^1,\theta^2) = \int_{\tau} f(\tau;\theta^1,\theta^2) R(\tau) d\tau, \ i\in\!\lbrace 1,2\rbrace\,,
\end{align}
thus, the gradient with respect to $\theta_i$ is given by
\begin{align}
D_{\theta^i}\eta = \int_{\tau} D_{\theta_i} f(\tau;\theta^1,\theta^2) R(\tau) d\tau, \ i\in\!\lbrace 1,2\rbrace\,.
\end{align}
using definition of $f(\tau;\theta^1,\theta^2)$ in \eq~\ref{eq: trajectory_distribution}, we can compute the gradient of the game objective, using $D_{\theta} \log p_{\theta}(\tau) = \frac{D_{\theta} p_{\theta}(\tau)}{p_{\theta}(\tau)}$ from standard calculus,
\begin{align}
D_{\theta^i}\eta &= \int_{\tau} f(\tau;\theta^1,\theta^2) (D_{\theta^i}\log(\prod_{k=0}^{|\tau|-1} \pi(a_k|s_k;\theta^i))) R(\tau) d\tau\,, \nonumber\\
&= \int_{\tau} f(\tau;\theta^1,\theta^2) g(\tau, \theta^i) R(\tau) d\tau
\end{align} 
with $g(\tau, \theta^i) = D_{\theta^i}(\log(\prod_{k=0}^{|\tau|-1} \pi(a_{k}|s_k;\theta^i)))$. 
 By definition we know that the second order bilinear approximation of game objective is $D_{\theta^2\theta^1} \eta(\theta^1,\theta^2) = D_{\theta^2} D_{\theta^1}\eta(\theta^1,\theta^2)$. Hence,
\begin{align}
D_{\theta^2\theta^1} \eta &= \int_{\tau} D_{\theta^2}f(\tau;\theta^1,\theta^2) \ g(\tau, \theta^1)^\top \ R(\tau) d\tau\,. \nonumber\\
&= \int_{\tau} f(\tau;\theta^1,\theta^2) (D_{\theta^2}\log(\prod_{k=0}^{|\tau|-1} \pi(a_k|s_k;\theta^2))) g(\tau, \theta^1)^\top R(\tau) d\tau\,, \nonumber\\
&= \int_{\tau} f(\tau;\theta^1,\theta^2) \ g(\tau, \theta^2) \ g(\tau, \theta^1)^\top \ R^1(\tau) d\tau \, . \nonumber
\end{align}
% Using the definition of $f(\tau;\theta^1,\theta^2)$ in \eq~\ref{eq: trajectory_distribution}, and standard calculus, similar to \lem~\ref{prop: PGtrajectorydistribution}, we get the following second order bilinear hessian term of the game objective,
which concludes the proof.
\end{proof}

\subsection{Proof for \thm~\ref{thm: CPGGradHessianVal}}
\label{appx: CPGGradHessianVal}
\subsubsection{Derivation of Gradient term \texorpdfstring{$D_{\theta^1} \eta$}{Lg}}
% \begin{proposition}
% For any two player \CMDP, the gradient of value of the strategic pair $(\theta^1, \theta^2)$ starting from $s_0$ with respect to player 1 is given by,
% \begin{gather*}
% D_{\theta^1} V(s_0;\theta^1,\theta^2) = \int_s d(s) \int_{a^1} \int_{a^2} \Bigl(\frac{\partial \pi(a^1|s;\theta^1)}{\partial \theta^1}  \pi(a^2|s;\theta^2) Q(s,a^1,a^2;\theta^1,\theta^2) \Bigr) \ da^1 \ da^2 \ ds \numberthis 
% \end{gather*}
% where, $d(s)$ is stationary distribution of states under $\pi(\theta^1)$ and $\pi(\theta^2)$, $d(s) = \sum_0^{\infty} \gamma^k Pr(s_0\rightarrow s,\theta^1,\theta^2)$.
% \end{proposition}
\begin{proof}
Using \eq~\ref{eqn: val_rew}, which defines $V^i(s_k;\theta^1, \theta^2)$ and $Q^i(s_k,a^1_{k},a^2_{k};\theta^1, \theta^2)$. We define,
\begin{align}\label{eqn: appxValIntegral}
V(s_0;\theta^1,\theta^2) &= \int_{a_0^1} \int_{a_0^2} \pi(a_0^1|s_0;\theta^1) \  \pi(a_0^2|s_0;\theta^2) Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2) \ da_0^1 \ da_0^2\,, \\
where, \,\, Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2) &= r(s_0,a_0^1,a_0^2) + \ \gamma \int_{s1} T(s_1|s_0,a_0^1,a_0^2) \  V(s_0;\theta^1,\theta^2) \ ds_1\,. \nonumber
\end{align}
Hence, the gradient of the state-value $V$ is,
\begin{align}\label{eqn: gradv}
D_{\theta^1} V(s_0;\theta^1,\theta^2) &= \int_{a_0^1} \int_{a_0^2} \frac{\partial \pi(a_0^1|s_0;\theta^1)}{\partial \theta^1} \ \pi(a_0^2|s_0;\theta^2) \ Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2) \ da_0^1 \ da_0^2 \nonumber\\
& + \int_{a_0^1} \int_{a_0^2}  \pi(a_0^1|s_0;\theta^1) \ \pi(a_0^2|s_0;\theta^2) \ \frac{\partial Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2)} {\partial \theta^1} \ da_0^1 \ da_0^2 \,.
\end{align}
The gradient of the state-action value $Q$, in term of gradient of state-value $V$ is given by
\begin{align}\label{eqn: gradq}
D_{\theta^1} Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2) = \gamma \int_{s1} T(s_1|s_0,a_0^1,a_0^2) \  \frac{\partial V(s_1;\theta^1,\theta^2)}{\partial \theta^1} \ ds_1 \numberthis \,.
\end{align}
Substituting \eq~\ref{eqn: gradq} in \eq~\ref{eqn: gradv} we get,
\begin{align}\label{eqn: recursive_gradv}
D_{\theta^1} V(s_0;\theta^1,\theta^2) &= \int_{a_0^1} \int_{a_0^2} \frac{\partial \pi(a_0^1|s_0;\theta^1)}{\partial \theta^1} \ \pi(a_0^2|s_0;\theta^2) \ Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2) \ da_0^1 \ da_0^2 \nonumber\\
 &+ \int_{a_0^1} \int_{a_0^2}  \pi(a_0^1|s_0;\theta^1) \  \pi(a_0^2|s_0;\theta^2) \  \gamma \int_{s1} T(s_1|s_0,a_0^1,a_0^2) \  \frac{\partial V(s_1;\theta^1,\theta^2)}{\partial \theta^1} \ ds_1 \ da_0^1 \ da_0^2\,. 
\end{align}
By exploring the recursive nature of the state-value $V$ and $D_{\theta^1} V(s_0;\theta^1,\theta^2)$, we can unroll \eq~\ref{eqn: recursive_gradv} as,
% Exploiting recursive structure of \eq \eqref{eqn: recursive_gradv} in terms of $D_{\theta^1} V(s_0;\theta^1,\theta^2)$

\begin{align}
 \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!D_{\theta^1} V(s_0;\theta^1,\theta^2)\!\!&=\int_{a_0^1} \int_{a_0^2} \frac{\partial \pi(a_0^1|s_0;\theta^1)}{\partial \theta^1}\pi(a_0^2|s_0;\theta^2) Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2) da_0^1 da_0^2 \nonumber\\
 \!\!\!&\!\!\!+\!\!\!\int_{a_0^1} \int_{a_0^2}\!\!\!\pi(a_0^1|s_0;\theta^1) \pi(a_0^2|s_0;\theta^2) \gamma\!\!\! \int_{s1}\!\!\! T(s_1|s_0,a_0^1,a_0^2)  \Biggl( \int_{a_1^1} \int_{a_1^2}\!\!\!\frac{\partial \pi(a_1^1|s_1;\theta^1)}{\partial \theta^1} \pi(a_1^2|s_1;\theta^2) Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2) da_1^1 da_1^2 \nonumber\\
 \!\!\!&\!\!\!+\!\!\!\int_{a_1^1} \int_{a_1^2}  \pi(a_1^1|s_1;\theta^1)  \pi(a_1^2|s_1;\theta^2) \gamma \int_{s2} T(s_2|s_1,a_1^1,a_1^2)  \frac{\partial V(s_2;\theta^1,\theta^2)}{\partial \theta^1} ds_2 da_1^1 da_1^2 \Biggr) ds_1  da_0^1 da_0^2 \numberthis \, .\label{eqn: recursive_gradv2}
 \end{align}
 by further marginalizing over actions, we get
 %%%%%%%%%%%%%%%%%%
 {\makeatletter\def\f@size{10}\check@mathfonts\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}
 \begin{align}\label{eqn: Val_Unrolled2steps}
 D_{\theta^1} V(s_0;\theta^1,\theta^2) &= \int_{a_0^1} \int_{a_0^2} \frac{\partial \pi(a_0^1|s_0;\theta^1)}{\partial \theta^1} \  \pi(a_0^2|s_0;\theta^2) \ Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2) \ da_0^1 \ da_0^2 \nonumber\\
 &+ \gamma \int_{s_1} Pr(s_0\rightarrow s_1,1,\theta^1,\theta^2) \biggl(
\int_{a_1^1} \int_{a_1^2} \frac{\partial \pi(a_1^1|s_1;\theta^1)}{\partial \theta^1} \  \pi(a_1^2|s_1;\theta^2) \ Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2) \ da_1^1 \ da_1^2 \biggr)ds_1 \nonumber\\
 &+ \gamma \int_{s_1} Pr(s_0\rightarrow s_1,1,\theta^1,\theta^2) \biggl( \gamma \int_{s_2} Pr(s_1\rightarrow s_2,1,\theta^1,\theta^2) \ \frac{\partial V(s_2;\theta^1,\theta^2)}{\partial \theta^1} \ ds_2 \  \biggr)ds_1\,,
 %%%%%%%%%%%%%%%%%%%
\end{align}}
where, $Pr(s_0\rightarrow s,k,\theta^1,\theta^2)$ represents probability of going from state $s_0$ to state $s$ in $k$ steps. Similar to the two previous step, unrolling and marginalisation can be continued for entire trajectory length, which results in,
% Unrolling and substituting for $ \frac{\partial V(s_2;\theta^1,\theta^2)}{\partial \theta^1} $
%%%%%%%%%%%%%%%%%%
% {\makeatletter\def\f@size{10}\check@mathfonts\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}
%  \begin{align} \label{eqn: Val_Unrolled2steps}
%  D_{\theta^1} V(s_0;\theta^1,\theta^2) &= \int_{a_0^1} \int_{a_0^2} \frac{\partial \pi(a_0^1|s_0;\theta^1)}{\partial \theta^1} \ \pi(a_0^2|s_0;\theta^2) \  Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2) \ da_0^1 \ da_0^2 \nonumber\\
%  &+ \gamma Pr(s_0\rightarrow s_1,1,\theta^1,\theta^2) \biggl(
% \int_{a_1^1} \int_{a_1^2} \frac{\partial \pi(a_1^1|s_1;\theta^1)}{\partial \theta^1} \ \pi(a_1^2|s_1;\theta^2) \  Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2) \ da_1^1 \ da_1^2 \biggr) \nonumber\\
%  &+ \gamma Pr(s_0\rightarrow s_1,1,\theta^1,\theta^2) \gamma Pr(s_1\rightarrow s_2,1,\theta^1,\theta^2)
%  \Biggl( \biggl( \int_{a_2^1} \int_{a_2^2} \frac{\partial \pi(a_2^1|s_2;\theta^1)}{\partial \theta^1} \  \pi(a_2^2|s_2;\theta^2) \ Q(s_2,a_2^1,a_2^2;\theta^1,\theta^2) \nonumber\\
%  &da_2^1 \ da_2^2 \biggr) + \int_{a_2^1} \int_{a_2^2}  \pi(a_2^1|s_2;\theta^1) \ \pi(a_2^2|s_2;\theta^2) \ \gamma \int_{s3} T(s_3|s_2;a_1^1,a_1^2) \  \frac{\partial V(s_3;\theta^1,\theta^2)}{\partial \theta^1} \ ds_3 \ da_2^1 \ da_2^2 \Biggr) \
% \end{align}}
%%%%%%%%%%%%%
% Summing over all the states and for $\infty$ steps, we get: 
{\makeatletter\def\f@size{10}\check@mathfonts\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}
\begin{align}
D_{\theta^1} V(s_0;\theta^1,\theta^2) = \int_{s_k} \sum_{k=0}^{|\tau|} \gamma^k Pr(s_0\rightarrow s_k,k,\theta^1,\theta^2) \int_{a_k^1} \int_{a_k^2} \frac{\partial \pi(a_k^1|s_k;\theta^1)}{\partial \theta^1} \ \pi(a_k^2|s_k;\theta^2) \ Q(s,a_k^1,a_k^2;\theta^1,\theta^2) \ da_k^1 \ da_k^2 \ ds_k \nonumber
\end{align}
$d(s_k) = \sum_{k=0}^{|\tau|} \gamma^k Pr(s_0\rightarrow s_k,k,\theta^1,\theta^2)$, is average number of times player visit state $s_k$ in an episode.
\begin{align}
D_{\theta^1} V(s_0;\theta^1,\theta^2) = \Bigl( \int_{s_k} d(s_k) ds_k \Bigr) \int_{s} \frac{d(s_k)}{\int_{s_k} d(s_k) ds_k} \int_{a_k^1} \int_{a_k^2} \frac{\partial \pi(a_k^1|s_k;\theta^1)}{\partial \theta^1} \ \pi(a_k^2|s_k;\theta^2) \ Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2) \ da_k^1 \ da_k^2 \ ds_k \nonumber
\end{align}}
\begin{align}
D_{\theta^1} V(s_0;\theta^1,\theta^2) = \Bigl( \int_{s_k} d(s_k) ds_k \Bigr) \int_{s_k} \mu(s_k) \int_{a_k^1} \int_{a_k^2} \frac{\partial \pi(a_k^1|s;\theta^1)}{\partial \theta^1} \ \pi(a_k^2|s;\theta^2) \ Q(s,a_k^1,a_k^2;\theta^1,\theta^2) \ da_k^1 \ da_k^2 \ ds \numberthis
\end{align}
where, $\mu(s) = \frac{d(s)}{\int_s d(s) ds}$, is on policy distribution which is fraction of time spent in each state normalised to sum to one. $\int_s d(s) ds$  is average episode length. 

Also, using \eq~\ref{eq: eta_game}, \eq~\ref{eqn: Val_Unrolled2steps}, can be written as:

\begin{align}
D_{\theta^1}\eta(\theta^1,\theta^2) &= \int_{s_0} p(s_0) D_{\theta^1} V(s_0;\theta^1,\theta^2) ds_0 \nonumber\\
&= \int_{s_0} p(s_0) \Biggl[\int_{a_0^1} \int_{a_0^2} \frac{\partial \pi(a_0^1|s_0;\theta^1)}{\partial \theta^1} \  \pi(a_0^2|s_0;\theta^2) \ Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2) \ da_0^1 \ da_0^2 \nonumber\\
 &+ \gamma \int_{s_1} Pr(s_0\rightarrow s_1,1,\theta^1,\theta^2) \biggl(
\int_{a_1^1} \int_{a_1^2} \frac{\partial \pi(a_1^1|s_1;\theta^1)}{\partial \theta^1} \  \pi(a_1^2|s_1;\theta^2) \ Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2) \ da_1^1 \ da_1^2 \biggr)ds_1 \nonumber\\
 &+ \gamma \int_{s_1} Pr(s_0\rightarrow s_1,1,\theta^1,\theta^2) \biggl( \gamma \int_{s_2} Pr(s_1\rightarrow s_2,1,\theta^1,\theta^2) \ \frac{\partial V(s_2;\theta^1,\theta^2)}{\partial \theta^1} \ ds_2 \  \biggr)ds_1\Biggr] ds_0\,,
\end{align}
In terms of trajectory distribution $f(\cdot;\theta^1,\theta^2)$, it can be written as,
\begin{align}
D_{\theta^1} \eta(\theta^1,\theta^2) &= \int_{\tau} \sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0..k-1},s_k;\theta^1,\theta^2) \int_{a_k^1} \int_{a_k^2} \frac{\partial \pi(a_k^1|s_k;\theta^1)}{\partial \theta^1} \ \pi(a_k^2|s_k;\theta^2) \ Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2) \ da_k^1 \ da_k^2 \ d\tau \nonumber\\
&= \int_{\tau} \sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0..k};\theta^1,\theta^2) \frac{\partial \log(\pi(a_k^1|s_k;\theta^1))}{\partial \theta^1} Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2) \ d\tau
\end{align}
% \begin{align}
% D_{\theta^1} V(s_0;\theta^1,\theta^2) = \int_s \sum_0^{\infty} d(s) \int_{a_k^1} \int_{a_k^2} \frac{\partial \pi(a_k^1|s;\theta^1)}{\partial \theta^1} \ \pi(a_k^2|s;\theta^2) \ Q(s,a_k^1,a_k^2;\theta^1,\theta^2) \ da_k^1 \ da_k^2 \ ds \numberthis
% \end{align}
% where $d(s) = \sum_0^{\infty} \gamma^k Pr(s_0\rightarrow s,k,\theta^1,\theta^2)$, which is the $\gamma$ discounted stationary distribution encountered after starting from $s_0$. This concludes our proof. %$\blacksquare$
\end{proof}

% Note that this also allows us to give compute the derivative of the game objecive, which according to Definition \ref{def:gameObj} is given by $\eta^1 (\theta^1,\theta^2) = \int_{s_{0}} p(s_{0})  V^1(s_0;\theta^1, \theta^2) ds_{0} $. Thus, derivative of the game objective is $D_{\theta}\eta^1 (\theta^1,\theta^2) = \int_{s_{0}} p(s_{0})  D_{\theta} V^1(s_0;\theta^1, \theta^2) ds_{0} $. Which 

% \begin{itemize}
% \item Let, $ d(s) = \sum_0^{\infty} \gamma^k Pr(s_0\rightarrow s,k,\theta^1,\theta^2)$ be the $\gamma$ discounted stationary distribution encountered after starting from $s_0$. You can think of it as: \textit{You start from state $s_0$, following policy $(\pi(\theta^1),\pi(\theta^1))$ and as time progress, the probability of going to any state becomes unchanged}. This probability of reaching any state $'s'$ is stationary distribution of $(\pi(\theta^1),\pi(\theta^1))$ starting from $s_0$. 
% \item The game objective in terms of state value function is given by $\eta^1 (\theta^1,\theta^2) = \int_{s_{0}} p(s_{0})  V^1(s_0;\theta^1, \theta^2) ds_{0} $.
% \item Using log trick  ($D_{\theta} \log p_{\theta}(\tau) = \frac{D_{\theta} p_{\theta}(\tau)}{p_{\theta}(\tau)}$)
% \end{itemize}
% Utilising above definitions and trick, we get
%  \begin{align}
% D_{\theta^1} \eta^1 (\theta^1,\theta^2) = \int_{s_0} p(s_0) \int_s d(s) \int_{a_k^1} \int_{a_k^2} \pi(a_k^1|s;\theta^1) \ \pi(a_k^2|s;\theta^2) D_{\theta^1} \log(\pi(a_k^1|s;\theta^1)) \ Q(s,a_k^1,a_k^2;\theta^1,\theta^2) \ da_k^1 \ da_k^2 \ ds \ ds_0  \numberthis
%  \end{align}
% Hence, 
% \begin{gather*}
% D_{\theta^1} \eta^1 (\theta^1,\theta^2) = \mathbb{E} \bigl[ D_{\theta^1} \log(\pi(a_k^1|s;\theta^1)) \ Q(s,a_k^1,a_k^2;\theta^1,\theta^2) \bigr]  \numberthis
%  \end{gather*}

\subsubsection{Derivation of Bilinear term  \texorpdfstring{$D_{\theta^1 \theta^2} \eta(\theta^1,\theta^2)$}{Lg}}
% \begin{theorem}[2]
% For any two player \CMDP, the hessian term second order bilinear approximation of the value function with respect to agent 2 and then agent 1, given a policy parametrization pair $(\theta^1, \theta^2)$, starting from $s_0$, is given by,
% {\makeatletter\def\f@size{9}\check@mathfonts\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}
% \begin{align}
% D_{\theta^1 \theta^2} V(s_0;\theta^1,\theta^2) &= \int_{s} d(s) \int_{a^1} \int_{a^2} \Bigl( \frac{\partial \pi(a^1|s;\theta^1)}{\partial \theta^1} \ \frac{\partial \pi(a^2|s;\theta^2)}{\partial \theta^2}^\top Q(s,a^1,a^2;\theta^1,\theta^2) \Bigr) \ da^1 \ da^2 \ ds \\
% + \mathbb{E}_{a_0^1}\mathbb{E}_{a_0^2} \mathbb{E}_{s_{T1}} \ \Biggl[  \mathbb{E}_{a_1^1}\mathbb{E}_{a_1^2} &\mathbb{E}_{s_{T2}} ...  \biggl[ \sum_{k=1}^{\infty} \ \gamma^k \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i+1}^1|s_i;\theta^1))}{\partial \theta^1} \frac{\partial \log(\pi(a_{k+1}^2|s_{k};\theta^2))}{\partial \theta^2}^\top  Q(s_k,a_{k+1}^1,a_{k+1}^2;\theta^1,\theta^2) \ \bigg] \Bigg] \nonumber\\
% + \mathbb{E}_{a_0^1}\mathbb{E}_{a_1^2} \mathbb{E}_{s_{T1}} \ \Biggl[ \mathbb{E}_{a_1^1}\mathbb{E}_{a_1^2} &\mathbb{E}_{s_{T2}} ...  \biggl[ \sum_{k=1}^{\infty} \ \gamma^k \frac{\partial \log(\pi(a_{k+1}^1|s_{k};\theta^1))}{\partial \theta^1} \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i+1}^2|s_i;\theta^2))}{\partial \theta^2}^\top  Q(s_k,a_{k+1}^1,a_{k+1}^2;\theta^1,\theta^2) \ \bigg] \Bigg] \nonumber
% \end{align}}
% \end{theorem}

\textit{Proof:} By definition we know that $D_{\theta^1 \theta^2} V(s_0;\theta^1,\theta^2) = D_{\theta^1}(D_{\theta^2} V(s_0;\theta^1,\theta^2))$. Thus we can use $D_{\theta^2} V(s_0;\theta^1,\theta^2)$ as defined in \eq~\ref{eqn: gradv} and differentiating with respect to $\theta^1$, thereby we get,
\begin{align}
D_{\theta^1 \theta^2} V(s_0;\theta^1,\theta^2) &= \int_{a_0^1} \int_{a_0^2} \frac{\partial \pi(a_0^1|s_0;\theta^1)}{\partial \theta^1} \  \frac{\partial \pi(a_0^2|s_0;\theta^2)}{\partial \theta^2}^\top \ Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2) \ da_0^1 \ da_0^2 \nonumber\\
&+ \int_{a_0^1} \int_{a_0^2} \frac{\partial \pi(a_0^1|s_0;\theta^1)}{\partial \theta^1} \  \pi(a_0^2|s_0;\theta^2) \ \frac{\partial Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2)}{\partial \theta^2}^\top \ da_0^1 \ da_0^2 \nonumber\\
&+ \int_{a_0^1} \int_{a_0^2}  \pi(a_0^1|s_0;\theta^1) \  \frac{\partial Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2)} {\partial \theta^1} \ \frac{\partial \pi(a_0^2|s_0;\theta^2)}{\partial \theta^2}^\top \ da_0^1 \ da_0^2 \nonumber\\
&+ \int_{a_0^1} \int_{a_0^2}  \pi(a_0^1|s_0;\theta^1) \  \pi(a_0^2|s_0;\theta^2) \ \frac{\partial^2 Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2)} {\partial \theta^1 \partial \theta^2} \ da_0^1 \ da_0^2 \label{eqn: doublegradv}
\end{align}
% Since, the reward $r(s_0,a_0^1,a_0^2)$ does not depend on the players policies parameters. The bilinear derivative of state-action value $Q$, in the \eq \eqref{eqn: doublegradv}, can be obtained as follows. First, we know by Definition \ref{def:ValueDef} that $Q(s_0,a_1^1,a_1^2;\theta^1,\theta^2) = r(s_0,a_1^1,a_1^2) +  \gamma \int_{s1} T(s_1|s_0;a_1^1,a_1^2) \  V(s_1;\theta^1,\theta^2) \ ds_1$. Thus $D_{\theta^1 \theta^2} Q(s_0,a_1^1,a_1^2;\theta^1,\theta^2)$ can be obtained as follows,
% \begin{gather*}
% % D_{\theta^2} Q(s_0,a_1^1,a_1^2;\theta^1,\theta^2) = \gamma \int_{s1}  T(s_1|s_0;a_1^1,a_1^2) \  \frac{\partial V(s_1;\theta^1,\theta^2)}{\partial \theta^2} \ ds_1\\
% D_{\theta^1 \theta^2} Q(s_0,a_1^1,a_1^2;\theta^1,\theta^2) = \gamma \int_{s1}  T(s_1|s_0;a_1^1,a_1^2) \  \frac{\partial^2 V(s_1;\theta^1,\theta^2)}{\partial \theta^1 \partial \theta^2} \ ds_1 \numberthis \label{eqn: doublegradq}
% \end{gather*}
% We can plug \eq~\ref{eqn: doublegradq} into \eq~\ref{eqn: doublegradv}, which results in,
% \begin{gather*}
% D_{\theta^1 \theta^2} V(s_0;\theta^1,\theta^2) = \int_{a_1^1} \int_{a_1^2} \frac{\partial \pi(a_1^1|s_0;\theta^1)}{\partial \theta^1} \  \frac{\partial \pi(a_1^2|s_0;\theta^2)}{\partial \theta^2}^\top \ Q(s_0,a_1^1,a_1^2;\theta^1,\theta^2) \ da_1^1 \ da_1^2 \\
% + \int_{a_1^1} \int_{a_1^2} \frac{\partial \pi(a_1^1|s_0;\theta^1)}{\partial \theta^1} \  \pi(a_1^2|s_0;\theta^2) \ \frac{\partial Q(s_0,a_1^1,a_1^2;\theta^1,\theta^2)}{\partial \theta^2}^\top \ da_1^1 \ da_1^2 \\
% + \int_{a_1^1} \int_{a_1^2}  \pi(a_1^1|s_0;\theta^1) \  \frac{\partial Q(s_0,a_1^1,a_1^2;\theta^1,\theta^2)} {\partial \theta^1} \ \frac{\partial \pi(a_1^2|s_0;\theta^2)}{\partial \theta^2}^\top \ da_1^1 \ da_1^2 \\
% + \int_{a_1^1} \int_{a_1^2}  \pi(a_1^1|s_0;\theta^1) \  \pi(a_1^2|s_0;\theta^2) \ \biggl( \gamma \int_{s1} T(s_1|s_0;a_1^1,a_1^2) \  \frac{\partial^2 V(s_1;\theta^1,\theta^2)}{\partial \theta^1 \partial \theta^2} \ ds_1 \biggr)\ da_1^1 \ da_1^2 \numberthis \label{eqn: recursive_double_gradv}
% \end{gather*}
Let's define some short hand notations, the first term in \eq~\ref{eqn: doublegradv} be $b_0$, second term be $c_0$, third term be $d_0$, forth term as $e_0$ and $Pr_0 = Pr(s_0\rightarrow s_1, 1, \theta^1,\theta^2)$ where subscript zero represents step index. Exploiting recursive structure of $D_{\theta^1 \theta^2} V(s_0;\theta^1,\theta^2)$, we can evaluate $D_{\theta^1 \theta^2} V(s_1;\theta^1,\theta^2)$ and substitute it back in \eq~\ref{eqn: doublegradv},we get
{\makeatletter\def\f@size{10}\check@mathfonts\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}
\begin{align}\label{eqn: subs_double_gradv}
D_{\theta^1 \theta^2} V(s_0;\theta^1,\theta^2) &= \int_{a_0^1} \int_{a_0^2} \frac{\partial \pi(a_0^1|s_0;\theta^1)}{\partial \theta^1} \ \frac{\partial \pi(a_0^2|s_0;\theta^2)}{\partial \theta^2}^\top \ Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2) \ da_0^1 \ da_0^2 \nonumber\\
&+ \int_{a_0^1} \int_{a_0^2} \frac{\partial \pi(a_0^1|s_0;\theta^1)}{\partial \theta^1} \  \pi(a_0^2|s_0;\theta^2) \ \frac{\partial Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2)}{\partial \theta^2}^\top \ da_0^1 \ da_0^2 \nonumber\\
&+ \int_{a_0^1} \int_{a_0^2}  \pi(a_0^1|s_0;\theta^1) \  \frac{\partial Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2)} {\partial \theta^1} \ \frac{\partial \pi(a_0^2|s_0;\theta^2)}{\partial \theta^2}^\top \ da_0^1 \ da_0^2 \nonumber\\
+ \int_{a_0^1} \int_{a_0^2}  \pi(a_0^1|s_0;\theta^1) \ & \pi(a_0^2|s_0;\theta^2) \ \Biggl( \gamma \int_{s1} T(s_1|s_0,a_0^1,a_0^2) \ \biggl( \int_{a_1^1} \int_{a_1^2} \frac{\partial \pi(a_1^1|s_1;\theta^1)}{\partial \theta^1} \ \frac{\partial \pi(a_1^2|s_1;\theta^2)}{\partial \theta^2}^\top \ Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2) \ da_1^1 \ da_1^2 \nonumber\\
&+ \int_{a_1^1} \int_{a_1^2} \frac{\partial \pi(a_1^1|s_1;\theta^1)}{\partial \theta^1} \  \pi(a_1^2|s_1;\theta^2) \ \frac{\partial Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2)}{\partial \theta^2}^\top \ da_1^1 \ da_1^2 \nonumber\\
&+ \int_{a_1^1} \int_{a_1^2}  \pi(a_1^1|s_1;\theta^1) \  \frac{\partial Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2)} {\partial \theta^1} \ \frac{\partial \pi(a_1^2|s_1;\theta^2)}{\partial \theta^2}^\top \ da_1^1 \ da_1^2 \nonumber\\
&+ \int_{a_1^1} \int_{a_1^2}  \pi(a_1^1|s_1;\theta^1) \  \pi(a_1^2|s_1;\theta^2) \ \bigl( \gamma \int_{s2} T(s_2|s_1,a_1^1,a_1^2) \  \frac{\partial^2 V(s_2;\theta^1,\theta^2)}{\partial \theta^2 \partial \theta^1} \ ds_2 \bigr)\ da_1^1 \ da_1^2 \biggr) \ ds_1 \Biggr)\ da_0^1 \ da_0^2 
\end{align}}
Note that in short term notations, the 4th term $e_0$ is expanded to, $e_0 = \gamma \int_{s1} Pr_0 ( b_1 + c_1 + d_1 + e_1) ds_1$. Using this one can write,
\begin{align}
D_{\theta^1 \theta^2} V(s_0;\theta^1,\theta^2) &= b_0 + c_0 + d_0 
+ \gamma \int_{s1}Pr_0 \Bigl(b_1 + c_1 + d_1 
+ \gamma \int_{s2}Pr_1 \Bigl(b_2 + c_2 + d_2 \nonumber\\
&+ \gamma \int_{s3}Pr_2 \Bigl(b_3 + c_3 + d_3 
+ \gamma \int_{s4}Pr_3 \Bigl(...\Bigr)ds_4\Bigr)ds_3\Bigr)ds_2\Bigr)ds_1 \nonumber\\
& = b_0 + \gamma \int_{s1}Pr_0 \Bigl(b_1 + \gamma \int_{s2}Pr_1 \Bigl(b_2 + \gamma \int_{s3}Pr_2 \Bigl(b_3 + \gamma \int_{s4}Pr_3 \Bigl(...\Bigr)ds_4\Bigr)ds_3\Bigr)ds_2\Bigr)ds_1 \nonumber\\
& + c_0 + \gamma \int_{s1}Pr_0 \Bigl(c_1 + \gamma \int_{s2}Pr_1 \Bigl(c_2 + \gamma \int_{s3}Pr_2 \Bigl(c_3 + \gamma \int_{s4}Pr_3 \Bigl(...\Bigr)ds_4\Bigr)ds_3\Bigr)ds_2\Bigr)ds_1 \nonumber\\
& + d_0 + \gamma \int_{s1}Pr_0 \Bigl(d_1 + \gamma \int_{s2}Pr_1 \Bigl(d_2 + \gamma \int_{s3}Pr_2 \Bigl(d_3 + \gamma \int_{s4}Pr_3 \Bigl(...\Bigr)ds_4\Bigr)ds_3\Bigr)ds_2\Bigr)ds_1 \nonumber
\end{align}
{\makeatletter\def\f@size{10}\check@mathfonts\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}
\begin{align}
D_{\theta^1 \theta^2} \eta(\theta^1,\theta^2) &= \int_{s_0} p(s_0) D_{\theta^1 \theta^2} V(s_0;\theta^1,\theta^2) ds_0 \nonumber\\
& = \int_{s_0} p(s_0) \Bigl[b_0 + \gamma \int_{s1}Pr_0 \Bigl(b_1 + \gamma \int_{s2}Pr_1 \Bigl(b_2 + \gamma \int_{s3}Pr_2 \Bigl(b_3 + \gamma \int_{s4}Pr_3 \Bigl(...\Bigr)ds_4\Bigr)ds_3\Bigr)ds_2\Bigr)ds_1\Bigr]ds_0\label{eqn: term1}\\
& + \int_{s_0} p(s_0)\Bigl[ c_0 + \gamma \int_{s1}Pr_0 \Bigl(c_1 + \gamma \int_{s2}Pr_1 \Bigl(c_2 + \gamma \int_{s3}Pr_2 \Bigl(c_3 + \gamma \int_{s4}Pr_3 \Bigl(...\Bigr)ds_4\Bigr)ds_3\Bigr)ds_2\Bigr)ds_1 \Bigr]ds_0\label{eqn: term2}\\
& + \int_{s_0} p(s_0)\Bigl[d_0 + \gamma \int_{s1}Pr_0 \Bigl(d_1 + \gamma \int_{s2}Pr_1 \Bigl(d_2 + \gamma \int_{s3}Pr_2 \Bigl(d_3 + \gamma \int_{s4}Pr_3 \Bigl(...\Bigr)ds_4\Bigr)ds_3\Bigr)ds_2\Bigr)ds_1\Bigr]ds_0 \label{eqn: term3}
\end{align}}
Let~\ref{eqn: term1} be \textit{term\_b},~\ref{eqn: term2} be \textit{term\_c}  and~\ref{eqn: term3} be \textit{term\_d}. Hence, $D_{\theta^1 \theta^2} V(s_0;\theta^1,\theta^2) = term\_b + term\_c + term\_d$.
We tackle each part of separately.
% Even thought this equation is similar to \eq~\ref{eqn: gradv}, for this proof we use a different technique. More precisely we tackle each part of \eq~\ref{eqn: doublegradv} separately. Therefore, we introduce the following notation to name the different parts, 

% Note that similar to \eq \eqref{eqn: recursive_gradv}, we can exploit the recursive structure of \eq \eqref{eqn: doublegradv}. However, since in this case the number of terms quickly gets out of hands, we divide the unrolling and marginalization part into three parts, one for each term in \eq~\ref{eqn: doublegradv}. To name the different parts, we introduce the notation \textbf{$a1b2$} where $(a, b) \in \{\pi^1, \pi^2, V, Q\}$ and $(1,2)$ refers to the derivatives with respect to $\theta^1$ and  $\theta^2$, e.g., $\pi^1 1 \pi^2 2$ refers to the first term in \eq~\ref{eqn: doublegradv}. 

% But here, the number of terms will quickly explode, so will divide proof in 3 parts corresponding to each term. Let's follow the notation \textbf{$a1b2$} denotes term containing gradient of $a$ with respect to $\theta^1$ and $b$ with respect to $\theta^2$, here $(a, b) \in \{\pi^1, \pi^2, V, Q\}$. 
%%%%%
% \manish{Ask about f notation}
% \begin{gather}
%     Pr(s_0\rightarrow s_1,\theta^1,\theta^2) = \int_{a^1_0} \int_{a^2_0} \pi(a_0^1|s_0;\theta^1) \  \pi(a_0^2|s_0;\theta^2) T(s_1|s_0;a^1_0,a^2_0) da^1_0 da^2_0\\ 
%     f(\tau_1,s1;\theta^1,\theta^2) = \int_{s_0} p(s_0) \int_{a^1_0}\int_{a^2_0} \pi(a_0^1|s_0;\theta^1) \  \pi(a_0^2|s_0;\theta^2) T(s_1|s_0, a^1_0,a^2_0) da^1_0 da^2_0 ds_0\\
%     f(\tau_1;\theta^1,\theta^2) = \Biggl[\int_{s_0} p(s_0) \int_{a^1_0}\int_{a^2_0} \pi(a_0^1|s_0;\theta^1) \  \pi(a_0^2|s_0;\theta^2) T(s_1|s_0, a^1_0,a^2_0) da^1_0 da^2_0 ds_0\Biggr]\pi(a_1^1|s_1;\theta^1) \pi(a_1^2|s_1;\theta^2)
% \end{gather}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Solving for the \textit{term\_b}:}
\vspace{\baselineskip}
\noindent\textbf{Solving for the \textit{term\_b}:}\\
\vspace{\baselineskip}
In term\_b in line ~\ref{eqn: term1}, on substituting value of $b_0$ and $b_1$ we get,
% \begin{gather*}
% \pi^11\pi^22 + q1q2 =\int_{a_1^1} \int_{a_1^2} \frac{\partial \pi(a_1^1|s_0;\theta^1)}{\partial \theta^1} \ \frac{\partial \pi(a_1^2|s_0;\theta^2)}{\partial \theta^2}^\top \ Q(s_0,a_1^1,a_1^2;\theta^1,\theta^2) \ da_1^1 \ da_1^2 \\
% + \int_{a_1^1} \int_{a_1^2}  \pi(a_1^1|s_0;\theta^1) \ \pi(a_1^2|s_0;\theta^2) \ \frac{\partial^2 Q(s_0,a_1^1,a_1^2;\theta^1,\theta^2)} {\partial \theta^1 \partial \theta^2} \ da_1^1 \ da_1^2 \numberthis\\
% \end{gather*}
% The hessian term v1v2 in \eq \eqref{eqn: doublegradv} for any state $s_i$ will unfold to 3 terms upon utilising recursive structure of \eq \eqref{eqn: doublegradv}. As far simplification of term 1 p1p2 is considered, we will only focus on terms corresponding to p1p2 after unrolling of v1v2 term. The p1q2 and q1p2 unrolled terms will be combined with term 2 and term 3 of \eq \eqref{eqn: doublegradv} later in~\ref{appx: term2} and~\ref{appx: term3} respectively.    
\begin{align}
term\_b &= \int_{s_0} p(s_0) \Biggl[\int_{a_0^1} \int_{a_0^2} \frac{\partial \pi(a_0^1|s_0;\theta^1)}{\partial \theta^1} \ \frac{\partial \pi(a_0^2|s_0;\theta^2)}{\partial \theta^2}^\top \ Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2) \ da_0^1 \ da_0^2 \nonumber\\
&+ \gamma \int_{s_1} Pr(s_1|s_0;\theta^1,\theta^2)\ \Biggl( \int_{a_1^1} \int_{a_1^2} \frac{\partial \pi(a_1^1|s_1;\theta^1)}{\partial \theta^1} \ \frac{\partial \pi(a_1^2|s_1;\theta^2)}{\partial \theta^2}^\top \  Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2) \ da_1^1 \ da_1^2 \nonumber\\
&+ \int_{a_1^1} \int_{a_1^2}  \pi(a_1^1|s_1;\theta^1) \ \pi(a_1^2|s_1;\theta^2) \ \gamma \int_{s2} T(s_2|s_1,a_1^1,a_1^2) \ \biggl(...\biggr) \ ds_2\ da_1^1 \ da_1^2  \Biggr)\ ds_1 \ da_0^1 \ da_0^2\Biggr] ds_0\numberthis
\end{align}
Similar to \eq~\ref{eqn: Val_Unrolled2steps} on unrolling and marginalising, we can write in compact form as, 
\begin{align} \label{eqn: summed_gradv}
term\_b &= \int_{\tau} \sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0:k-1},s_k;\theta^1,\theta^2) \int_{a_k^1} \int_{a_k^2} \frac{\partial \pi(a_k^1|s_k;\theta^1)}{\partial \theta^1} \ \frac{\partial \pi(a_k^2|s_k;\theta^2)}{\partial \theta^2}^\top \ Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2) \ da_k^1 \ da_k^2 d\tau \nonumber\\
&=\int_{\tau} \sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0:k};\theta^1,\theta^2) \frac{\partial \log(\pi(a_k^1|s_k;\theta^1))}{\partial \theta^1} \ \frac{\partial \log(\pi(a_k^2|s_k;\theta^2))}{\partial \theta^2}^\top \ Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2) \ d\tau 
\end{align}

% \subsubsection{Solving for the second term\_c}
\vspace{\baselineskip}
\noindent\textbf{Solving for the \textit{term\_c}:}\\
\vspace{\baselineskip}
% \label{appx: term2}
In \textit{term\_c} on line ~\ref{eqn: term2}, with substituting value of $c_0$ and $c_1$ we get,
% \begin{gather*}
%  term\_c = \int_{s_0} p(s_0) \Biggl[ \int_{a_1^1} \int_{a_1^2} \frac{\partial \pi(a_1^1|s_0;\theta^1)}{\partial \theta^1} \ \pi(a_1^2|s_0;\theta^2) \ \frac{\partial Q(s_0,a_1^1,a_1^2;\theta^1,\theta^2)}{\partial \theta^2}^\top \ da_1^1 \ da_1^2 \\ 
%  + \int_{a_1^1} \int_{a_1^2}  \pi(a_1^1|s_0;\theta^1) \  \pi(a_1^2|s_0;\theta^2) \ \frac{\partial^2 Q(s_0,a_1^1,a_1^2;\theta^1,\theta^2)} {\partial \theta^1 \partial \theta^2} \ da_1^1 \ da_1^2 \Biggr] \numberthis \label{eqn: term2_4}
%  \end{gather*}
%  In this part, we will try to club together terms containing $\frac{\partial Q}{\partial \theta^2}$. Upon unrolling of the fourth term q1q2 in \eq \eqref{eqn: term2_4}, we get 
{\makeatletter\def\f@size{9.5}\check@mathfonts\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}
\begin{align}
term\_c &= \int_{s_0} p(s_0) \Biggl[ \int_{a_0^1} \int_{a_0^2} \frac{\partial \pi(a_0^1|s_0;\theta^1)}{\partial \theta^1} \ \pi(a_0^2|s_0;\theta^2) \ \frac{\partial Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2)}{\partial \theta^2}^\top \ da_0^1 \ da_0^2 \nonumber\\
&+ \int_{a_0^1} \int_{a_0^2} \pi(a_0^1|s_0;\theta^1)  \pi(a_0^2|s_0;\theta^2) \ \gamma \int_{s1} T(s_1|s_0,a_0^1,a_0^2)
\biggl( \int_{a_1^1} \int_{a_1^2} \frac{\partial \pi(a_1^1|s_1;\theta^1)}{\partial \theta^1} \pi(a_1^2|s_1;\theta^2) \frac{\partial Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2)}{\partial \theta^2}^\top  da_1^1 \ da_1^2 \nonumber\\
&+ \int_{a_1^1} \int_{a_1^2}  \pi(a_1^1|s_1;\theta^1) \  \pi(a_1^2|s_1;\theta^2) \ \gamma \int_{s2} T(s_2|s_1,a_1^1,a_1^2) \Bigl(...\Bigr)ds_2\ da_1^1 \ da_1^2  \biggr)ds_1\ da_0^1 \ da_0^2 \Biggr] ds_0  \label{eqn: term2_unrolling}
\end{align}}
Note that \textit{term\_c} contains $\frac{\partial Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2)}{\partial \theta^2}$. On unfolding it using \eq~\ref{eqn: gradq} and \eq~\ref{eqn: recursive_gradv}, upto state $s_1$ we get:
{\makeatletter\def\f@size{9.5}\check@mathfonts\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}
\begin{align}
term\_c &= \int_{s_0} p(s_0) \Biggl[ \int_{a_0^1} \int_{a_0^2} \frac{\partial \pi(a_0^1|s_0;\theta^1)}{\partial \theta^1} \ \pi(a_0^2|s_0;\theta^2) \ \biggl[ \int_{s1} \gamma \ T(s_1|s_0,a_0^1,a_0^2) \biggl(
\int_{a_1^1} \int_{a_1^2} \ \pi(a_1^1|s_1;\theta^1) \ \frac{\partial \pi(a_1^2|s_1;\theta^2)}{\partial \theta^2} \nonumber\\ 
& \ Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2) \ da_1^1 \ da_1^2 \
+ \int_{a_1^1} \int_{a_1^2}  \pi(a_1^1|s_1;\theta^1) \  \pi(a_1^2|s_1;\theta^2) \ \frac{\partial Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2)}{\partial \theta^2} \ da_1^1 \ da_1^2 \biggl)^\top ds_1 \biggr] \ da_0^1 \ da_0^2 \nonumber\\
&+ \int_{a_0^1} \int_{a_0^2} \pi(a_0^1|s_0;\theta^1) \  \pi(a_0^2|s_0;\theta^2) \ \biggl[ \gamma \int_{s1} T(s_1|s_0,a_0^1,a_0^2) 
\biggl( \int_{a_1^1} \int_{a_1^2} \frac{\partial \pi(a_1^1|s_1;\theta^1)}{\partial \theta^1} \pi(a_1^2|s_1;\theta^2) \ \frac{\partial Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2)}{\partial \theta^2}^\top \ da_1^1 \ da_1^2 \nonumber \\
&+ \int_{a_1^1} \int_{a_1^2}  \pi(a_1^1|s_1;\theta^1) \  \pi(a_1^2|s_1;\theta^2) \ \gamma \int_{s2} T(s_2|s_1,a_1^1,a_1^2) \Bigl(...\Bigr) \ ds_2 \ da_1^1 \ da_1^2 \biggr) ds_1 \biggr] \ da_0^1 \ da_0^2 \Biggr] ds_0  \nonumber
\end{align}}
Using log trick ($D_{\theta} \log p_{\theta}(\tau) = \frac{D_{\theta} p_{\theta}(\tau)}{p_{\theta}(\tau)}$) and combining terms together, we get:
{\makeatletter\def\f@size{10}\check@mathfonts\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}
\begin{align}
term\_c &= \int_{s_0} p(s_0) \Biggl[ \int_{a_0^1} \int_{a_0^2} \pi(a_0^1|s_0;\theta^1) \ \pi(a_0^2|s_0;\theta^2) \ \biggl[ \int_{s1} \gamma \ T(s_1|s_0,a_0^1,a_0^2) \Biggl(
\int_{a_1^1} \int_{a_1^2} \ \pi(a_1^1|s_1;\theta^1) \ \pi(a_1^2|s_1;\theta^2)\nonumber\\
&\biggl[ \frac{\partial \log(\pi(a_0^1|s_0;\theta^1))}{\partial \theta^1} \frac{\partial \log(\pi(a_1^2|s_1;\theta^2))}{\partial \theta^2}^\top \ Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2) + \biggl( \frac{\partial \log(\pi(a_0^1|s_0;\theta^1))}{\partial \theta^1} + \frac{\partial \log(\pi(a_1^1|s_1;\theta^1))}{\partial \theta^1} \biggr)\nonumber\\
&\frac{\partial Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2)}{\partial \theta^2}^\top \ + \gamma \int_{s2} T(s_2|s_1,a_1^1,a_1^2) \Bigl(...\Bigr)\ ds_2 \ \biggr] \ da_1^1 \ da_1^2 \Biggr) ds_1 \biggr] \ da_0^1 \ da_0^2 \Biggr] ds_0 
\end{align}}
Let's simplify notation, $\int_a p(a)f(a)da = \mathbb{E}_a[f(a)]$ and $s_{T}$ is state transition.
\begin{align}
&= \mathbb{E}_{s_0}\mathbb{E}_{a_0^1}\mathbb{E}_{a_0^2} \mathbb{E}_{s_{T1}} \ \Biggl[ \mathbb{E}_{a_1^1}\mathbb{E}_{a_1^2} \gamma \biggl[ \frac{\partial \log(\pi(a_0^1|s_0;\theta^1))}{\partial \theta^1} \frac{\partial \log(\pi(a_1^2|s_1;\theta^2))}{\partial \theta^2}^\top \  Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2) \nonumber \\
&+ \biggl( \frac{\partial \log(\pi(a_0^1|s_0;\theta^1))}{\partial \theta^1} + \frac{\partial \log(\pi(a_1^1|s_1;\theta^1))}{\partial \theta^1} \biggr)\ \frac{\partial Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2)}{\partial \theta^2}^\top + \gamma \int_{s2} T(s_2|s_1,a_1^1,a_1^2) \Bigl(...\Bigr) ds_2 \biggr] \ \Biggr] 
\end{align}
$\Bigl(...\Bigr)$ will have terms of the form $\frac{\partial Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2)}{\partial \theta^2}$, which is added to similar term obtained after 1 step unrolling of $\frac{\partial Q(s_{k-1},a_{k-1}^1,a_{k-1}^2;\theta^1,\theta^2)}{\partial \theta^2}$. The equation below shows one step unrolling of $\frac{\partial Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2)}{\partial \theta^2}$,
\manish{This term also need $E_{a^2} terms$}
\manish{Change the notations to f($\tau_{0:k}$), remember to put it in 0:k just whole with $\tau$ is wrong, because of transition probablity}
\begin{gather*}
= \mathbb{E}_{s_0}\mathbb{E}_{a_0^1}\mathbb{E}_{a_0^2} \mathbb{E}_{s_{T1}} \ \Biggl[ \mathbb{E}_{a_1^1}\mathbb{E}_{a_1^2} \mathbb{E}_{s_{T2}} \biggl[ \frac{\partial \log(\pi(a_0^1|s_0;\theta^1))}{\partial \theta^1} \frac{\partial \log(\pi(a_1^2|s_1;\theta^2))}{\partial \theta^2}^\top \ \gamma \ Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2) \ \\
+ \biggl( \frac{\partial \log(\pi(a_0^1|s_0;\theta^1))}{\partial \theta^1} + \frac{\partial \log(\pi(a_1^1|s_1;\theta^1))}{\partial \theta^1} \ \biggr)\ \frac{\partial \log(\pi(a_2^2|s_2;\theta^2))}{\partial \theta^2}^\top \ \gamma^2 \ Q(s_2,a_2^1,a_2^2;\theta^1,\theta^2)\\
+ \biggl( \frac{\partial \log(\pi(a_0^1|s_0;\theta^1))}{\partial \theta^1} + \frac{\partial \log(\pi(a_1^1|s_1;\theta^1))}{\partial \theta^1} + \frac{\partial \log(\pi(a_2^1|s_2;\theta^1))}{\partial \theta^1} \biggr)\ \frac{\partial Q(s_2,a_2^1,a_2^2;\theta^1,\theta^2)}{\partial \theta^2}^\top + \Bigl(...\Bigr)\biggr] \ \Biggr] \numberthis
\end{gather*}
Observe the trend, on keep unrolling for $|\tau|$ steps we get,
\begin{align}
&= \mathbb{E}_{s_0}\mathbb{E}_{a_0^1}\mathbb{E}_{a_0^2} \mathbb{E}_{s_{T1}} \ \Biggl[ \mathbb{E}_{a_1^1}\mathbb{E}_{a_1^2} \mathbb{E}_{s_{T2}} ... \biggl[ \sum_{k=1}^{|\tau|-1} \ \gamma^k \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i}^1|s_i;\theta^1))}{\partial \theta^1} \frac{\partial \log(\pi(a_{k}^2|s_{k};\theta^2))}{\partial \theta^2}^\top \ Q(s_k,a_{k}^1,a_{k}^2;\theta^1,\theta^2) \ \bigg] \Bigg] \nonumber\\
&= \mathbb{E}_{f(\cdot;\theta^1,\theta^2)} \ \biggl[ \sum_{k=1}^{|\tau|-1} \ \gamma^k \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i}^1|s_i;\theta^1))}{\partial \theta^1} \frac{\partial \log(\pi(a_{k}^2|s_{k};\theta^2))}{\partial \theta^2}^\top \ Q(s_k,a_{k}^1,a_{k}^2;\theta^1,\theta^2) \ \biggr] 
\end{align}


% \subsubsection{Solving for the second term\_d}
\vspace{\baselineskip}
\noindent\textbf{Solving for the \textit{term\_d}:}\\
\vspace{\baselineskip}
% \label{appx: term3}
In \textit{term\_d} on line ~\ref{eqn: term3}, with substituting value of $d_0$ and $d_1$ we get,
{\makeatletter\def\f@size{9.5}\check@mathfonts\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}
\begin{align}
term\_d &= \int_{s_0} p(s_0) \Biggl[  \int_{a_0^1} \int_{a_0^2}  \pi(a_0^1|s_0;\theta^1) \ \frac{\partial Q(s_0,a_0^1,a_0^2;\theta^1,\theta^2)} {\partial \theta^1} \ \frac{\partial \pi(a_0^2|s_0;\theta^2)}{\partial \theta^2}^\top \ da_0^1 \ da_0^2 \nonumber\\ 
&+ \int_{a_0^1} \int_{a_0^2} \pi(a_0^1|s_0;\theta^1) \ \pi(a_0^2|s_0;\theta^2) \ \gamma \int_{s1} T(s_1|s_0;a_0^1,a_0^2)
\biggl(\int_{a_1^1} \int_{a_1^2}  \pi(a_1^1|s_1;\theta^1) \ \frac{\partial Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2)} {\partial \theta^1} \ \frac{\partial \pi(a_1^2|s_1;\theta^2)}{\partial \theta^2}^\top da_1^1 \ da_1^2 \nonumber\\
&+ \int_{a_0^1} \int_{a_0^2}  \pi(a_1^1|s_1;\theta^1) \  \pi(a_1^2|s_1;\theta^2) \ \frac{\partial^2 Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2)} {\partial \theta^1 \partial \theta^2} da_1^1 \ da_1^2 \biggr) ds_1 \ da_0^1 \ da_0^2\Biggr] ds_0  \label{eqn: term3_unrolling}
\end{align}}
Note that \textit{term\_d} contains $\frac{\partial Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2)}{\partial \theta^1}$. On unfolding it using \eq~\ref{eqn: gradq} and \eq~\ref{eqn: recursive_gradv}, upto state $s_1$ we get:
{\makeatletter\def\f@size{9.5}\check@mathfonts\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}
\begin{align}
term\_d &= \int_{s_0} p(s_0) \Biggl[ \int_{a_0^1} \int_{a_0^2} \pi(a_0^1|s_0;\theta^1)\ \biggl[ \int_{s1} \gamma \ T(s_1|s_0;a_0^1,a_0^2) \Biggl(
\int_{a_1^1} \int_{a_1^2} \ \frac{\partial \pi(a_1^1|s_1;\theta^1)}{\partial \theta^1} \ \pi(a_1^2|s_1;\theta^2) Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2) \ da_1^1 \ da_1^2 \nonumber\\
&+ \int_{a_1^1} \int_{a_1^2}  \pi(a_1^1|s_1;\theta^1) \
\pi(a_1^2|s_1;\theta^2) \ \frac{\partial Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2)}{\partial \theta^1} \ da_1^1 \ da_1^2 \biggl) ds_1 \biggr] \frac{\partial \pi(a_0^2|s_0;\theta^2)}{\partial \theta^2}^\top \ da_0^1 \ da_0^2 \nonumber\\
&+ \int_{a_0^1} \int_{a_0^2} \pi(a_0^1|s_0;\theta^1) \  \pi(a_0^2|s_0;\theta^2) \ \biggl[ \gamma \int_{s1} T(s_1|s_0;a_0^1,a_0^2) \biggl( \int_{a_1^1} \int_{a_1^2}  \pi(a_1^1|s_1;\theta^1) \frac{\partial Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2)} {\partial \theta^1} \ \frac{\partial \pi(a_1^2|s_1;\theta^2)}{\partial \theta^2}^\top \ da_1^1 \ da_1^2 \nonumber\\
&+ \int_{a_1^1} \int_{a_1^2}  \pi(a_1^1|s_1;\theta^1) \  \pi(a_1^2|s_1;\theta^2) \ \gamma \int_{s2} T(s_2|s_1,a_1^1,a_1^2) \Bigl(...\Bigr) \ ds_2 \ da_1^1 \ da_1^2 \biggr) ds_1 \biggr] \ da_0^1 \ da_0^2 \Biggr] ds_0  \nonumber
\end{align}}

Using log trick ($D_{\theta} \log p_{\theta}(\tau) = \frac{D_{\theta} p_{\theta}(\tau)}{p_{\theta}(\tau)}$) and combining terms together, we get:

{\makeatletter\def\f@size{10}\check@mathfonts\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}
\begin{align}
term\_d &= \int_{s_0} p(s_0) \Biggl[ \int_{a_0^1} \int_{a_0^2} \pi(a_0^1|s_0;\theta^1) \ \pi(a_0^2|s_0;\theta^2) \ \Biggl[ \int_{s1} \gamma \ T(s_1|s_0;a_0^1,a_0^2) \Biggl(
\int_{a_1^1} \int_{a_1^2} \ \pi(a_1^1|s_1;\theta^1) \ \pi(a_1^2|s_1;\theta^2) \nonumber\\
&\biggl[ \frac{\partial \log(\pi(a_0^1|s_0;\theta^1))}{\partial \theta^1} \frac{\partial \log(\pi(a_1^2|s_1;\theta^2))}{\partial \theta^2}^\top \  Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2) + \frac{\partial Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2)}{\partial \theta^1} \biggl( \frac{\partial \log(\pi(a_0^2|s_0;\theta^2))}{\partial \theta^2} \nonumber\\
&+ \frac{\partial \log(\pi(a_1^2|s_1;\theta^2))}{\partial \theta^2} \biggr)^\top + \gamma \int_{s2} T(s_2|s_1,a_1^1,a_1^2) \Bigl(...\Bigr)\ ds_2 \ \biggr] \ da_1^1 \ da_1^2 \Biggr) ds_1 \biggr] \ da_0^1 \ da_0^2 \Biggr] ds_0 \nonumber 
\end{align}}
with simplified notations,
\begin{align}
&= \mathbb{E}_{s_0}\mathbb{E}_{a_0^1}\mathbb{E}_{a_0^2} \mathbb{E}_{s_{T1}} \ \Biggl[ \mathbb{E}_{a_1^1}\mathbb{E}_{a_1^2} \gamma \biggl[ \frac{\partial \log(\pi(a_0^1|s_0;\theta^1))}{\partial \theta^1} \frac{\partial \log(\pi(a_1^2|s_1;\theta^2))}{\partial \theta^2}^\top \  Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2) \nonumber \\
&+ \frac{\partial Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2)}{\partial \theta^1} \biggl( \frac{\partial \log(\pi(a_0^2|s_0;\theta^2))}{\partial \theta^2} + \frac{\partial \log(\pi(a_1^2|s_1;\theta^2))}{\partial \theta^2} \biggr)^\top + \gamma \int_{s2} T(s_2|s_1,a_1^1,a_1^2) \Bigl(...\Bigr) ds_2 \biggr] \ \Biggr]
\end{align}
$\Bigl(...\Bigr)$ will have terms of the form $\frac{\partial Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2)}{\partial \theta^1}$, which is added to similar term obtained after 1 step unrolling of $\frac{\partial Q(s_{k-1},a_{k-1}^1,a_{k-1}^2;\theta^1,\theta^2)}{\partial \theta^1}$. The equation below shows one step unrolling of $\frac{\partial Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2)}{\partial \theta^1}$,
\begin{align}
&= \mathbb{E}_{s_0}\mathbb{E}_{a_0^1}\mathbb{E}_{a_0^2} \mathbb{E}_{s_{T1}} \ \Biggl[ \mathbb{E}_{a_1^1}\mathbb{E}_{a_1^2} \mathbb{E}_{s_{T2}} \biggl[ \frac{\partial \log(\pi(a_0^1|s_0;\theta^1))}{\partial \theta^1} \frac{\partial \log(\pi(a_1^2|s_1;\theta^2))}{\partial \theta^2}^\top \ \gamma \ Q(s_1,a_1^1,a_1^2;\theta^1,\theta^2) \ \nonumber \\
&+ \frac{\partial \log(\pi(a_2^1|s_2;\theta^1))}{\partial \theta^1} \ \biggl( \frac{\partial \log(\pi(a_0^2|s_0;\theta^2))}{\partial \theta^2} + \frac{\partial \log(\pi(a_1^2|s_1;\theta^2))}{\partial \theta^2} \ \biggr)^\top \ \gamma^2 \ Q(s_2,a_2^1,a_2^2;\theta^1,\theta^2) \nonumber\\
&+ \frac{\partial Q(s_2,a_2^1,a_2^2;\theta^1,\theta^2)}{\partial \theta^1} \biggl( \frac{\partial \log(\pi(a_0^2|s_0;\theta^2))}{\partial \theta^2} + \frac{\partial \log(\pi(a_1^2|s_1;\theta^2))}{\partial \theta^2} + \frac{\partial \log(\pi(a_2^2|s_2;\theta^2))}{\partial \theta^2} \biggr)^\top + \Bigl(...\Bigr) \biggr] \ \Biggr] \nonumber
\end{align}
Observe the trend and keep unrolling for $|\tau|$ steps we get,
\begin{align}
&= \mathbb{E}_{s_0}\mathbb{E}_{a_1^1}\mathbb{E}_{a_1^2} \mathbb{E}_{s_{T1}} \ \Biggl[ \mathbb{E}_{a_2^1}\mathbb{E}_{a_2^2} \mathbb{E}_{s_{T2}} ... \biggl[ \sum_{k=1}^{|\tau|-1} \ \gamma^k \frac{\partial \log(\pi(a_{k}^1|s_{k};\theta^1))}{\partial \theta^1} \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i}^2|s_i;\theta^2))}{\partial \theta^2}^\top \ Q(s_k,a_{k}^1,a_{k}^2;\theta^1,\theta^2) \ \bigg] \Bigg] \nonumber\\
&= \mathbb{E}_{f(\cdot;\theta^1,\theta^2)} \biggl[ \sum_{k=1}^{|\tau|-1} \ \gamma^k \frac{\partial \log(\pi(a_{k}^1|s_{k};\theta^1))}{\partial \theta^1} \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i}^2|s_i;\theta^2))}{\partial \theta^2}^\top \ Q(s_k,a_{k}^1,a_{k}^2;\theta^1,\theta^2) \ \biggr] 
\end{align}

% \subsubsection{Combining all 3 terms}
\vspace{\baselineskip}
\noindent\textbf{Combining all 3 terms:}\\
\vspace{\baselineskip}
Combining term\_b, term\_c and term\_d derived above we get,
{\makeatletter\def\f@size{10}\check@mathfonts\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}
\begin{align}
D_{\theta^1 \theta^2} \eta(\theta^1,\theta^2) &=\int_{\tau} \sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0:k};\theta^1,\theta^2) \frac{\partial \log(\pi(a_k^1|s_k;\theta^1))}{\partial \theta^1} \ \frac{\partial \log(\pi(a_k^2|s_k;\theta^2))}{\partial \theta^2}^\top \ Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2) d\tau \nonumber \\
& + \mathbb{E}_{f(\cdot;\theta^1,\theta^2)} \biggl[ \sum_{k=1}^{|\tau|-1} \ \gamma^k \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i}^1|s_i;\theta^1))}{\partial \theta^1} \frac{\partial \log(\pi(a_{k}^2|s_{k};\theta^2))}{\partial \theta^2}^\top \ Q(s_k,a_{k}^1,a_{k}^2;\theta^1,\theta^2) \ \biggr] \nonumber\\
&+ \mathbb{E}_{f(\cdot;\theta^1,\theta^2)} \biggl[ \sum_{k=1}^{|\tau|-1} \ \gamma^k \frac{\partial \log(\pi(a_{k}^1|s_{k};\theta^1))}{\partial \theta^1} \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i}^2|s_i;\theta^2))}{\partial \theta^2}^\top \ Q(s_k,a_{k}^1,a_{k}^2;\theta^1,\theta^2) \ \biggr] 
% \label{eqn: bilinear_derivative}
\end{align}}
% Given the game objective in terms of state value pair, we can get bilinear derivative of game object as ,
% \begin{gather*}
%     D_{\theta^2 \theta^1} \eta^1 (\theta^1,\theta^2) = \int_{s_{0}} p(s_{0})  D_{\theta^2 \theta^1} V^1(s_0;\theta^1, \theta^2) ds_{0} \numberthis \label{eq: bilinear_game_derivative}
% \end{gather*}
% Using \eq \eqref{eq: bilinear_game_derivative}, $ d(s) = \sum_0^{\infty} \gamma^k Pr(s_0\rightarrow s,\theta^1,\theta^2)$ and log trick,
% {\makeatletter\def\f@size{9}\check@mathfonts\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}
% \begin{align}
% D_{\theta^1 \theta^2} \eta(\theta^1,\theta^2) = \int_{s_0} p(s_0) \int_{s} d(s) \int_{a_k^1} \int_{a_k^2} \pi(a_k^1|s;\theta^1) \pi(a_k^2|s;\theta^2) \frac{\partial \log(\pi(a_k^1|s;\theta^1))}{\partial \theta^1} \ \frac{\partial \log(\pi(a_k^2|s;\theta^2))}{\partial \theta^2}^\top \ Q(s,a_k^1,a_k^2;\theta^1,\theta^2) \ da_k^1 \ da_k^2 ds ds_0\\
% + \mathbb{E}_{s_0}\mathbb{E}_{a_1^1}\mathbb{E}_{a_1^2} \mathbb{E}_{s_{T1}} \ \Biggl[ \mathbb{E}_{a_2^1}\mathbb{E}_{a_2^2} \mathbb{E}_{s_{T2}} ... \biggl[ \sum_{k=1}^{\infty} \ \gamma^k \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i+1}^1|s_i;\theta^1))}{\partial \theta^1} \frac{\partial \log(\pi(a_{k+1}^2|s_{k};\theta^2))}{\partial \theta^2}^\top \ Q(s_k,a_{k+1}^1,a_{k+1}^2;\theta^1,\theta^2) \ \bigg] \Bigg] \\
% + \mathbb{E}_{s_0}\mathbb{E}_{a_1^1}\mathbb{E}_{a_1^2} \mathbb{E}_{s_{T1}} \ \Biggl[ \mathbb{E}_{a_2^1}\mathbb{E}_{a_2^2} \mathbb{E}_{s_{T2}} ... \biggl[ \sum_{k=1}^{\infty} \ \gamma^k \frac{\partial \log(\pi(a_{k+1}^1|s_{k};\theta^1))}{\partial \theta^1} \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i+1}^2|s_i;\theta^2))}{\partial \theta^2}^\top \ Q(s_k,a_{k+1}^1,a_{k+1}^2;\theta^1,\theta^2) \ \bigg] \Bigg] \numberthis \label{eqn: game_bilinear_all}
% \end{align}}
% With simplified notation,
% \begin{gather*}
% D_{\theta^1 \theta^2} \eta(\theta^1,\theta^2) = \mathbb{E} \biggl[ D_{\theta^1}\log(\pi(a_k^1|s;\theta^1))\ D_{\theta^2} \log(\pi(a_k^2|s;\theta^2))^\top \ Q(s,a_k^1,a_k^2;\theta^1,\theta^2) \biggr]\\
% + \mathbb{E} \biggl[ \sum_{k=1}^{\infty} \ \gamma^k \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i+1}^1|s_i;\theta^1))}{\partial \theta^1} \frac{\partial \log(\pi(a_{k+1}^2|s_{k};\theta^2))}{\partial \theta^2}^\top \ Q(s_k,a_{k+1}^1,a_{k+1}^2;\theta^1,\theta^2) \ \bigg] \\
% + \mathbb{E} \biggl[ \sum_{k=1}^{\infty} \ \gamma^k \frac{\partial \log(\pi(a_{k+1}^1|s_{k};\theta^1))}{\partial \theta^1} \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i+1}^2|s_i;\theta^2))}{\partial \theta^2}^\top \ Q(s_k,a_{k+1}^1,a_{k+1}^2;\theta^1,\theta^2) \ \biggr]  \numberthis \label{eqn: game_bilinear_simple}
% \end{gather*}


% In the equation above, 2nd term represents action taken by player 2 on $k^{th}$ time step depending on the action taken by player 1 from start till $(k-1)^{th}$ time step and similarly 3rd term represents action taken by player 1 on $k^{th}$ time step depending on the action taken by player 2 from start till $(k-1)^{th}$ time step. 

\subsection{Generalization of bilinear term to include variants of return}
\label{appx: advantagebilinear}
\subsubsection{Estimating gradient and bilinear term using a baseline}
The \eq~\ref{eq:CPGGradHessianVal1} and \eq~\ref{eq:CPGGradHessianVal} estimates gradient and bilinear term based on $Q(s_k, a^1_k, a^2_k;\theta^1,\theta^2)$ state-action value function. In practice, this can perform poorly due to variance and missing the notion of relative improvement. During learning, policy parameters are updated such that agent visits good trajectories more often and reduce chances of encountering bad trajectories. But for eg, let say good samples have zero reward and bad samples have negative reward. In this case policy distribution will move away from negative sample but can move in any direction as zero doesn't provide information on being better state-action pairs. This causes high variance and slow learning. In another case, suppose that a non zero constant is added to reward function for all states-action pairs, ideally this constant factor should not affect policy update but in the current formulation $Q(s_k, a^1_k,a^2_k;\theta^1,\theta^2)$ it does because the notion of better or worse sample is with respect to zero. Hence missing the notion of relative improvement.

To mitigate the issues, a baseline $b$ can be subtracted from $Q(s, a^1_k, a^2_k;\theta^1,\theta^2)$. The baseline can be any random variable as long as it is not a function of $(a^1_k,a^2_k)$ ~\citep{Sutton2018}. For \MDP, a good baseline $b$ is a function of state $b(s)$, because let say in some states all actions have high values and we need a high baseline to differentiate the higher valued actions from the less highly valued ones; in other states all actions will have low values and a low baseline is appropriate. This is equivalent to $Q(s_k, a^1_k, a^2_k;\theta^1,\theta^2) \xleftarrow{} Q(s, a^1, a^2;\theta^1,\theta^2) - b(s)$ in \eq~\ref{eq:CPGGradHessianVal} and \eq~\ref{eq:CPGGradHessianVal1}.

\subsubsection{Extending \thm~\ref{thm: CPGGradHessianVal} using Advantage function}
A popular choice of baseline $b(s)$ is $V(s,\theta^1,\theta^2)$, which results in advantage function given in \eq~\ref{eqn: AdvDef}. The \thm~\ref{thm: CPGGradHessianAdv} extends \thm~\ref{thm: CPGGradHessianVal} to estimate gradient and bilinear terms using advantage function.
\begin{align}
    A(s_k, a^1_k, a^2_k;\theta^1,\theta^2) = Q(s_k, a^1_k, a^2_k;\theta^1,\theta^2) - V(s_k;\theta^1,\theta^2)
\end{align}

\begin{theorem}\label{thm: CPGGradHessianAdv}
Given \eq~\ref{eqn: AdvDef}, \eq~\ref{eq:CPGGradHessianVal} and \eq~\ref{eq:CPGGradHessianVal1} then  for player $i,j\in\lbrace1,2\rbrace$ and $i \neq j$,
\begin{align}
D_{\theta^i} \eta &=\int_{\tau} \sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0:k};\theta^1,\theta^2) D_{\theta^i} (\log\pi(a_k^i|s_k;\theta^i)) A(s_k,a_k^1,a_k^2;\theta^1,\theta^2) d\tau\label{eq:CPGGradHessianAdv1}\\
\!\! D_{\theta^i \theta^j} \eta &=\!:\!\!\int_{\tau} \!\sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0:k};\theta^1,\theta^2)D_{\theta^i}( \log\pi(a_k^i|s_k;\theta^i)) D_{\theta^j}( \log\pi(a_k^j|s_k;\theta^j))^{\top}  A(s_k,a_k^1,a_k^2;\theta^1,\theta^2) d\tau \nonumber \\
&\!\!\!\!\!\!\!\!\!\!\!+\!\!\! \int_{\tau}\!f(\tau;\theta^1,\theta^2) \sum_{k=1}^{|\tau|-1}\!\!\!\gamma^k D_{\theta^i} (\log \prod_{l=0}^{k-1}\pi(a_{l}^i|s_l;\theta^i)) D_{\theta^j}(\log \pi(a_{k}^j|s_{k};\theta^j))^\top  A(s_k,a_{k}^1,a_{k}^2;\theta^1,\theta^2) d\tau \ \nonumber\\
&\!\!\!\!\!\!\!\!\!\!\!+\!\!\! \int_{\tau}\! f(\tau;\theta^1,\theta^2) \sum_{k=1}^{|\tau|-1}\!\!\!\gamma^k D_{\theta^i} (\log \pi(a_{k}^i|s_{k};\theta^i)) D_{\theta^j} (\log \prod_{l=0}^{k-1}\pi(a_{l}^j|s_l;\theta^j))^\top  A(s_k,a_{k}^1,a_{k}^2;\theta^1,\theta^2) d\tau  \!\!\!\label{eq:CPGGradHessianAdv}
% \label{eqn: bilinear_derivative}
\end{align}
\end{theorem}
\begin{proof} RHS of \eq~\ref{eq:CPGGradHessianAdv1} is, 
\begin{align}
&\int_{\tau} \sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0:k};\theta^1,\theta^2) D_{\theta^i} (\log\pi(a_k^i|s_k;\theta^i)) A(s_k,a_k^1,a_k^2;\theta^1,\theta^2)d\tau \nonumber\\
&= \int_{\tau} \sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0:k};\theta^1,\theta^2) D_{\theta^i} (\log\pi(a_k^i|s_k;\theta^i)) ( Q(s, a^1, a^2;\theta^1,\theta^2) - V(s;\theta^1,\theta^2))d\tau\nonumber\\
&= D_{\theta^i} \eta
- \int_{\tau} \sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0:k};\theta^1,\theta^2) D_{\theta^i} (\log\pi(a_k^i|s_k;\theta^i)) V(s;\theta^1,\theta^2))d\tau\\
&= D_{\theta^i} \eta
- \int_{\tau} \sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0:k-1},s_k;\theta^1,\theta^2) D_{\theta^i} (\pi(a_k^i|s_k;\theta^i)) V(s;\theta^1,\theta^2))d\tau=D_{\theta^i}\eta\\
% &= D_{\theta^i} \eta \;\;\;\;\;\;\;\;\;\;\;\;\;\; \because  D_{\theta^i} (\int_{a_k}\pi(a_k^i|s_k;\theta^i)da_k) = 0
\end{align}
RHS of \eq~\ref{eq:CPGGradHessianAdv},
\begin{align}
&\!\!\!\!\!\!\!\!\!\!\!=\!:\!\!\int_{\tau} \!\sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0:k};\theta^1,\theta^2)D_{\theta^i}( \log\pi(a_k^i|s_k;\theta^i)) D_{\theta^j}( \log\pi(a_k^j|s_k;\theta^j))^{\top}  A(s_k,a_k^1,a_k^2;\theta^1,\theta^2) d\tau \nonumber \\
&\!\!\!\!\!\!\!\!\!\!\!+\!\!\! \int_{\tau}\!f(\tau;\theta^1,\theta^2) \sum_{k=1}^{|\tau|-1}\!\!\!\gamma^k D_{\theta^i} (\log \prod_{l=0}^{k-1}\pi(a_{l}^i|s_l;\theta^i)) D_{\theta^j}(\log \pi(a_{k}^j|s_{k};\theta^j))^\top  A(s_k,a_{k}^1,a_{k}^2;\theta^1,\theta^2) d\tau \ \nonumber\\
&\!\!\!\!\!\!\!\!\!\!\!+\!\!\! \int_{\tau}\! f(\tau;\theta^1,\theta^2) \sum_{k=1}^{|\tau|-1}\!\!\!\gamma^k D_{\theta^i} (\log \pi(a_{k}^i|s_{k};\theta^i)) D_{\theta^j} (\log \prod_{l=0}^{k-1}\pi(a_{l}^j|s_l;\theta^j))^\top  A(s_k,a_{k}^1,a_{k}^2;\theta^1,\theta^2) d\tau  \!\!\! \\
\end{align}{}
\begin{align}
&\!\!\!\!\!\!\!\!\!\!\!=\!:\!\!\int_{\tau} \!\sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0:k};\theta^1,\theta^2)D_{\theta^i}( \log\pi(a_k^i|s_k;\theta^i)) D_{\theta^j}( \log\pi(a_k^j|s_k;\theta^j))^{\top}  (Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2)\!-\! V(s_k;\theta^1,\theta^2)) d\tau \nonumber \\
&\!\!\!\!\!\!\!\!\!\!\!+\!\!\! \int_{\tau}\!f(\tau;\theta^1,\theta^2) \sum_{k=1}^{|\tau|-1}\!\!\!\gamma^k D_{\theta^i} (\log \prod_{l=0}^{k-1}\pi(a_{l}^i|s_l;\theta^i)) D_{\theta^j}(\log \pi(a_{k}^j|s_{k};\theta^j))^\top   (Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2)\!-\! V(s_k;\theta^1,\theta^2)) d\tau \ \nonumber\\
&\!\!\!\!\!\!\!\!\!\!\!+\!\!\! \int_{\tau}\! f(\tau;\theta^1,\theta^2) \sum_{k=1}^{|\tau|-1}\!\!\!\gamma^k D_{\theta^i} (\log \pi(a_{k}^i|s_{k};\theta^i)) D_{\theta^j} (\log \prod_{l=0}^{k-1}\pi(a_{l}^j|s_l;\theta^j))^\top   (Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2)\!-\! V(s_k;\theta^1,\theta^2)) d\tau  \!\!\!
\end{align}
\begin{align}
&\!\!\!\!\!\!\!\!= D_{\theta^i \theta^j} \eta - \!\!\int_{\tau} \!\sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0:k};\theta^1,\theta^2)D_{\theta^i}( \log\pi(a_k^i|s_k;\theta^i)) D_{\theta^j}( \log\pi(a_k^j|s_k;\theta^j))^{\top} V(s_k;\theta^1,\theta^2) d\tau \nonumber \\
&\!\!\!\!\!\!\!\!\!\!-\!\! \int_{\tau}\!f(\tau;\theta^1,\theta^2) \sum_{k=1}^{|\tau|-1}\!\!\!\gamma^k D_{\theta^i} (\log \prod_{l=0}^{k-1}\pi(a_{l}^i|s_l;\theta^i)) D_{\theta^j}(\log \pi(a_{k}^j|s_{k};\theta^j))^\top V(s_k;\theta^1,\theta^2) d\tau \ \nonumber\\
&\!\!\!\!\!\!\!\!\!\!-\!\! \int_{\tau}\! f(\tau;\theta^1,\theta^2) \sum_{k=1}^{|\tau|-1}\!\!\!\gamma^k D_{\theta^i} (\log \pi(a_{k}^i|s_{k};\theta^i)) D_{\theta^j} (\log \prod_{l=0}^{k-1}\pi(a_{l}^j|s_l;\theta^j))^\top V(s_k;\theta^1,\theta^2) d\tau  \!\!\!
\end{align}
\begin{align}
&\!\!\!\!\!\!\!\!= D_{\theta^i \theta^j} \eta - \!\!\int_{\tau} \!\sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0:k-1},s_k;\theta^1,\theta^2)D_{\theta^i}(\pi(a_k^i|s_k;\theta^i)) D_{\theta^j}( \pi(a_k^j|s_k;\theta^j))^{\top} V(s_k;\theta^1,\theta^2) d\tau \nonumber \\
&\!\!\!\!\!\!\!\!\!\!-\!\! \int_{\tau}\! \sum_{k=1}^{|\tau|-1}\!\!\!f(\tau_{0:k-1},s_k, a^i_k;\theta^1,\theta^2)\gamma^k D_{\theta^i} (\log \prod_{l=0}^{k-1}\pi(a_{l}^i|s_l;\theta^i)) D_{\theta^j}( \pi(a_{k}^j|s_{k};\theta^j))^\top V(s_k;\theta^1,\theta^2) d\tau \ \nonumber\\
&\!\!\!\!\!\!\!\!\!\!-\!\! \int_{\tau}\! \sum_{k=1}^{|\tau|-1}\!\!\!f(\tau_{0:k-1},s_k, a^j_k;\theta^1,\theta^2)\gamma^k D_{\theta^i} (\pi(a_{k}^i|s_{k};\theta^i)) D_{\theta^j} (\log \prod_{l=0}^{k-1}\pi(a_{l}^j|s_l;\theta^j))^\top V(s_k;\theta^1,\theta^2) d\tau  \!\!\! \nonumber\\
&\!\!\!\!\!\!\!\!= D_{\theta^i \theta^j} \eta  \;\;\;\;\;\;\;\;\;\;\;\;\;\;
% \because  D_{\theta^i} (\int_{a_k}\pi(a_k^i|s_k;\theta^i)da_k) =  0 , D_{\theta^j} (\int_{a_k}\pi(a_k^j|s_k;\theta^j)da_k) =  0
\end{align}
\end{proof}
% \manish{Ask kamyar how to write sample only s, $a^2$ I am using $f(\cdot;\theta^1,\theta^2)$, is this correct?}
\subsubsection{Approaches to estimate Advantage function}
The other approaches to estimate $A(s_k,a^1_k,a^2_k; \theta^1,\theta^2)$ are, 
Monte Carlo \eq~\ref{eqn: MonteCarloAdv}, 1 step TD residual \eq~\ref{eqn: step1Adv} and t step TD residual \eq~\ref{eqn: steptAdv}.
\begin{align}
    A(s_k,a^1_k,a^2_k; \theta^1,\theta^2) &= \sum_{j=k}^{|\tau|-1} \gamma^{j-k} r(s_j,a^1_j,a^2_j) - V(s_k;\theta^1,\theta^2) \label{eqn: MonteCarloAdv}\\
     A(s_k,a^1_k,a^2_k; \theta^1,\theta^2) &= r(s_k,a^1_k,a^2_k) + \gamma V(s_{k+1};\theta^1,\theta^2) - V(s_k;\theta^1,\theta^2)\label{eqn: step1Adv}\\
     A(s_k,a^1_k,a^2_k; \theta^1,\theta^2) &= r(s_k,a^1_k,a^2_k) + \gamma r(s_{k+1},a^1_{k+1},a^2_{k+1}) +....+ \gamma^{t-1}r(s_{k+t-1},a^1_{k+t-1},a^2_{k+t-1})\nonumber\\ 
     &+ \gamma^t V(s_{k+t};\theta^1,\theta^2) - V(s_k;\theta^1,\theta^2)\label{eqn: steptAdv}
\end{align}{}
The Monte Carlo approach experience high variance in gradient estimation particularly in long trajectories, which may result in slow learning or not learning at all. On the other had 1 step TD residual has huge bias towards initialisation of value function. t-step TD residual can lower this effect upto an extent. To trade between bias and variance we propose to use generalised advantage estimation (\GAE) ~\citep{schulman2015highdimensional}, which is exponentially $\lambda$ weighted average over t-step estimators. It is given by,

\begin{align}
    A^{\GAE}(s_k,a^1_k,a^2_k; \theta^1,\theta^2) &= \sum_{l=0}^{|\tau|-1} (\lambda\gamma)^l\delta^V_{l+k} \nonumber\\
    where, \delta^V_{k} &= r(s_k,a^1_k,a^2_k) + \gamma V(s_{k+1};\theta^1,\theta^2) - V(s_k;\theta^1,\theta^2) \nonumber
\end{align}{}

Note that at $\lambda = 0, \ A^{\GAE}(s_k,a^1_k,a^2_k; \theta^1,\theta^2)$ reduces to 1 step TD residual and at $\lambda = 1$ it is equivalent to Monte Carlo approach to estimate advantage function. We refer interested reader to ~\citep{schulman2015highdimensional} for more information.

Based on the discussion above we propose \alg~\ref{appxalg: cpg}.
% \begin{align}
% &\int_{\tau} \sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0:k};\theta^1,\theta^2) \frac{\partial \log(\pi(a_k^1|s_k;\theta^1))}{\partial \theta^1} \ \frac{\partial \log(\pi(a_k^2|s_k;\theta^2))}{\partial \theta^2}^\top \ A(s_k,a_k^1,a_k^2;\theta^1,\theta^2)d\tau \\
% & + \mathbb{E}_{f(\cdot;\theta^1,\theta^2)} \biggl[ \sum_{k=1}^{|\tau|-1} \ \gamma^k \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i}^1|s_i;\theta^1))}{\partial \theta^1} \frac{\partial \log(\pi(a_{k}^2|s_{k};\theta^2))}{\partial \theta^2}^\top \ (Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2) - b(s_k) ) \ \biggr] \\
% &+ \mathbb{E}_{f(\cdot;\theta^1,\theta^2)} \biggl[ \sum_{k=1}^{|\tau|-1} \ \gamma^k \frac{\partial \log(\pi(a_{k}^1|s_{k};\theta^1))}{\partial \theta^1} \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i}^2|s_i;\theta^2))}{\partial \theta^2}^\top Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2)\biggr] \\
% = &D_{\theta^2\theta^1}\eta - \int_{\tau} \sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0:k};\theta^1,\theta^2) \frac{\partial \log(\pi(a_k^1|s_k;\theta^1))}{\partial \theta^1} \ \frac{\partial \log(\pi(a_k^2|s_k;\theta^2))}{\partial \theta^2}^\top \ (b(s_k) )d\tau \nonumber \\
% & - \mathbb{E}_{f(\cdot;\theta^1,\theta^2)} \biggl[ \sum_{k=1}^{|\tau|-1} \ \gamma^k \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i}^1|s_i;\theta^1))}{\partial \theta^1} \frac{\partial \log(\pi(a_{k}^2|s_{k};\theta^2))}{\partial \theta^2}^\top \ ( b(s_k) ) \ \biggr] \nonumber\\
% &- \mathbb{E}_{f(\cdot;\theta^1,\theta^2)} \biggl[ \sum_{k=1}^{|\tau|-1} \ \gamma^k \frac{\partial \log(\pi(a_{k}^1|s_{k};\theta^1))}{\partial \theta^1} \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i}^2|s_i;\theta^2))}{\partial \theta^2}^\top \ ( b(s_k) ) \ \biggr] \\
% = &D_{\theta^2\theta^1}\eta
% \end{align}{}
% Since summing over actions, $D_{\theta^i} \int_a \pi(a|s,\theta^i)b(s)da = b(s) D_{\theta^i} 1 = 0$ 
% \end{proof}
% The notion of increasing probablity of visiting relatively good rewards and decresing probablity of relatively bad reward is missing in this defination of reward function. 



% put the explainaiton for advantage function and its theorem

% also the discusison of basline

% also GAE

% all three should be there

% and why you are propose ing each

% b(s) to reduce the variance further,

% MC - V is one way to do it

% and advantage is enother way

% then you say, people have obseved combining Q and MC helps and then propse GAE version of it

% then in the exp section, refere to b.3 and say per that discussion you use GAE for the exp










% \begin{align}
% &\int_{\tau} \sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0:k};\theta^1,\theta^2) \frac{\partial \log(\pi(a_k^1|s_k;\theta^1))}{\partial \theta^1} \ \frac{\partial \log(\pi(a_k^2|s_k;\theta^2))}{\partial \theta^2}^\top \ (Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2) - b(s_k) )d\tau \\
% & + \mathbb{E}_{f(\cdot;\theta^1,\theta^2)} \biggl[ \sum_{k=1}^{|\tau|-1} \ \gamma^k \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i}^1|s_i;\theta^1))}{\partial \theta^1} \frac{\partial \log(\pi(a_{k}^2|s_{k};\theta^2))}{\partial \theta^2}^\top \ (Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2) - b(s_k) ) \ \biggr] \\
% &+ \mathbb{E}_{f(\cdot;\theta^1,\theta^2)} \biggl[ \sum_{k=1}^{|\tau|-1} \ \gamma^k \frac{\partial \log(\pi(a_{k}^1|s_{k};\theta^1))}{\partial \theta^1} \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i}^2|s_i;\theta^2))}{\partial \theta^2}^\top \ (Q(s_k,a_k^1,a_k^2;\theta^1,\theta^2) - b(s_k) ) \ \biggr] \\
% = &D_{\theta^2\theta^1}\eta - \int_{\tau} \sum_{k=0}^{|\tau|-1} \gamma^k f(\tau_{0:k};\theta^1,\theta^2) \frac{\partial \log(\pi(a_k^1|s_k;\theta^1))}{\partial \theta^1} \ \frac{\partial \log(\pi(a_k^2|s_k;\theta^2))}{\partial \theta^2}^\top \ (b(s_k) )d\tau \nonumber \\
% & - \mathbb{E}_{f(\cdot;\theta^1,\theta^2)} \biggl[ \sum_{k=1}^{|\tau|-1} \ \gamma^k \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i}^1|s_i;\theta^1))}{\partial \theta^1} \frac{\partial \log(\pi(a_{k}^2|s_{k};\theta^2))}{\partial \theta^2}^\top \ ( b(s_k) ) \ \biggr] \nonumber\\
% &- \mathbb{E}_{f(\cdot;\theta^1,\theta^2)} \biggl[ \sum_{k=1}^{|\tau|-1} \ \gamma^k \frac{\partial \log(\pi(a_{k}^1|s_{k};\theta^1))}{\partial \theta^1} \frac{\partial \log(\prod_{i=0}^{k-1}\pi(a_{i}^2|s_i;\theta^2))}{\partial \theta^2}^\top \ ( b(s_k) ) \ \biggr] \\
% = &D_{\theta^2\theta^1}\eta
% \end{align}{}
% Since summing over actions, $D_{\theta^i} \int_a \pi(a|s,\theta^i)b(s)da = b(s) D_{\theta^i} 1 = 0$ 







\begin{algorithm}[h!]
\SetAlgoLined
\textbf{Input:} $\pi(.|.;\theta^1)$, $\pi(.|.;\theta^2)$, $V_{\phi}(s)$, N, B, $\alpha$, Choice of $A(s,a^1,a^2;\theta^1,\theta^2)$ mentioned in Sec~\ref{sec:cpg_theory}\\ 
\For{$episode:e=1$ {\bfseries to} $N$}{
 \For{$batch:b=1$ {\bfseries to} $B$}{
  \For{$k=0$ {\bfseries to} $|\tau|-1$}{
  Sample $a^1_k \sim \pi(a^1_k|s_k;\theta_1)$, $a^2_k \sim \pi(a^2_k|s_k;\theta_2)$.\\
  Execute actions $a_k = (a_k^1,a_k^2)$ \\
  Record $\lbrace s_k, a^1_k, a^2_k, r^1_k, r^2_k \rbrace$ in $\tau_{b}$
  }
  Record $\tau_b$ in \textit{M}
  }
%   \textbf{1.} Compute R($\tau$) and $A(s,a^1,a^2;\theta^1,\theta^2)$ $\tau$ in M, \\
%   \textbf{2.} Update critic by $\min_{\phi} \sum_{\tau}||V_{\phi}(\tau) - R(\tau)||^2$\\
\textbf{1.} Estimate $A(s,a^1,a^2;\theta^1,\theta^2)$ with $\tau$ in M\\
  \textbf{2.} Estimate $D_{\theta^1} \eta $, \, $D_{\theta^2} \eta$, \, $D_{\theta^2\theta^1} \eta$, \, $D_{\theta^1\theta^2} \eta$  using \thm~\ref{thm: CPGGradHessianVal}\\
 \textbf{3.} Simultaneously update $(\theta^1,\theta^2)$ using \eq~\ref{eqn: CGDSolution}
}
\caption{Competitive Policy Gradient}
\label{appxalg: cpg}
\end{algorithm}


% \section{Experiments}
% \subsubsection{Linear Bilinear game}
% Next, we considered a cases in which cost is given by \eq \eqref{eq: bilinear }. Here, $K^{1},K^{2}$ are controller policies, modelled as Gaussian distribution. $K^{1*} = K^{2*} = 0$ is a stationary point for this game. Different horizon lengths were considered, if it's is higher, then learning rate has to be low otherwise larger steps make system unstable. With increasing horizon, \gdapg diverges more readily and \cpg takes more time to converge to the origin. We never observed divergence of \cpg in our experiments for reasonable learning rate for the bilinear game. \fig~\ref{Fig: LinearBilinear}, shows plots for trajectories of both the agents with horizon h=2,5 for both \gdapg and \cpg. We trained it for 20,000 iterations, parameters for \gdapg and \cpg were exactly same, although \cpg could have much high lr as compared to \gdapg. Also, it was observed that if critic loss increases, the controller policies moves away from the origin until critic loss is reduces again this is presumably due to exploring new states.  

% \begin{gather*} \label{eq: bilinear }
%     J(K^1,K^2) = \max_{K^1} \min_{K^2} \mathbb{E} \biggl[ \sum_{k=0}^{\infty} {u^1_k}^\top R_{12} u^2_k + {u^2_k}^\top R_{21} u^1_k \biggr] \numberthis
% \end{gather*}


% \begin{figure}[ht]
% 	\centering
%     \begin{subfigure}[t]{0.48\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/sgd_h2.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: sgd_h2}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[t]{0.48\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/cpg_h2.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: cpg_h2}
%     \end{subfigure}
    
%     \begin{subfigure}[t]{0.48\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/sgd_bilinear_lre_h5.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{}
%     \label{Fig: sgd_bilinear_lre_h5}
%     \end{subfigure}
% ~
%   \begin{subfigure}[t]{0.48\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}  
%     \caption{}
%     \label{Fig: cpg_bilinear_lr2_h5_critic_lr2}
%   \end{subfigure}
% %  \includegraphics[width=0.85\linewidth]{images/cpg_bilinear_lr2_h5_critic_lr2.pdf}
% %   \setlength{\abovecaptionskip}{-13pt}
% %   \setlength{\belowcaptionskip}{-10pt}
% \protect\caption{Represents policy trajectories for player 1 and player 2. \protect\mystar{green} is start point and \protect\mystar{red} is end point. (a) \gdapg, h = 2 (b) \cpg, h=2 (c) \gdapg, h=5 (d) \cpg, h=5 }
%   \label{Fig: LinearBilinear}
% \end{figure}


==> extra/extra.tex <==
\begin{lemma}
\label{lemma: GradValCPG}
For any two player CMDP, the gradient of the value function with respect to agent 1, given a policy parametrization pair $(\theta^1, \theta^2)$, starting from $s_0$, is given by,
\begin{gather*}
D_{\theta^1} V(s_0;\theta^1,\theta^2) = \int_s d(s) \int_{a^1} \int_{a^2} \Bigl(\frac{\partial \pi(a^1|s;\theta^1)}{\partial \theta^1}  \pi(a^2|s;\theta^2) Q(s,a^1,a^2;\theta^1,\theta^2) \Bigr) \ da^1 \ da^2 \ ds\,, \numberthis 
\end{gather*}
where, $d(s) = \sum_0^{\infty} \gamma^k Pr(s_0\rightarrow s,\theta^1,\theta^2)$ is the stationary state distribution under the polices $\pi(\theta^1)$ and $\pi(\theta^2)$.

\textit{Proof:} Using Definition \ref{def:ValueDef}, which defines $V^i(s_k;\theta^1, \theta^2)$ and $Q^i(s_k,a^1_{k},a^2_{k};\theta^1, \theta^2)$. We define,
\begin{gather*}
V(s_0;\theta^1,\theta^2) = \int_{a_1^1} \int_{a_1^2} \pi(a_1^1|s_0;\theta^1) \  \pi(a_1^2|s_0;\theta^2) Q(s_0,a_1^1,a_1^2;\theta^1,\theta^2) \ da_1^1 \ da_1^2\,, \numberthis
\end{gather*}
where,
\begin{gather*}
Q(s_0,a_1^1,a_1^2;\theta^1,\theta^2) = r(s_0,a_1^1,a_1^2) + \ \gamma \int_{s1} T(s_1|s_0;a_1^1,a_1^2) \  V(s_1;\theta^1,\theta^2) \ ds_1\,. \numberthis
\end{gather*}
Given $V(s_0;\theta^1,\theta^2)$ we can take the derivative with respect to $\theta_1$,
\begin{align*}
D_{\theta^1} V(s_0;\theta^1,\theta^2) &= \int_{a_1^1} \int_{a_1^2} \Bigl( \frac{\partial \pi(a_1^1|s_0;\theta^1)}{\partial \theta^1} \ \pi(a_1^2|s_0;\theta^2) \  Q(s_0,a_1^1,a_1^2;\theta^1,\theta^2) \Bigr) \ da_1^1 \ da_1^2 
 \\ &+ \int_{a_1^1} \int_{a_1^2} \Bigl( \pi(a_1^1|s_0;\theta^1) \pi(a_1^2|s_0;\theta^2) \ \frac{\partial Q(s_0,a_1^1,a_1^2;\theta^1,\theta^2)} {\partial \theta^1} \Bigr) \ da_1^1 \ da_1^2\,. \numberthis 
 \label{eqn: gradv}
\end{align*}
Motivated by \cite{sutton2000policy}, we can unroll \eq \ref{eqn: gradv} for infinitely many steps, which yields,
\begin{gather*}
D_{\theta^1} V(s_0;\theta^1,\theta^2) = \int_x \sum_0^{\infty} \gamma^k Pr(s_0\rightarrow x,\theta^1,\theta_2) \int_{a_k^1} \int_{a_k^2} \frac{\partial \pi(a_k^1|x;\theta^1)}{\partial \theta^1}  \pi(a_k^2|x;\theta^2) \ Q(x,a_k^1,a_k^2;\theta^1,\theta^2) \ da_k^1 \ da_k^2\,.
\end{gather*}
Using the definition of the stationary state distribution $d(s) = \sum_0^{\infty} \gamma^k Pr(s_0\rightarrow s,\theta^1,\theta^2)$ concludes our proof. $\blacksquare$
\end{lemma}



% @article{sutton2000policy,
%     title={Policy gradient methods for reinforcement learning with function approximation},
%     author={Richard S. Sutton, David McAllester, Satinder Singh, Yishay Mansour},
%     year={1999},
%     journal={Proceedings of the 12th International Conference on Neural Information Processing},
% }


Competitive policy gradient algorithm can be used to learn game strategies by self-play. In a self-play, player competes with itself and improves over time by defeating it self. In contrast to two player training, in self-play the player receive two states from perspective of player 1 and player 2 for the same game instant. The player samples actions from the same policy for two different state instances $s^{1}=[s^{l1}, s^{l2}]$ and $s^{2}=[s^{l2}, s^{l1}]$, where $s^{l1}$ and $s^{l2}$ are local states being player 1 and player 2. Let $\tau = \big( (s^{l1}_k$,$s^{l2}_k,a^1_{k},a^2_{k},r_{k})_{k=0}^{|\tau^1|-1} ,s_{|\tau^1|}\big)$ and $\tau^2 = \big( (s^2_k,a^1_{k},a^2_{k},-r_{k})_{k=0}^{|\tau^2|-1} ,s_{|\tau^2|}\big)$ are trajectories obtained from perspective of player 1 and player 2 respectively. Using \eq~\ref{eq:CPGGradHessianVal1} and \eq~\ref{eq:CPGGradHessianVal}, we can define gradient and bilnear terms estimated from $|\tau^i|$ as $D_{\theta}\eta^i$ and $D_{\theta \theta} \eta^i$ , $i,j \in \lbrace 1,2 \rbrace$, $i \neq j$ as,
\begin{align}
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!D_{\theta} \eta^i &=\int_{\tau^i} \sum_{k=0}^{|\tau^i|-1} \gamma^k f(\tau^i_{0:k};\theta) D_{\theta} (\log\pi(a_k^i|s_k^i;\theta)) Q(s_k^i,a_k^i,a_k^j;\theta) d\tau^i,\!\!\!\!\! \label{eq: selfplayGrad}\\
\!\! D_{\theta \theta} \eta^i &= \int_{\tau^i} \!\sum_{k=0}^{|\tau^i|-1}\!\!\! \gamma^k f(\tau^i_{0:k};\theta) D_{\theta}( \log\pi(a_k^i|s_k^i;\theta)) D_{\theta}( \log\pi(a_k^j|s_k^j;\theta))^{\top}  Q(s_k^i,a_k^i,a_k^j;\theta) d\tau^i \nonumber \\
&+\!\! \int_{\tau^i}\!\!\sum_{k=1}^{|\tau^i|-1}\!\!\!\gamma^k \!f(\tau^i_{0:k};\theta) D_{\theta} (\log\!\! \prod_{l=0}^{k-1}\!\!\pi(a_{l}^i|s_l^i;\theta)) D_{\theta}(\log \pi(a_{k}^j|s_{k}^j;\theta))\!^\top \! Q(s_k^i,a_{k}^i,a_{k}^j;\theta) d\tau^i \ \nonumber\\
&+\!\! \int_{\tau^i}\!\! \sum_{k=1}^{|\tau^i|-1}\!\!\!  \gamma^k  \!f(\tau^i_{0:k};\theta) D_{\theta} (\log \pi(a_{k}^i|s_{k}^i;\theta)) D_{\theta} (\log\!\! \prod_{l=0}^{k-1}\!\!\pi(a_{l}^j|s_l^j;\theta))\!^\top \! Q(s_k^i,a_{k}^i,a_{k}^j;\theta) d\tau^i.\label{eq: selfplayHessian}
% \label{eqn: bilinear_derivative}
\end{align}

Utilizing gradients and bilinear term in \eq~\ref{eq: selfplayGrad} and \eq~\ref{eq: selfplayHessian}, parameters are updated twice which results in the following update rule for self play, 
\begin{align}\label{eqn: selfplayCGDSolution}
\theta^t &\leftarrow \theta + \alpha \bigl( Id + \alpha^2 D_{\theta\theta} \eta^1 D_{\theta\theta}\eta^2 \bigr)^{-1} \bigl( D_{\theta} \eta^1 - \alpha D_{\theta\theta}\eta^1 D_{\theta}\eta^2 \bigr) , \nonumber \\
\theta &\leftarrow \theta^t - \alpha \bigl( Id + \alpha^2 D_{\theta\theta}\eta^2 D_{\theta \theta}\eta^1 \bigr)^{-1} \bigl( D_{\theta}\eta^2 + \alpha D_{\theta\theta}\eta^2 D_{\theta} \eta^1 \bigr) 
\end{align}
where $\theta^t$ is just a temporary variable. 

==> extra/old-6-exp-cpg-trcpo.tex <==
In this section, we empirically study the performance of \cpg and \trcpo with their counterparts \gda and \trpogda respectively, on six games, ranging from single-state repeated games to general sequential games, and tabular games to infinite/continuous states/action games. They are 1) linear-quadratic(LQ) game, 2) bilinear game, 3) matching pennies (MP), 4) rock paper scissors (RPS),  5) Markov soccer, and 6) car racing. These games (first four have known closed-form Nash equilibrium) are representative enough that their study provides insightful conclusions, and challenging enough to carry the core difficulties and interactions in competitive games. 

We show that \cpg and \trcpo converge to stable points, and learns opponent aware strategies, whereas \gda's and \trpogda's greedy approach shows poor performance and even diverges when applied on the bi-linear, MP, and RPS games. For LQ game, when \gda does not diverge, it almost requires 150\% samples, and is $1.5$ times slower as of \cpg.
%
In highly strategic games, where players' policies are tightly coupled, we show that \cpg and \trcpo learn much better interactive strategies. In the soccer game, \cpg and \trcpo players learn to defend, dodge and score goals, whereas \gda and \trpogda players learn how to score when they are initialized with the ball, and give way to the other player otherwise. In the car racing, while \gda and \trpogda show poor performance, \cpg and \trcpo produce competing players, those that learn to block and fake each other. Overall, we observe \cpg and \trcpo considerably outperform their counterparts in terms of convergence, learned strategies, and gradient dynamics.
% When a \cpg and \trcpo trained agents compete with \gda and \trpogda trained agents respectively, we observe significant superior of \cpg and \trcpo agents in both the games.
% Also we compared \trcpo with \cpg, \trcpo converges significantly faster as compared with \cpg in all environment setup. 

% We observe that \cpg converges to a stable point whereas \gda based algorithms diverge in the bi-linear, MP, and RPS game. Unlike \gda, where each player foolishly maximizes his reward which often leads to diverging behavior, \cpg is able to learn an opponent aware strategy. 

% \manish{For eg: In the LQ Game, gradient dynamics was nearly 8\% faster but more importantly \cpg could take steps 10 times larger than that of \gda.}
% \manish{In the soccer game \cpg has 12 times more tendency of seizing ball from \gda as compared to \gda from \cpg} 

% We implemented all algorithms on Pytorch platform~\citep{NEURIPS2019_9015}, and made the code and the videos public %\footnote{https://github.com/manish-pra/Competitive-Policy-Gradient}
% % \footnote{https://github.com/manish-pra/trcpo}
% . In our \gda/\cgd implementation, we deploy Pytorch's autograd package as well as Hessian vector product approach to efficiently compute the gradients and Hessian vector product to compute the bilinear terms in the optimizer.  Moreover, we use conjugate gradient trick to efficiently computed the inverses in \eq\ref{eqn: CGDSolution} which incurs a minimal computational overhead (see \citep{CG_Jonathan1994} for more details). Also we computed inverse matrix vector product only for one player strategy let say $\Delta \theta^1$, and use optimal counter strategy for other player $\Delta \theta^2$ which can be computed without inverse matrix vector product. Also, the last optimal strategy can be used for warm start of conjugate gradient which ease in convergence. 



% \kamyar{Manish, can you elaborate here on the computation?} 
% In the following we split the study to two sections, \textbf{(I)} games that we have their closed form Nash equilibria (games 1,2,3,4), and \textbf{(I)} those that we do not (games 5,6).
% \subsubsection{Games with known Nash Equilibrium}
% \paragraph{Games with known closed-form Nash equilibrium (games 1,2,3,4).}
% Firstly, we considered a \textbf{zero sum LQ game}
% which is studied theoretically and have convergence guarantees~\citep{zhang2019policyZerosum}. This makes LQ game an ideal platform to compare range of allowable step sizes and convergence rate of \cpg with \gda.
% In a LQ game, state and action spaces are continuous, state is propagated using linear dynamics and the cost is quadratic.
% \begin{gather} \label{eqn: lq_game}
%     J(K^1,K^2) = \max\nolimits_{K^1} \min\nolimits_{K^2} \mathbb{E}\big[  \sum\nolimits_{k=0}^{\infty} \gamma^k \bigl({s_k}^T Q s_k + {a^1_k}^T R_{11} a^1_k   + \ {a^2_k}^T R_{22} a^2_k \bigr)\big]  \\
%     \text{where:} \ s_{k+1} = As_k + B_{1}a^1_k + B_{2}a^2_k,~\textit{and} \ \  a^1_{k+1} = -K^1s_k, \ a^2_{k+1} = -K^2s_k \nonumber
% \end{gather}
% \textbf{Games with known closed-form Nash equilibrium (games 1,2,3,4).} 
\textbf{Zero-sum LQ game} is a continuous state-action linear dynamical game between two players, where \gda, with considerably small learning rate, has favorable convergence guarantees~\citep{zhang2019policyZerosum}. This makes LQ game an ideal platform to study the range of allowable step sizes and convergence rate of \cpg and \gda.
We show that, with increasing learning rate, \gda generates erratic trajectories and policy updates, which cause instability (see ``$\oslash$'' in \tab~\ref{tab: LQgameLR}), where as \cpg is robust towards this behavior(the figure (a) in \fig~\ref{Fig: GradDirection} is for the \cpg instantiation of \cpo.). \fig~\ref{fig: LQlr_1e2} shows that \cpg dynamics are not just faster at the same learning rate but more importantly, \cpg can potentially take even larger steps. 
% In the LQ game (defined further in \appx~\ref{appxsec: LQgame}), we observed that with the initially collected samples \gda estimated large gradients, along with high learning rate it resulted in large steps. The resulting policy then generated erratic trajectories in the next rollout, which caused instability and thus \gda did not converge (we denoted this runs with a $\oslash$ in \appx \tab~\ref{tab: LQgameLR}). \cpg is robust towards this behavior and can potentially take even larger steps. \fig~\ref{fig: LQlr_1e2} shows the advantage estimates $\sum_{\tau} f(\tau;\theta^1,\theta^2) \sum_{k=0}^{|\tau|-1}A(s_k,a_{k}^1,a_{k}^2;\theta^1,\theta^2)$ of \gda and \cpg for different learning rates. We can see that \cpg dynamics are not just faster at the same learning rate but more importantly, \cpg allows having larger learning rates.
% as shown in \fig~\ref{fig: LQlr_1e2}.
\begin{figure}[h]
	\hspace{-3.00mm}
	\centering
    \begin{subfigure}[t]{0.27\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/LQlr_1e2.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: LQlr_1e2}
    \end{subfigure}
    \hspace{-6.00mm}
~
    \begin{subfigure}[t]{0.27\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/combined_bilinear_mat.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: combined_bilinear_mat}
    \end{subfigure}
    \hspace{-6.00mm}
   ~
    \begin{subfigure}[t]{0.27\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/combine_matching_pennies.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: combine_matching_pennies}
    \end{subfigure}
    \hspace{-6.00mm}
~
  \begin{subfigure}[t]{0.27\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/combined_rps.pdf}  
    \caption{}
    \label{fig: combined_rps}
  \end{subfigure}
  \hspace{-4.00mm}
  \vspace{-3.00mm}
  \caption{During training \cpg (C) vs \gda (G) a) difference in game objective due to policy update for LQ game b) $\mu^1$ vs $\mu^2$ in bilinear game c) P$\lbrace Head(H),Tail(T)\rbrace$ in MP d) P$\lbrace R,P,S\rbrace$ in RPS game} 
  \hspace{-4.00mm}
  \vspace{-6.00mm}
\end{figure}
% Next we considered a single shot \textbf{bilinear game}, where players exhibit a strong non cooperative behavior. \gda is known to diverge in the bilinear game and hence, it is widely studied to propose other gradient based optimizers~\citep{BalduzziHamiltonian}.

\textbf{Bilinear game} is a state-less strongly non-cooperative game, with reward $r(a^1,a^2)=\langle{a^1},a^2\rangle$, where \gda is known to diverge~\citep{BalduzziHamiltonian}. In this game, $a^1\sim\mathcal{N}(\mu_1,\sigma_1)$ and $a^2\sim\mathcal{N}(\mu_2,\sigma_2)$, and policies parameterized with $(\mu_1,\sigma_1)$, $(\mu_2,\sigma_2)$, and $a^1\sim\mathcal{N}(\mu_1,\sigma_1)$ and $a^2\sim\mathcal{N}(\mu_2,\sigma_2)$.
We show that \gda diverges for all learning rates, whereas \cpg converges to the unique Nash equilibrium \fig~\ref{fig: combined_bilinear_mat}.

\textbf{Matching pennies} and \textbf{Rock paper scissors}, as challenging matrix games with mixed strategies as Nash equilibria, demand opponent aware optimization.\footnote{Traditionally, fictitious and counterfactual regret minimization, as regularized method, are studied~\citep{CFR_RPS}.} We show that \cpg and \trcpo both converge to the unique Nash equilibrium of the MP \fig~\ref{fig: combine_matching_pennies} and RPS \fig~\ref{fig: combined_rps}, whereas \gda and \trpogda diverges, if we pick a policy corresponding to any iteration, it is easily exploitable with a deterministic strategy.
%\gda and \trpogda converge to coarse correlated equilibria (CCE) in its limit cycles~\cite{singleshotCCE_RM,singleshotCCE}, but if we pick a policy corresponding to any iteration, it is easily exploitable with a deterministic strategy. %moves away from the Nash equilibrium for all learning rates.
% \trcpo vs \trpogda results are in \appx~\ref{appx: TRCPOgameNash}. \gda and \trpogda actually approaches near deterministic strategies that are easily exploitable by other deterministic strategies leading to unstable learning.
% In contrast, \cpg and \trcpo agents learn to play the unique mixed Nash strategy, where players anticipate that exploiting a deviation from the Nash equilibrium increases their immediate return, but also renders them to be more exploitable by the opponent. 
Detailed empirical study, formulation and explanation of games 1,2,3,4, in \appx~\ref{appxsec: NashGame}.
% More details and results are documented in \appx~\ref{appxsec: CPGMP} and \appx~\ref{appxsec: CPGRPS}.

% \begin{table}[ht]
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{|c||c|c|c|}
% \hline
%  & Rock & Paper & Scissors  \\
%  \hline \hline
%  Rock & 0,0 & -1,1 & 1,-1   \\
%  \hline
%  Paper & 1,-1 & 0,0 & -1,1   \\
%  \hline
%  Scissors & -1,1 & 1,-1 & 0,0   \\
% \hline
% \end{tabular}
% \caption{Game matrix for rock paper scissors}
% \label{tab: rock_paper_scissors}
% }
% \hfill
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{|c||c|c|}
% \hline
%  & Head & Tail  \\
%  \hline \hline
%  Head & 1,-1 & -1,1   \\
%  \hline
%  Tail & -1,1 & 1,-1   \\
% \hline
% \end{tabular}
% \caption{Game matrix for matching pennies}
% \label{tab: matching_pennies}
% }
% \end{table}

% \paragraph{Markov soccer}
\input{FigTables/MS_GDA_TRCPO}
\label{sec: CPGMarkovSoccer}
% \hspace{1cm}
\begin{wrapfigure}{r}{0.3\textwidth}
\vspace*{-1em}
% \hspace{-2em}
    \begin{subfigure}[t]{0.30\columnwidth}
  	\includegraphics[width=\linewidth]{images/Soccer.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    % \caption{CPG}
% \hspace*{4.em}(a) \cpo
    \end{subfigure}
    \hspace{-2cm}
    % \vspace{-3cm}
  \vspace*{-.5em}
  \caption{Markov Soccer}
  \label{fig: Soccer}
  \vspace{-1em}
\end{wrapfigure}
\textbf{Markov soccer} game~\fig~\ref{fig: Soccer} consists of players A and B that are randomly initialised in the field, that are supposed to pick up the ball and put it in the opponent's goal~\citep{littmansoccer,HeHeOppo}. 
The winner is awarded with +1 and the loser with -1 (see \appx~\ref{appxsec: soccer} for more details). This game is a strategic game that we show all methods converge. Therefore, it a suitable game to compare the learned strategies. In this game, we expect a reasonable agent to learn sophisticated strategies of defending, dodging and scoring. 
%
For different algorithm playing against their counter parts, e.g., \cpg against \cpg and \gda, \fig~\ref{Fig: InteractionBilinear} shows the number of times the ball is seized between the players before one player finally scores a goal, or time-out.
In (\ref{Fig: cpg_cpg_interaction_plot}), \cpg vs \cpg, we see agents seize ball, twice the times as compared to (\ref{Fig: sgd_sgd_interaction_plot}),\gda vs \gda (see $A_2$ and $B_2$ in (\ref{Fig: cpg_cpg_interaction_plot}) and (\ref{Fig: sgd_sgd_interaction_plot})).
In the matches \cpg vs \gda (\ref{Fig: cpg_sgd_interaction_plot}), \cpg trained agent could seize the ball from \gda agent ($A_2$) nearly 12 times more due to better seizing and defending strategy, but \gda can hardly take the ball back from \cpg ($B_2$) due to a better dodging strategy of \cpg agent. Playing \cpg agent against \gda one, we observe that \cpg wins more than 74\% of the games~\fig~\ref{Fig: sgd_cpg_winning_plot}. We observe a similar trend for trust region based methods \trcpo and \trpogda, playing against each other (a slightly stronger results of 85\% wins, A2 in ~\ref{Fig: trpo_trcpo_gmres_interaction_plot} and ~\ref{Fig: cpg_sgd_interaction_plot}).
% Moreover, \trpogda even renders unequal players, due to which player 1 g ets ball quite often which corresponds to high bar at x = $B_2$ and a very low at x=$A_2$ as shown in \fig~\ref{Fig: trpo_trpo_gmres_interaction_plot}.
% Out of both the \trpogda agents, even the best one cannot seize ball from \trcpo as shown in \fig~\ref{Fig: trpo_trcpo_gmres_interaction_plot} at x=$A_2$. 



%
% For comparison between \cpg and \gda, we played 10000 games between them, where in 50\% of the games, \cpg was player A and for the remaining \gda was player A. \cpg won more than 74\% of all games against \gda as shown in \fig~\ref{Fig: sgd_cpg_winning_plot}. (Similar contrast was observed between \trpogda and \trcpo shown in \fig~\ref{Fig: trpo_trcpo_winning_plot}).
%
%

% In order to capture the interaction between players,  \fig~\ref{Fig: InteractionBilinear}[a-c, e-g](see caption) shows the number of times the ball is seized between the players before one player finally scores a goal.
% In \cpg vs \cpg games we see agents seize ball, twice the times as compared to \gda vs \gda (see x=$A_2$, x=$B_2$ in \fig~\ref{Fig: cpg_cpg_interaction_plot} vs \fig~\ref{Fig: sgd_sgd_interaction_plot}).
% In the matches between \cpg vs \gda as shown in \fig~\ref{Fig: cpg_sgd_interaction_plot}, \cpg agent could seize ball from \gda agent (x=$A_2$) nearly 12 times more due to better seizing and defending strategy of \cpg agent but \gda can hardly take the ball back from \cpg (x=$B_2$) due to better dodging strategy of \cpg agent.
% Moreover, \trpogda even renders unequal players, due to which player 1 gets ball quite often which corresponds to high bar at x = $B_2$ and a very low at x=$A_2$ as shown in \fig~\ref{Fig: trpo_trpo_gmres_interaction_plot}.
% Out of both the \trpogda agents, even the best one cannot seize ball from \trcpo as shown in \fig~\ref{Fig: trpo_trcpo_gmres_interaction_plot} at x=$A_2$. 
% \cpg and \trcpo were able to learn better tactics for seizing and dodging the ball, as well as defending its goal post.

%MADDPG implementation details are in \appx~/ref{appx: maddpg_comp}
We also compared \cpg with \maddpg~\citep{lowe2017multi} and \lola~\citep{FoersterLOLA}(this work has empirical study just on MP, random coin, and prisoners dilemma, and we generalized it to MS). We observe that the \maddpg learned policy behaves similar to \gda. When competed against \cpg, \cpg agent wins 80\% of the games as shown in \fig~\ref{fig: EX_cpg_maddpg_winning_plot}. \lola performs better than \gda due to the learning being second order aware but it lose against \cpg for 72\% of matches. For the sake of completeness, we also compared \gdapg, \cpg, \trpogda, and \trcpo playing against each other. \trcpo performs best,\cpg was runner up, then \trpogda, and lastly \gda (see \appx~\ref{appxsec: soccer}).
% \begin{figure}[h]
% \centering
% \hspace{-7.00mm}
%     \begin{subfigure}[t]{0.30\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/Soccer.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
% % \vspace{-6.00mm}
%     \caption{}
%     \label{fig: Soccer}
%     \end{subfigure}
%      \hspace{-2.00mm}
%     ~
%   	\hspace{-5.00mm}
%     \begin{subfigure}[t]{0.26\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/EX_sgd_maddpg_winning_plot.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{\gda vs \maddpg}
%     \label{fig: EX_sgd_maddpg_winning_plot}
%     \end{subfigure}
%     \hspace{-5.00mm}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%NEW FIGURE
% \begin{figure}[!h]
% \hspace{-3.00mm}
% 	\centering
%     \begin{subfigure}[t]{0.26\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/EX_sgd_trpo_winning_plot.pdf}
%     \caption{\gda vs \trpogda}
%     \label{Fig: EX_sgd_trpo_winning_plot}
%     \end{subfigure}
%     \hspace{-4.00mm}
%     ~
%     \begin{subfigure}[t]{0.26\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/EX_trpo_cpg_winning_plot.pdf}
% %   	\setlength{\abovecaptionskip}{0pt}
% %   	\setlength{\belowcaptionskip}{0pt}
%     \caption{\trpogda vs \cpg }
%     \label{Fig: EX_trpo_cpg_winning_plot}
%     \end{subfigure}
%     \hspace{-4.00mm}
%     ~
%     \begin{subfigure}[t]{0.26\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/EX_cpg_trcpo_winning_plot.pdf}
%     \caption{\cpg vs \trcpo}
%     \label{Fig: EX_cpg_trcpo_winning_plot}
%     \end{subfigure}
%     \hspace{-4.00mm}
% ~
%   \begin{subfigure}[t]{0.26\columnwidth}
%   	\centering
%   	\includegraphics[width=\linewidth]{images/EX_sgd_trcpo_winning_plot.pdf}
%     \caption{\gda vs \trcpo}
%     \label{Fig: EX_sgd_trcpo_winning_plot}
%   \end{subfigure}
%   \hspace{-4.00mm}
%   \caption{ Win probability in soccer game played between \gda, \cpg, \trpogda and \trcpo }
%   \label{fig: CompMarkovScoccer}
% \end{figure}
% \vspace{-10.00mm}
% \paragraph{Car Racing}

\label{sec: CPG_ORCA}
Our final experimental setup is a continuous state action space \textbf{Car Racing} game between two race cars, where the goal is to finish the race first. The game involves both, learning a policy that can control a car at the limit of handling, as well as strategic interactions with the opposing car. The test track is challenging, consisting of 13 turns with different curvature can be seen in \fig~\ref{fig: overtaking_manuever_northsouth}. The game is formulated as a zero-sum, with reward $r(s_k,a^1_{k},a^2_{k}) = \Delta \rho_{car_1} - \Delta \rho_{car_2}$, where $\Delta \rho = \rho_{k+1} - \rho_k$ and $\rho_k$ is a progress of the car till $k^{th}$ timestep in the track. If a car crosses track boundaries, it is penalised and the opponent receives rewards, this encourage cars to play rough and push each other into the track boundaries. During a collision, the rear car is penalizes and the car in the front receives rewards, which promotes blocking by the car in front and overtaking by the car in the rear.
% If $car_1$ ($car_2$) crosses track boundaries, then it is freezed i.e $\Delta \rho_{car_1} = 0$ ($\Delta \rho_{car_2} = 0$), which results in its penalization using the above reward formulation corresponding to the $\Delta \rho_{car_2}$ ($\Delta \rho_{car_1}$) of the other agent. Similarly during a collision, the rear car is freezed, which penalizes it and the car in the front receives positive rewards. This formulation promotes blocking by the car in front and overtaking by the car in the rear.
% Here we explain reward shaping to give intuition behind the competition involved. To formulate the racing game between two cars, we convert the objective of finishing the race first without an accident into a zero sum game. First to model our no accident constraints we use a freezing mechanism:
% % (where one car is frozen and other is allowed to ear rewards): 
% (i) If the car is leaving the track we freeze it until the episode ends, 
% (ii) If the cars collide, the rear car is stopped for 1s. Note that this gives an advantage to the car ahead, but in car racing, the following car has to avoid collisions. 
% (iii) The car which finishes first gets a +1 reward and the other car gets -1 reward. Furthermore, an episode ends if both cars are either frozen due to leaving the track or the first car finished the lap. 
% (iv) Finally, to reward racing the players at every time step receive the following reward $r(s_k,a^1_{k+1},a^2_{k+1}) = \Delta \rho_{car_1} - \Delta \rho_{car_2}$, where $\Delta \rho = \rho_{k+1} - \rho_k$. $\rho$ is a progress of the car at $k^{th}$ time step in the track. This reward encourages the player to get as far ahead of the opponent player as possible. 

We trained agents with all \gda, \trpogda, \maddpg, \lola, \cpg and \trcpo in the racing game, even though all players were able to learn to "drive" only \cpg and \trpogda were able to learn how to "race". With \gda based algorithms, only one player was able to learn, this either manifested in one player completely failing and the other finishing the race (\fig~\ref{fig: orca_sgd}), or by an oscillation behavior where when one agent learns to go ahead, the other agent learns to stay at lower progress(\fig~\ref{fig: trpo2gda_oscillations}, \fig~\ref{fig: progress_plot_orca_maddpg}).
%  In \lola training, cars did not learn to drive due to non adaptive learning rate.
Even if at some point one of the players learns to finish one lap, the player does not learn to interact with the other opponent. The players trained with \cpg and \trpogda on the other hand, both progress and learn to finish the lap and to interact with each other (See \fig~\ref{fig: orca_cpg_progress_plot} and \fig~\ref{fig: progress_plot_orca_trcpo}). 
% In all \fig~\ref{fig: ProgressOrca} it is clearly visible that with competitive optimisation both players get better over time, whereas in \gda based algorithm the two player have an oscillation behavior, or at the end, only one of the two players finishes the lap. 

\begin{figure}[h!]
~\hspace{-5.00mm}
	\centering
    \begin{subfigure}[t]{0.22\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/orca_sgd.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: orca_sgd}
    \end{subfigure}
    ~\hspace{-6.00mm}
    ~
    \begin{subfigure}[t]{0.22\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/orca_cpg_progress_plot.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: orca_cpg_progress_plot}
    \end{subfigure}
    ~\hspace{-6.00mm}
    ~
    \begin{subfigure}[t]{0.22\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/trpo2gda_oscillations.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: trpo2gda_oscillations}
    \end{subfigure}
    ~\hspace{-6.00mm}
    ~
    \begin{subfigure}[t]{0.22\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/progress_plot_orca_trcpo.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: progress_plot_orca_trcpo}
    \end{subfigure}
    ~\hspace{-6.00mm}
        ~
    \begin{subfigure}[t]{0.22\columnwidth}
  	\centering
  	\includegraphics[width=\linewidth]{images/progress_plot_orca_maddpg.pdf}
%   	\setlength{\abovecaptionskip}{0pt}
%   	\setlength{\belowcaptionskip}{0pt}
    \caption{}
    \label{fig: progress_plot_orca_maddpg}
    \end{subfigure}
    ~\hspace{-5.00mm}
  \caption{Normalised Progress of agents while training in the car racing game a)\gda b) \cpg c) \trpogda d) \trcpo e) \maddpg, progress = 0 corresponds to start line and 1 is Lap finish}
% \caption{Normalised Progress of agents while training in the car racing game a)\gda $\alpha=5e-5$ b) \cpg $\alpha=5e-5$ c) \trpogda $\delta=1e-5$ d) \trcpo $\delta=1e-5$ e) \maddpg $\alpha = 5e-5$}
  \label{fig: ProgressOrca}
\end{figure}

% To test the policies, we run 5000 episodes with the obtained policy. To evaluate the performance we run three types of races, \gda vs \gda, \cpg vs \cpg, \gda vs \cpg. For each episode, we counted the number of overtakes, the number of collisions with the track constraints, and recorded the lap time. For the \gda vs \cpg test we also counted the number of times which policy won, where we defined winning as finishing first. Since, \gda often collided with the track constraints, for the test, we replaced the freezing with a reset at the reference path routine. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Uncomment this
To test the policies, we performed races between \cpg and \gda, \trcpo and \trpogda, and \cpg and \trcpo. As shown in \tab~\ref{tab: orca_diff_players}, \cpg and \trcpo win almost all races against their counterparts. It is clearly visible that with competitive optimization both players get better over time and able to explore and learn strategic interactions, which results in both \cpg and \trcpo learned a policy that is both faster, more precise and it learns to overtake.
% Although \gda and \trpogda were also able to overtake, almost all of their overtaking maneuvers lead to crash with the track boundaries. 
% Further comparisons and implementation details are in ~\sect~\ref{appxsec: TRCPOorca}. 


% P1 collision tensor(0.3278)
% P2 Collision tensor(0.2434)
% P1 Win tensor(0.7588)
% P2 Win tensor(0.2412)
% P1 Overtake tensor(2.0364)
% P2 Overtake tensor(1.7776)

\begin{table}[ht]
\setlength{\tabcolsep}{12pt}
\centering
\begin{tabular}{l c c c c c c}
\toprule\midrule
 & \multicolumn{2}{c}{\cpg vs \gda} & \multicolumn{2}{c}{\trcpo vs \trpogda} & \multicolumn{2}{c}{\makebox[0pt]{\cpg vs \trcpo}} \\
% \textit{a} & 70 & 30 & 70 & 30 & 70 & 30 \\ [0.5ex]
\midrule
\\\\[-3.9\medskipamount]
 Wins & \textbf{1} & 0 & \textbf{1} & 0 & 0.27 & \textbf{0.73}  \\
 Overtake  & \textbf{1.28} & 0.78 & \textbf{1.27} & 0.77 & 1.04 & \textbf{1.65} \\
 Collision & \textbf{0.18} & 16.17 & \textbf{0.28} & 2.01 & 1.46 &  \textbf{0.23}\\
\bottomrule
\end{tabular}
\caption{Normalised score computed based on 5000 races in the car racing game}
\vspace{-4.00mm}
\label{tab: orca_diff_players}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% \begin{table}[ht]
% \centering 
% \begin{tabular}{|c||c|c|c|}
% \hline
%  & \cpg vs \cpg & \gda vs \gda \\
%  \hline \hline
%  Overtaking per lap & 3.35 & 0.68  \\
%  \hline
%  Track collision per lap & 0.59 & 1.12  \\
%  \hline
%  Laptime  & 10.89 & 13.32  \\
%  \hline
% \end{tabular}
% \caption{Quantitative results for the racing game}
% \label{tab: orca_same_players}
% \end{table}

% In Table \ref{tab: orca_same_players} we can clearly see that \cpg learned a policy that is both faster and more precise, as well as more interactive with about six times as many overtaking maneuvers. Thus, it is not surprising that in the 5000 race between \gda vs \cpg, \gda was only able to win 103 times. For the \gda vs \cpg races, we also noted that the \gda player got ``confused" by the interactive \cpg player which resulted in crashes of the \gda player, since the \gda player never experience such interactions in training. 



% \section{TRCPO Experiments}
% \label{sec:trcpo_experiments}
% In this section we describe an empirical study for \trcpo algorithm on the same platform as used in \sect~\ref{sec:cpg_experiments}. The TRCPO code link and experiment videos are available here. We compared \trcpo with \trpogda, where 2 agents trained with \TRPO in \gda fashion. Empirically, the contrast between \trcpo vs \trpogda similar to that of \cpg vs \gda. \trcpo converges to the unique Nash equilibrium where as \trpogda based algorithm diverges in the bi-linear, MP, and RPS game. 

% Similar to \sect~\ref{fig: TRCPOMarkovScoccer}, \trcpo was competed with \trpogda in the game of soccer. \fig~\ref{fig: TRCPOMarkovScoccer} shows interaction plots.
% It is clear that the \trcpo agent learned much better strategies of seizing ball from opponent and scoring goal, whereas \trpogda could hardly take the ball from \trcpo.
% Also note that 



% Next we compared \trcpo and \trpogda performance on the car racing game similar to ~\sect~\ref{sec: CPG_ORCA}. During training, we observed that \trpogda faces oscillation while training i.e. when an agent maximizes his progress, the other agent performance shrink to low progress due to zero-sum formulation. Also, a few times, one agent collapses near-zero progress, and the other agent learns to drive in this stationary environment as shown in the \fig~\ref{fig: ProgressOrca}. Due to this \trpogda trained agents had hard time to reach the goal together, presumably because of unexplored state space. Where as in the case of \trcpo, as shown in ~\fig ~\ref{fig: progress_plot_orca_trcpo} we observe that both agents are trained together to maximize their progress.  On competing with \trcpo with \trpogda, \trcpo wins almost all the matches due to better interactive strategies learned by \trcpo agent. 



==> macros.tex <==
\newcommand{\CMDP}{\textsc{\small{CoMDP}}\xspace}
% \newcommand{\CMDP}{{\small{Competitive MDP}}\xspace}
\newcommand{\PG}{\textsc{\small{PG}}\xspace}
\newcommand{\RL}{\textsc{\small{RL}}\xspace}
\newcommand{\gdapg}{\textsc{\small{GDA-PG}}\xspace}
\newcommand{\gda}{\textsc{\small{GDA}}\xspace}
\newcommand{\cgd}{\textsc{\small{CGD}}\xspace}
\newcommand{\cpo}{\textsc{\small{CoPO}}\xspace}
\newcommand{\cpg}{\textsc{\small{CoPG}}\xspace}
\newcommand{\cpgsp}{\textsc{\small{CoPG-SP}}\xspace}
\newcommand{\gan}{\textsc{\small{GAN}}\xspace}
\newcommand{\trcpo}{\textsc{\small{TRCoPO}}\xspace}
\newcommand{\trpogda}{\textsc{\small{TRGDA}}\xspace}
\newcommand{\maddpg}{\textsc{\small{MADDPG}}\xspace}
\newcommand{\lola}{\textsc{\small{LOLA}}\xspace}
\newcommand{\MARL}{\textsc{\small{MARL}}\xspace}
\newcommand{\stermination}{s_{T}}
\newcommand{\GAE}{GAE}

\newcommand*{\eg}{e.g.\@\xspace}
\newcommand*{\eq}{Eq.}
\newcommand*{\fig}{Fig.}
\newcommand*{\lem}{Lem.}
\newcommand*{\tab}{Tab.}
\newcommand*{\appx}{Apx.}
\newcommand*{\sect}{Sec.}
\newcommand*{\thm}{Thm.}
\newcommand*{\alg}{Alg.}
\newcommand*{\prop}{Prop.}

\newcommand{\GTRPO}{\textsc{\small{GTRPO}}\xspace}
\newcommand{\GPPO}{\textsc{\small{GPPO}}\xspace}
\newcommand{\POMDP}{\textsc{\small{POMDP}}\xspace}
\newcommand{\MDP}{\textsc{\small{MDP}}\xspace}
\newcommand{\TRPO}{\textsc{\small{TRPO}}\xspace}
\newcommand{\PPO}{\textsc{\small{PPO}}\xspace}
\newcommand*{\Scale}[2][4]{\scalebox{#1}{$#2$}}
\newcommand{\cost}{c}
\newcommand{\vecy}{\vec y}
\newcommand{\history}{\mathfrak{H}}
\newcommand{\trans}{T}
\newcommand{\obs}{O}
\newcommand{\policy}{\Pi}
\newcommand{\vpi}{{\pi}}
\newcommand{\vobs}{\vec{o}}
\newcommand{\stait}{\omega}
\newcommand{\rxa}{\Gamma}
\newcommand{\rya}{\Upsilon}
\newcommand{\U}{\mathcal{U}}
\newcommand{\Est}{M_1}
\newcommand{\End}{M_2}
\newcommand{\Erd}{M_3}
\newcommand{\decompos}{\gamma}
\newcommand{\pertM}{\Delta M_3}
\newcommand{\pertMM}{\Delta \tilde{M_3}}
\newcommand{\samplenum}{m_s}
\newcommand{\reward}{\Psi}
\newcommand{\tuple}{\mathcal{M}}
\newcommand{\bellman}{\mathcal{E}}
\newcommand{\whole}{\tilde{\mathcal{M}}}
\newcommand{\approxim}{\breve{\mathcal{M}}}
\newcommand{\subst}{{\breve{\eta}}_{\vpi^*}}
\newcommand{\effect}{v}
\newcommand{\block}{\Xi}
\newcommand{\vect}{Vec}
\newcommand{\rprob}{z}
\newcommand{\past}{n}
\newcommand{\smucrl}{\textsc{\small{SM-UCRL}}\xspace}
\newcommand{\tslive}{\textsc{\small{TS-LIVE}}\xspace}
\newcommand{\olive}{\textsc{\small{OLIVE}}\xspace}
\newcommand{\cdp}{\textsc{{CDP}}\xspace}
\newcommand{\cdps}{\textsc{{CDPs}}\xspace}
\newcommand{\ts}{\textsc{TS}\xspace}
\newcommand{\ofu}{\textsc{OFU}\xspace}
\newcommand{\ucrl}{\textsc{\small{UCRL}}\xspace}
\newcommand{\mdp}{\textsc{\small{MDP}}\xspace}
\newcommand{\pomdp}{\textsc{\small{POMDP}}\xspace}
\newcommand{\Azuma}{\mathcal{J}}
\newcommand{\Dr}{D_{\text{ratio}}}
\newcommand{\Ke}{\mathcal{K}_\epsilon}
\newcommand{\Le}{L_\epsilon}
\newcommand{\w}{W}
\newcommand{\VV}{B}
\newcommand{\vv}{b}
\newcommand{\HH}{S}
\newcommand{\hhh}{s}
\newcommand{\deltaO}{d_O}

\newcommand*{\defeq}{\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt
                     \hbox{\scriptsize.}\hbox{\scriptsize.}}}%
                     =}

% Misc symbols
\renewcommand{\Re}{\mathbb{R}}
\newcommand{\calP}{\mathcal P}
\newcommand{\PP}{\mathbb P}
\newcommand{\F}{\mathcal F}
\newcommand{\Z}{\mathcal Z}
\newcommand{\A}{\mathcal A}
\newcommand{\B}{\mathcal B}
\newcommand{\X}{\mathcal X}
\newcommand{\T}{\mathcal T}
\newcommand{\KL}{\mathcal D_{KL}}
\newcommand{\wKL}{\wh{\mathcal{D}}_{KL}}
\newcommand{\D}{\mathcal D}
\newcommand{\Gr}{\nabla_{\theta}}
\newcommand{\Greta}{\nabla \eta}
\newcommand{\Grrho}{\nabla \rho}
\newcommand{\Grphi}{\nabla_\phi}
\newcommand{\adv}{A}
\newcommand{\TN}{N}
\newcommand{\hh}{\hat h}
\newcommand{\hL}{\hat L}
\renewcommand{\L}{\mathcal L}
\newcommand{\Hyp}{\mathcal H}
\newcommand{\Y}{\mathcal Y}
\newcommand{\V}{\mathcal V}
\newcommand{\M}{\mathcal M}
\renewcommand{\S}{\mathcal S}
\newcommand{\C}{\mathcal C}
\newcommand{\K}{\mathcal K}
\newcommand{\E}{\mathbb E}
\newcommand{\calE}{\mathcal E}
\newcommand{\Cov}{\textnormal{Cov}}
%\newcommand{\V}{\mathbb V}
\newcommand{\Prob}{\mathbb P}
\newcommand{\I}{\mathbbm 1}
\newcommand{\N}{\mathcal N}
\newcommand{\balpha}{\boldsymbol \alpha}
\newcommand{\bmu}{\boldsymbol \mu}
\newcommand{\bSigma}{\boldsymbol \Sigma}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\MV}{\textnormal{MV}}
\newcommand{\hMV}{\widehat{\textnormal{MV}}}
\newcommand{\barmu}{\bar\mu}
\newcommand{\hmu}{\hat\mu}
\newcommand{\tmu}{\tilde\mu}
\newcommand{\barvar}{\bar\sigma^2}
%\newcommand{\hvar}{\hat\sigma^2}
\newcommand{\tvar}{\tilde\sigma^2}
\newcommand{\R}{\mathcal{R}}
\newcommand{\hR}{\widehat{\mathcal{R}}}
\newcommand{\tR}{\widetilde{\mathcal R}}
%\newcommand{\var}{\sigma^2}
\newcommand{\invdelta}{1/\delta}
\newcommand{\boldR}{\mathbb R}
\newcommand{\eps}{\varepsilon}
\newcommand{\mvlcb}{\textnormal{\texttt{MV-LCB }}}
\newcommand{\ucb}{\textnormal{\textsl{UCB }}}
\newcommand{\ucbv}{\textnormal{\textsl{UCB-V }}}
\newcommand{\mvlcbt}{\textnormal{\texttt{MV-LCB(t) }}}
\newcommand{\htheta}{\hat{\theta}}
\newcommand{\hi}{\hat{i}}
\newcommand{\btheta}{\bar{\theta}}
\newcommand{\tTheta}{\widetilde{\Theta}}

\newcommand{\cvar}{\textnormal{C}}
\newcommand{\hcvar}{\widehat{\textnormal{C}}}
\newcommand{\var}{\textnormal{V}}
\newcommand{\hvar}{\widehat{\textnormal{V}}}
\newcommand{\Pinit}{P_\varnothing}



\newcommand{\avg}[2]{\frac{1}{#2} \sum_{#1=1}^{#2}}
\newcommand{\hDelta}{\widehat{\Delta}}
\newcommand{\hGamma}{\widehat{\Gamma}}

\newcommand{\wt}{\widetilde}
\newcommand{\wh}{\widehat}
\newcommand{\wb}{\overline}
 \newcommand{\mbb}{\mathbbm}

% Propositions
%
%\newtheoremstyle{dotless}{}{}{\itshape}{}{\bfseries}{}{ }{}
%\theoremstyle{dotless}
\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}

\newtheorem{definition}{Definition}
\newtheorem{theorem*}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{remark}{Remark}
% \newtheorem{proof}{Proof}
% \newtheorem*{proof*}{Proof}
% Misc
%\newcommand{\note}[1]{\textbf{Note.} \textit{#1}}
%\newcommand{\TODO}[1]{(\textbf{TODO: {#1}})}
%\renewcommand{\remark}[1]{\textbf{Remark #1.}}

==> sections/9-broader_impacts.tex <==
\section*{Broader Impact}
The research work presented in this paper can positively impact the field of reinforcement learning, game theory, and multi-agent systems. The \RL field as a whole aims to develop the next level of automation by creating intelligent robots/processes that are capable of making smart sequential decisions. Our work contributes towards it.  On a positive side, Automation can reduce human dependence. Robots can show more strength, durability, accuracy, and in some cases “beyond human” decision-making ability, which results in achieving better resource management, productivity, and higher quality results. Further, it can reduce the costs of processes by getting rid of  “repetitive” or “time-consuming” tasks from workers. If successful, it can lead to machines taking care of those relevant jobs. If happen in a short time, it could potentially have a negative impact on the labor market and in general on the stability of the economic market.

Further research in \RL and multi-agent systems can potentially make robots intelligent enough to work alongside humans or other robots. Our work is a step in this direction to make robots learn better and stable strategies efficiently while operating alongside other players.  Due to the immense number of applications involving multiple agents, agents for such environments can create a huge positive impact. For example, consider a complex traffic scenario, where an AI agent can ease human lives by making complicated decisions for them. Moreover, it can eliminate the risk of fatalities due to human errors. But the failure of such systems can create mass destruction of properties and human lives. Our work contributes toward building more robust multi-agent systems to reduce the probability of such mass failures.

% The research work presented in this paper can positively impact the field of reinforcement learning, games, and multi-agent systems. The \RL field as a whole aims to bring the next level of automation by creating intelligent robots/processes that are capable of making smart sequential decisions. Our work contributes towards it.  On a positive side, Automation can reduce human dependence. Robots have shown more strength, durability, accuracy, and in some cases “beyond human” decision-making ability, which results in achieving better resource management, productivity, and higher quality results. Further, it can also reduce the costs of processes by eliminating “repetitive” or “time-consuming” tasks for workers. But on the contrary, if successful it can lead to large-scale job loss, which could have a negative impact on the labor market and in general on the stability of the economic market.

% Further, research in \RL and multi-agent systems can potentially make robots intelligent enough to work along with humans or other robots. Our work is a step in this direction to make robots learn better and stable strategies efficiently while operating alongside other players.  Due to immense number of applications involve multiple agents, agents for such environments can create a huge positive impact. For example, consider a complex traffic scenario, where an AI agent can ease human lives by making complicated decisions for them. Moreover, it can eradicate the risk of fatalities due to human errors and intuitions. But the failure of such systems can create mass destruction of properties and human lives. Our work contributes toward building more robust multi-agent systems to reduce the probability of such mass failures.
% \manish{work in progress}
% The research presented in this paper can create an impact in the field of reinforcement learning, games, and multi-agent systems. The field of \RL as a whole aims to bring the next level of automation by creating smart and intelligent machines/processes that are capable of making sequential decisions. This can have a huge positive impact and our work contributes towards it. It can ease human lives by making complicated decisions for them as an example consider a complex traffic scenario. In turn, this eradicates the risk of fatalities due to human errors and intuitions. Further, it can also reduce the costs of processes by eliminating “repetitive” or “time-consuming” tasks for workers. But on the contrary, if successful it can lead also to large-scale job loss, which can negatively impact the labor force and stability of the economic market.

% \RL has roots in psychology, biology, and neuroscience. Further research can potentially make robots intelligent enough to work along with humans. Our work is a step in this direction to make robots learn better and stable strategies efficiently while operating alongside other players. On a positive side, it can reduce human dependence. Moreover, robots can show more strength, durability, accuracy, and “beyond human” decision-making abilities, which helps in better resource management, more precision, and higher quality results. Negatively, the failure of such systems can create mass destruction of property and human lives. Our work contributes toward building more robust multi-agent systems to reduce the probability of such mass failures.

%, by making robots learn stable and interactive strategies.
% , and hence perform better alternative to the existing methods
  


% Further research in this direction would overcome failures of current algorithms and potentially lead to more robust agents.  


% The negative impact of failure of such a system depends on the level of autonomy used in the system. In the highest level of autonomy it can be danger to life but on the contrary this work helps to make existing methods robust to such failure cases. 

% This work does not involve or raise bias or fairness related issue towards any living species. 
 
% Later down the line, further research in this direction could potentially enable agents to take up complex task, learn and perform it efficiently. As an \RL agent it will learn with rewards, which can defer from human world and it could lead to fatalities. In real world an RL agent can often lead to unsafe states. 



% Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
% Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
% who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
% biases in the data. If authors believe this is not applicable to them, authors can simply state this.

% Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}


